Gradient-Free Optimization for Non-Smooth Saddle Point Problems under Adversarial Noise

We consider non-smooth saddle point optimization problems. To solve these problems, we propose a zeroth-order method under bounded or Lipschitz continuous noise, possible adversarial. In contrast to the state-of-the-art algorithms, our algorithm is optimal in terms of both criteria: oracle calls complexity and the maximum value of admissible noise. The proposed method is simple and easy to implement as it is built on zeroth-order version of the stochastic mirror descent. The convergence analysis is given in terms of the average and probability. We also pay special attention to the duality gap $r$-growth condition $(r\geq 1)$, for which we provide a modification of our algorithm using the restart technique. We also comment on infinite noise variance and upper bounds in the case of Lipschitz noise. The results obtained in this paper are significant not only for saddle point problems but also for convex optimization.

==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/gas_upper.tex <==
\section{``Upper'' bound in the case of Lipschitz noise}
Now let us consider a stochastic convex optimization problem of the form
\begin{equation}\label{eq:conv_prob}
    \min_{x \in \X} F(x) \triangleq \mathds{E}_{\xi} f(x,\xi),
\end{equation}
where  $X \subseteq \R^{d}$ is a convex set, and for all $\xi$, $f(x,\xi)$ is convex in $x\in\X$  and satisfies Assumption \ref{ass:Lip_obj}. The empirical counterpart of this problem \eqref{eq:conv_prob} is
% for all $\xi$ 
%and for all $x,y \in \X$, $\xi$
% \begin{equation}\label{M}
%      \left|f(y,\xi) - f(x,\xi)\right| \le M_2 \|y-x\|_2.
% \end{equation}
% where $p\ge 1$.  
% Consider Monte Carlo (also known as Sample Average Approximation) approach for \eqref{eq:conv_prob} \cite{shapiro2021lectures}:
\begin{equation}\label{emp_prob}
    \min_{x \in \X} \hat{F}(x)\triangleq \frac{1}{N}\displaystyle\sum_{k = 1}^{N} f(x, \xi^k).
\end{equation}
The exact solution ($\nicefrac{\e}{2}$-solution)  of \eqref{emp_prob} is an $\e$-solution of \eqref{eq:conv_prob} if the sample size $N$ is taken as follows  \cite{shapiro2005complexity,feldman2016generalization}
\begin{equation}\label{LB}
   N=\widetilde{ \Omega}\left(d {M_2^2 \D_2^2}/{\e^{2}}\right),
\end{equation}
where $\D_2$ is the diameter of $X$ in the $\ell_2$-norm. This lower bound is tight \cite{shapiro2005complexity,shapiro2021lectures}.

On the other hand,  $\hat{F}(x)$ from \eqref{emp_prob} can be considered as an inexact zeroth-order oracle for $F(x)$ from \eqref{eq:conv_prob}. If $\delta(x) = F(x) - \hat{F}(x)$ then  in $\text{Poly}\left(d,1/\e\right)$ points $y,x$ with probability $1 - \beta$ the following holds 
$$\left|\delta(y) - \delta(x)\right| = \O\left(\frac{M_2\|y-x\|_2}{\sqrt{N}}\ln\left(\frac{\text{Poly}\left(d,1/\e\right)}{\beta}\right)\right)= \widetilde{\O}\left(\frac{M_2\|y-x\|_2}{\sqrt{N}}\right),$$
i.e., $\delta(x)$ is a Lipschitz function with Lipschitz constant 
\begin{equation}\label{delta}
    {M_{2,\delta}} = \widetilde{\O}\left({M_2}/{\sqrt{N}}\right).
\end{equation}

Let us assume there exists a zeroth-order algorithm that can solve \eqref{eq:conv_prob} with accuracy  $\e$ in $\text{Poly}\left(d,1/\e\right)$ oracle calls, where an oracle returns an inexact value of $F(x)$ with a noise that has the following Lipschitz constant 
$$M_{2,\delta}  \gg \frac{\e}{\D_2\sqrt{d}}.$$ 
We can use this algorithm to solve problem \eqref{eq:conv_prob} with $N$ determines from (see \eqref{delta})
$$\frac{M_2}{\sqrt{N}} \gg \frac{\e}{\D_2\sqrt{d}},$$
i.e.
$$N \ll d{M_2^2 \D_2^2}/{\e^2},$$
that contradicts  the lower bound \eqref{LB}. 

Thereby it is impossible in general to solve with accuracy $\e$ (in function value) Lipschitz convex  optimization problem via $\text{Poly}\left(d,1/\e\right)$ inexact zero-order oracle calls if Lipschitz constant of noise is greater than  
\begin{equation}\label{LBN}
   {\e}/({\D_2\sqrt{d}}).
\end{equation}

Unfortunately, we obtain this upper bound assuming that $\text{Poly}\left(d,1/\e\right)$ points were chosen regardless of $\left\{\xi^k\right\}_{k=1}^N$. That is not the case for the most of practical algorithms, in particular, considered above. But the dependence of these points from $\left\{\xi^k\right\}_{k=1}^N$ is significantly weakened by randomization we use in zero-order methods. So we may expect that nevertheless this upper bound still takes place. 

For arbitrary $\text{Poly}\left(d,1/\e\right)$ points (possibly that could depend on $\left\{\xi^k\right\}_{k=1}^N$) we can guarantee only (see \cite{shapiro2021lectures})
\begin{equation}\label{delta_}
    M_{2,\delta}  = \widetilde{\O}\left(\sqrt{d}{M_2}/{\sqrt{N}}\right).
\end{equation}
That is large than \eqref{delta}. Consequently, the upper bound \eqref{LBN} should be 
rewritten as
\begin{equation}\label{LBN_}
    {\e}/{\D_2}.
\end{equation}

We believe that \eqref{LBN_} is not tight upper bound, rather than \eqref{LBN}. That is, there exists algorithm (see Algorithm \ref{alg:zoSPA}) that can solve \eqref{eq:conv_prob} with accuracy $\e$ (in function value) via $\simeq dM_2^2\D_2^2/\e^2$ inexact zero-order oracle calls if Lipschitz constant of noise is bounded from above by $M_{2,\delta}  \lesssim \e/(\D_2\sqrt{d})$. But there are no algorithms reaching the same accuracy $\e$ by using $\text{Poly}\left(d,1/\e\right)$ inexact zero-order oracle calls if Lipschitz constant of noise is bounded from above by $M_{2,\delta}  \gg \e/(\D_2\sqrt{d})$, in particular, for $M_{2,\delta} $ given by \eqref{LBN_}.

Note, that \eqref{LB} holds  also if $f(x,\xi)$ has Lipschitz $x$-gradient \cite{feldman2016generalization}. So we can expect that obtained above lower bounds take place also for smooth problems. Known maximal level of noise bounds for concrete algorithms confirm this \cite{gasnikov2017stochastic,berahas2021theoretical,vasin2021stopping}.

==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/gasnikov.tex <==
\section{The Basic Idea and Possible Generalization}
In this section, we give some possible generalizations
for our results. For simplicity, we consider a non-stochastic non-smooth convex optimization problem in the Euclidean proximal setup
% For visibility reasons we explain below the main idea on the case of non stochastic convex optimization problem in euclidean proximal setup:
\begin{equation}\label{prblm}
    \min_{x\in \X\subseteq \mathbb{R}^d} f(x),
\end{equation}
where $X \subseteq \R^{d}$ is a convex set and $f$ is  $M$-Lipschitz continuous.
In this problem, we replace the non-smooth objective $f(x)$ by its smooth  approximation $f^{\tau}(x)$ defined in  \eqref{eq:smoothedfunc}, i.e.:
$
f^{\tau}(x)\triangleq  \mathbb{E}_{\tilde{e}} f(x + \tau \tilde{e})
$, where  $\tau > 0$ is some constant and $\tilde{e}$ is a  vector 
picked uniformly at random from the Euclidean unit ball $\{\tilde{e}:\|\tilde{e}\|_2\leq 1\}$.
% Here $\tilde{e}$ is a random vector uniformly distributed on  the Euclidean ball in $\mathbb{R}^d$ with center at $0$ and radius $1$. 
From \cite{duchi2015optimal} it follows that
\begin{equation}\label{apprx}
f(x) \leq f^{\tau}(x) \leq f(x) + \tau M.
\end{equation}
Let the objective $f(x)$    can be not directly observed but instead, its noisy approximation $\vp(x) \triangleq f(x) + \delta(x)$ can be queried, where $\delta(x)$ is some adversarial noise such that $\|\delta(x)\| \leq \Delta$.
Similarly to  \eqref{eq:grad_approx} we can estimate the gradient of $\vp(x)$ d by the following gradient-free approximation 
\begin{equation*}\label{sg}
  g(x,e)    = \frac{d}{2\tau}\left(\vp(x+\tau e) - \vp(x-\tau e)\right)e,
\end{equation*}
 Due to 
\cite{gasnikov2017stochastic} (see also Lemma~\ref{lm:dotprodvece}) for all $r \in \R^d$
\begin{equation}\label{unbias}
 \mathbb{E}_e  \left[ \langle g(x, e)  - \nabla f^{\tau}(x), r\rangle \right]\lesssim \sqrt{d}{\Delta\|r\|_2}{\tau^{-1}}
 \end{equation}
 and \cite{shamir2017optimal,beznosikov2020gradient}
 \begin{equation}\label{var}
   \mathbb{E}_e \left[ \| g(x, e) - \mathbb{E}_e \nabla f^{\tau}(x, e) \|^2_2 \right]\simeq \mathbb{E}_e \left[ \| g(x, e) \|^2_2 \right] \lesssim 
   d M^2 + {d^2\Delta^2}{\tau^{-2}} ,
    \end{equation}
where $e$ is a random vector uniformly distributed on    the Euclidean unit sphere $\{e:\|e\|_2= 1\}$.  Bound  \eqref{unbias} is $\sqrt{d}$ better than in the bounds from \cite{beznosikov2020gradient,akhavan2020exploiting}. Moreover, for $M_{2,\delta}$-Lipschitz noise, Eq. \eqref{unbias} can be rewritten as follows
\begin{equation}\label{unbias_2}
 \mathbb{E}_e \left[ \langle  g(x, e)  - \nabla f^{\tau}(x), r\rangle \right] \lesssim \sqrt{d}M_{2,\delta}\|r\|_2.
 \end{equation}
We will say that an algorithm $\bf A$ (with $g(x, e)$ oracle) is \textit{robust} for  $f^{\tau}$ if the bias in the l.h.s. of \eqref{unbias} does not accumulate over method iterations. That is, if for $\bf A$ with $\Delta = 0$ 
$$\mathbb{E}f^{\tau}(x^N) - \min_{x\in \X} f^{\tau}(x)\le \Theta_A(N),$$
then with $\Delta > 0$ and (variance control)  ${d^2\Delta^2}{\tau^{-2}} \lesssim d M^2$, see \eqref{var}:  
\begin{equation}\label{ns}
    \mathbb{E} f^{\tau}(x^N) - \min_{x\in \X} f^{\tau}(x)= O\left(\Theta_A(N) + \sqrt{d}{\Delta\D}{\tau^{-1}}\right),
\end{equation}
 where $\D$ is a diameter of $\X$. Here  $N$ should be taken such that the first term of the r.h.s. of Eq. \eqref{ns}  is not smaller than the second one. Similar definition can be made for \eqref{unbias_2}. 
 Many known methods are robust, e.g., stochastic versions of mirror descent, mirror prox, gradient method and fast gradient  method are robust
\cite{juditsky2012first-order,d2008smooth,cohen2018acceleration,dvinskikh2020accelerated,dvinskikh2021decentralized,gorbunov2019optimal}. \\
Now we explain how to obtain the bound on the level of noise $\Delta$.

\textbf{Approximation.}
To approximate non-smooth function $f(x)$ by smooth function $f^{\tau}(x)$, constant $\tau$ should be taken as follows: $\tau = \frac{\e}{2M}$ (see \eqref{apprx}).

\textbf{Variance control.} To control the variance and obtain 
the second moment of the stochastic gradient with $\Delta>0$ and $\Delta=0$ of the same order, $\Delta$ should be taken not bigger that (see \eqref{var}):
$\Delta\lesssim\frac{\tau M}{\sqrt{d}}.$

\textbf{Bias.} From \eqref{ns} we will have more restrictive condition on the level of noise:
$\Delta\lesssim\frac{\tau\e}{\D\sqrt{d}}.$
Combining  the bias condition and approximation condition leads to the following bound on the $\Delta$:
\begin{equation}\label{lon}
\Delta \lesssim\frac{\e^2}{\D M\sqrt{d}}.
\end{equation}
For Lipschitz noise and for saddle point problems, the same bound holds by the same reasoning.

More interestingly, as stochastic (batched) versions of fast gradient method and mirror prox are also robust \cite{gorbunov2019optimal,stonyakin2021inexact} and $f^{\tau}$ has $\nicefrac{\sqrt{d}M}{\tau}$-Lipschitz gradient \cite{duchi2012randomized,gasnikov2022power}, we can improve the results of this  paper by using parallelized smoothing technique from \cite{gasnikov2022power}. For instance, for non-smooth convex optimization problem \eqref{prblm}, the gradient-free method from \cite{gasnikov2022power} (with optimal number of oracle calls and the best known number of consistent iterations) provides also the highest possible level of noise, given by \eqref{lon}.


==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/intro_main.tex <==
\section{Introduction}\label{sec:intro}
In this paper, we consider a stochastic non-smooth \textit{saddle point} problem of the form
\begin{equation}\label{eq:min_max_problem}
    \min_{x\in \X} \max_{y\in \Y} ~f(x,y),
\end{equation}
where $f(x,y) \triangleq \E_\xi \left[f(x,y,\xi)\right]$ is the expectation, w.r.t. $\xi \in \Xi$,  $f: \X \times\Y \to \R $   is convex-concave and Lipschitz continuous, and  $\X \subseteq \R^{d_x}$, $\Y \subseteq \R^{d_y}$ are  convex compact sets. We will denote $z_* = (x_*,y_*)$ a solution of the problem \eqref{eq:min_max_problem}. The standard interpretation of such min-max problems is the antagonistic game between a learner and an adversary, where the equilibria are the saddle points  \cite{neumann1928theorie}.
Now the interest in   saddle point problems 
is renewed due to the popularity of generative adversarial networks (GANs), whose training involves solving  min-max problems \cite{goodfellow2014generative,chen2017zoo}. 

Motivated by  many applications in the field of  reinforcement learning \cite{choromanski2018structured,mania2018simple} and statistics,  where only a  black-box access to the function values of the objective is available, we consider \textit{zeroth-order} oracle (also known as gradient-free oracle).  Particularly, we mention the classical problem of adversarial multi-armed bandit \cite{flaxman2004online,bartlett2008high,bubeck2012regret}, where a learner receives a feedback  given by the function evaluations from an adversary. Thus, zeroth-order methods  \cite{conn2009introduction}  are the workhorse technique when the    gradient information is prohibitively expensive or even  not available and optimization is performed based only on the function evaluations.


\paragraph{Related Work and Contribution.}

Zeroth-order methods in the non-smooth setup were developed in a wide range of works  \cite{polyak1987introduction,spall2003introduction,conn2009introduction,duchi2015optimal,shamir2017optimal,nesterov2017random,gasnikov2017stochastic,beznosikov2020gradient,gasnikov2022power}.  Particularly, in \cite{shamir2017optimal}, an optimal algorithm  was provided as an improvement to the work \cite{duchi2015optimal} for a non-smooth case but Lipschitz continuous  in stochastic convex optimization problems.
However, this algorithm uses the exact function evaluations that can be infeasible in some applications. 
Indeed, an objective $f(z,\xi)$    can be not directly observed but instead, its noisy approximation $\vp(z,\xi) \triangleq f(z,\xi) + \delta(z)$ can be queried, where $\delta(z)$ is some adversarial noise.
This noisy-corrupted setup was considered in
many works \dd{\cite{polyak1987introduction,granichin2003randomized}}, however, such an algorithm that is optimal in terms of the number of oracle calls complexity and the maximum value of adversarial noise has not been proposed.
For instance,   in \cite{bayandina2018gradient,beznosikov2020gradient},  optimal algorithms in terms of oracle calls complexity were proposed, however, they are not optimal in terms of the maximum value of the noise. 
%Namely, the bounds contain non-optimal term $1/d$ and$1/\sqrt{d}$  respectively, where  $d \triangleq d_x + d_y$ is the problem size.
 In papers \cite{risteski2016algorithms,vasin2021stopping},   algorithms are optimal in terms of the maximum value of the noise, however, they are not optimal in terms of the oracle calls complexity.  
In this paper, we provide an accurate analysis of a gradient-free version of the mirror descent method with an inexact oracle that shows that  the method is optimal both in terms of the inexact  oracle calls complexity and the maximum admissible noise.  We consider two possible scenarios for the nature of the adversarial noise arising in different applications: the noise is bounded by a small value or  is Lipschitz.  Table \ref{Table1} demonstrates our contribution by comparing our results with the existing optimal bounds. Finally, we consider the case when the objective satisfies the $\gamma$-growth condition and restate the results.



\begin{table}[!h]
   \centering
    \small
    \vspace{-0.3cm}
    \caption{Summary of the Contribution}
    \label{Table1}
    \begin{threeparttable}
    \begin{tabular}{|c|c|c|c|c|c|}
         \hline
         \scriptsize \textsc{Paper} 
        %&\begin{tabular}{c}\bf Supports \\ \bf distributed \\ \bf setup? \end{tabular}
        & \begin{tabular}{c} 
        %  \scriptsize \textsc{$\min$}
        % \scriptsize \textsc{or} \\ 
        %   \scriptsize \textsc{ $\mathbf  \min\max$ }
          \scriptsize \textsc{Problem}\tnote{{\color{blue}(1)}}
        \end{tabular} 
        & \begin{tabular}{c}
      \scriptsize \textsc{Expectation}  \\ 
        \scriptsize \textsc{or Large } \\
          \scriptsize \textsc{ Deviation }
        \end{tabular}  
        & \begin{tabular}{c}
      \scriptsize \textsc{Is the  Noise} \\ 
      \scriptsize \textsc{Lipschitz?}
        \end{tabular} 
         & \begin{tabular}{c}
         \scriptsize \textsc{Number of} \\  \scriptsize \textsc{Oracle Calls} \\ 
        \end{tabular} 
            & \begin{tabular}{c}
      \scriptsize \textsc{Maximum Noise}  
        \end{tabular} \\
    \hline\hline
% \tiny{\citet{gasnikov2017stochastic}}\tnote{{\color{blue}(1)}}  & 
%   \scriptsize{ convex optimization} & $\E$ & \xmark &  $\nicefrac{n}{\e^2}$ & $\min\left\{ \nicefrac{\e^{3/2}}{\sqrt{n}}, \nicefrac{\e}{n}\right\}$\\
  %%%%%%%             
\tiny{\citet{bayandina2018gradient}}   &   \scriptsize{ convex}  & $\E$& \xmark   &   $\nicefrac{d}{\e^2}$ & $\nicefrac{\e^2}{d^{3/2}}$\\   
  %%%%%%%     
    \tiny{\citet{beznosikov2020gradient}}   &   \scriptsize{ saddle point} & $\E$ & \xmark  &  $\nicefrac{d}{\e^2}$ & $\nicefrac{\e^2}{d}$\\ 
    %%%%%%%    
    \tiny{\citet{vasin2021stopping}}   &   \scriptsize{ convex} & $\E$ & \xmark   &  ${\rm Poly}\left(d, \nicefrac{1}{\e}\right)$ & $\nicefrac{\e^2}{\sqrt d}$\\\ 
%%%%%%%    
 
\tiny{\citet{risteski2016algorithms}}   &   \scriptsize{ convex} & $\E$ & \xmark   & $ {\rm Poly}\left(d, \nicefrac{1}{\e}\right)$ & $\max\left\{ \nicefrac{\e^{2}}{\sqrt{d}}, \nicefrac{\e}{d}\right\}$\tnote{{\color{blue}(2)}}~ ~\\ 
%%%%%%%      
    \hline
    { \scriptsize \textsc{ This work}}     &  \scriptsize{  saddle point}  &  $\E$~ and ~$\Prob$ & \xmark   & $\nicefrac{d}{\e^2}$ & $\nicefrac{\e^2}{\sqrt d}$\\    
    
       { \scriptsize \textsc{This work}}     &  \scriptsize{  saddle point}   & $\E$~ and ~$\Prob$ & \cmark  & $\nicefrac{d}{\e^2}$ & $\nicefrac{\e}{\sqrt d}$\tnote{{\color{blue}(3)}} \\    
      \hline
    \end{tabular} 
    
    %%%%%%%%%%%
\begin{tablenotes}
{\scriptsize
 \item[{\color{blue}(1)}] The results obtained for saddle point problems are also valid for convex optimization problems.
}\\
 {\scriptsize
 \item[{\color{blue}(2)}] Notice, that this bound (up to a logarithmic factor) is also an upper bound for maximum possible value of noise. It is  important to note, that $ \e/d\lesssim \e^2/\sqrt{d}$, when $\e^{-2}\lesssim d$. That is in the large-dimension regime, when subgradient method is better than center of gravity types methods \cite{nemirovskij1983problem}, the upper bound on the value of admissible noise (that allows one to solve the problem with accuracy $\e$) will be $\e^2/\sqrt{d}$. 
}

{\scriptsize
 \item[{\color{blue}(3)}] This estimate is for the Lipschitz constant of the noise and  it possibly is tight. However,  we prove that the upper bound (possibly not tight) for the Lipschitz-noise constant is $\e$ (see Appendix~\ref{app:upperbound} for details).
}
\end{tablenotes}    
\end{threeparttable}

\end{table}

% \paragraph{Contribution.} 


% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{-0.2em}
%     \item 
%     \item
%     \item
% \end{itemize}

 \vspace{-0.2cm}
\paragraph{Paper Organization.} This paper is organized as follows. In Section \ref{sec:prelim}, we begin with background material, notation, and assumptions.   In Section \ref{sec:mainthero}, we present  the main results of the paper: the algorithm and the analysis of its convergence. 
In Section \ref{sec:rest}, we consider  an additional assumption of $\gamma$-growth condition and restate the results.
%In Section \ref{sec:generalization}, we give some possible generalizations for our results. 
In Section \ref{sec:auxiliarylemmas}, we provide some of the key technical components used to prove the main results from Section \ref{sec:mainthero}.  

\section{Preliminaries: Notation, Setup and Assumptions}\label{sec:prelim}
In this section, we give some key notation, background material and assumptions.

\paragraph{Notation.} We use $\la x,y\ra \triangleq \sum_{i=1}^d x_i y_i$ to define the inner product of $x,y \in \R^d$, where $x_i$ is
  the $i$-th component of $x$. By  norm  $\|\cdot\|_p$ we mean  the $\ell_p$-norm. Then the dual norm of the norm $\|\cdot\|_p$ is $\|\lm\|_q \triangleq \max\{\la x,\lm \ra \mid \|x\|_p \leq 1 \} $. Operator $\E[\cdot]$  is the full  expectation and operator $\E_{\xi}[\cdot]$ is the conditional expectation, w.r.t. $\xi$.   
  
  
  
\paragraph{Setup.}
Let us introduce the embedding space $\Z \triangleq \X \times \Y$, and then  some $z\in \Z$ means $z \triangleq (x,y)$, where $x\in \X, y \in \Y$.
% Let us introduce the embedding space $\Z = \X \times \Y$ and introduce functions $f(z)$ and $f(z,\xi)$ by rewriting the objectives from Eq. \eqref{eq:min_max_problem} as follows
% \[
% f(z)\triangleq f(x,y) 
% \]
% where $z \triangleq (x,y) \in \Z$ and $x\in \X, y \in \Y$.
On this embedding space, we introduce  the $\ell_p$-norm
and  a prox-function $\omega(z)$ compatible with this norm. Then we define the  Bregman divergence associated with $\omega(z)$ as
\[V_z( v) \triangleq \omega(z) -\omega(v) - \la  \nabla \omega(v), z - v \ra \geq \|z-v\|_p^2/2, \quad \mbox{ for all } z,v \in Z.\] 
We also introduce a prox-operator as follows
\[ {\rm Prox}_z(\xi) \triangleq \arg\min_{v\in Z} \left(V_z(v) + \la \xi, v \ra\right), \quad \mbox{ for all } z \in Z.\]
Finally, we denote the $\omega$-diameter  of $\Z$ by 
$\D \triangleq \max\limits_{z,v\in \Z}\sqrt{2V_{z}(v)}= \widetilde{\O}\left(\max\limits_{z,v\in \Z}\|z-v\|_p\right)$. Here $\widetilde \O\left(\cdot\right)$ is $\O\left(\cdot\right)$ up to a $\sqrt{\log d}$-factor.




\begin{assumption}[Lischitz continuity of the objective]\label{ass:Lip_obj}
%  Function $f(x,y)$ is $M_x$-Lipschitz continuous w.r.t. $x\in \X$ and $M_y$-Lipschitz continuous w.r.t. $y\in \Y$, i.e., 
%  \begin{align*}
%      |f(x_1,\cdot)- f(x_2,\cdot)| &\leq M_x \|x_1- x_2\|_p, \quad \mbox{ for all } x_1,x_2\in \X,\\
%      |f(\cdot, y_1)- f(\cdot,y_2)| &\leq M_y \|y_1- y_2\|_p, \quad \mbox{ for all } y_1,y_2 \in \Y.
%  \end{align*}
 Function $f(z,\xi)$ is $M_2$-Lipschitz continuous in $z\in \Z$ w.r.t. the $\ell_2$-norm, i.e.,   for all  $z_1,z_2\in \Z$ and $\xi \in \Xi$, 
 \[|f(z_1, \xi)- f(z_2,\xi)| \leq M_2(\xi) \|z_1- z_2\|_2.\] 
 Moreover, there exists a positive constant $ M_2$ such that  $\E\left[M^2_2(\xi)\right] \leq M_2^2$.
%  \begin{align*}
%      |f(z_1)- f(z_2)| &\leq M_2 \|z_1- z_2\|_2, \quad \mbox{ for all } z_1,z_2\in \Z.
%  \end{align*}
\end{assumption}



\begin{assumption}\label{ass:err_noise}
For all  $z \in \Z$, it holds $|\delta(z)| \leq \Delta.$
\end{assumption}


\begin{assumption}[Lischitz continuity of the noise]\label{ass:Lip_noise}
Function $\delta(z)$ is $M_{2,\delta}$-Lipschitz continuous in $z\in \Z$ w.r.t. the $\ell_2$-norm, i.e., for all $z_1, z_2 \in \Z$, \[|\delta(z_1)- \delta(z_2)| \leq M_{2,\delta} \|z_1- z_2\|_2.\]
\end{assumption}





% The smoothing was introduced so that for a smoothed problem  it was possible to obtain an unbiased estimate of the subgradient.






\section{Main Results}\label{sec:mainthero}
In this section, we present one of the main results of the paper. For problem \eqref{eq:min_max_problem}, we present an
algorithm (see Algorithm \ref{alg:zoSPA}) that is optimal in terms of the number of inexact zeroth-order oracle calls and the maximum adversarial noise.  The algorithm  is based on a gradient-free version of the stochastic  mirror descent (SMD) \cite{ben2001lectures}. 

\paragraph{Black-box oracle.} We assume that we can query   zeroth-order oracle corrupted by an adversarial noise $\delta(z)$: 
\begin{equation}\label{eq:zerothorder}
    \vp(z,\xi) \triangleq f(z,\xi) + \delta(z).
\end{equation}
We will consider two cases:
\begin{enumerate}[leftmargin=*]
   \setlength\itemsep{-0.1em}
    \item Noise $\delta(z)$ is bounded (Assumption \ref{ass:err_noise})
    \item Noise $\delta(z)$ is Lipschitz (Assumption \ref{ass:Lip_noise})
\end{enumerate}
% Here $f(z,\xi)$ is the objective in the problem \eqref{eq:min_max_problem}.
% \paragraph{Zeroth-order oracle.}
% We assume that we can query biased zeroth-order oracle returning  \[\vp(z,\xi) \triangleq f(z,\xi) + \delta(z),\]
% where random variable $\xi$ is responsible for  unbiased stochastic noise and $\delta(z)$ is biased deterministic noise



\paragraph{Gradient approximation.}  The gradient of $\vp(z,\xi)$ from \eqref{eq:zerothorder}, w.r.t. $z$, can be approximated by the function evaluations in two random points closed to $z$. To do so, we define  vector $\be$ picked uniformly at random from the Euclidean unit sphere $\{\be:\|\be\|_2= 1\}$. Let $\be \triangleq (\be_x^\top, -\be_y^\top)^\top$, where ${\rm dim}(\be_x) \triangleq d_x$, ${\rm dim}(\be_y) \triangleq d_y$ and ${\rm dim}(\be) \triangleq d = d_x+d_y$. Then the gradient  of $ \vp(z,\xi)$ can be estimated by the following approximation with a  small variance \cite{shamir2017optimal}:
\begin{equation}\label{eq:grad_approx}
    g(z,\xi, \be) = \frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix},
\end{equation}
where $\tau$ is some constant. 
% In the one-dimensional ($d=1$), the estimate \eqref{eq:grad_approx} is trivial:
% when $\vp(z,\xi)$ is differentiable at $z$ and $\tau$  is sufficiently small, then the estimator \eqref{eq:grad_approx} approximates  the true gradient $\nabla \vp(z,\xi)$ well.





\paragraph{Randomized smoothing.}
For a non-smooth objective $f(z)$, we define the following function  
\begin{equation}\label{eq:smoothedfunc}
    f^\tau(z) \triangleq \E_{\tilde \be} f(z+\tau \tilde \be),
\end{equation}
where $\tau>0$ and $ \tilde\be$ is a vector picked uniformly at random from the Euclidean unit ball: $\{\tilde\be:\|\tilde\be\|_2\leq 1\}$. Function  $f^\tau(z)$ can be referred as a smooth approximation of $f(z)$. Here $f(z)\triangleq \E f(z,\xi)$. We notice that function $f^\tau(z)$ is introduced only for proof.\\

\noindent The next theorem presents the convergence rates for Algorithm \ref{alg:zoSPA} in terms of the expectation. For the convergence results in large deviation, we refer to the Appendix \ref{app:probab_converg}.

\begin{theorem}\label{th:conv_rate} 
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
% Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$.
%, where  $N$ is the number of iterations and $M^2 \triangleq  (M_2^2+M_{2,\delta}^2)$. 
Then  the following holds for\footnote{All the results obtained in this paper (except Section~\ref{sec:rest}) will have the same form for $\e_{\rm sad}  \triangleq \max_{y\in \Y}  f(\hat x^N, y) - \min_{x\in \X}   f(x, \hat y^N)$, but this required more accurate analysis, based on special trick from \cite{juditsky2011solving,beznosikov2020gradient}.} $\hat{\e}_{\rm sad}  \triangleq
% \max_{y\in \Y}  f(\hat x^N, y) - \min_{x\in \X}   f(x, \hat y^N)$ } $ \hat{\e}_{\rm sad}  \triangleq
f(\hat x^N, y_*) -  f(x_*, \hat y^N)$
% \max_{y\in \Y}  f(\hat x^N, y) - \min_{x\in \X}   f(x, \hat y^N)$,
where  $\hat z^N \triangleq (\hat x^N, \hat y^N)$ is the output of   Algorithm \ref{alg:zoSPA}:
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\D}{M_{\rm case1}}\sqrt{\frac{2 }{N}}$ with \\  $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + {d^2a_q^2\Delta^2}{\tau^{-2}}\right)$ 
 \begin{align}\label{eq:convergrate0}
      \E\left[ \hat{\e}_{\rm sad}\right]
     &\leq  M_{\rm case1}\D\sqrt{{2 }/{N}}
     + {\sqrt{d}\Delta \D}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\D}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\  $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate}
     \E\left[ \hat{\e}_{\rm sad}\right]
     \leq M_{\rm case2} \D   \sqrt{{2 }/{N}} + M_{2,\delta} \sqrt{d}  \D
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $\sqrt{\E\left[ \|\be\|_q^4\right]}= \O\left( \min\{q,\log d \} d^{2/q-1} \right)  =a_q^2$ \cite{gorbunov2019upper}. 
\end{theorem}

  \begin{wrapfigure}{L}{0.5\textwidth}
    \begin{minipage}{0.5\textwidth}
    \vspace{-0.7cm}
\begin{algorithm}[H]
 \caption{\textit{Zeroth-order} \textsc{SMD}}
\label{alg:zoSPA}
\KwData{ iteration number $N$}\\
$z^1  \leftarrow \arg\min_{z\in \Z} d(z)$
\For{$k=1,\dots, N$}{
  Sample $\be^k, \xi^k$ independently\\
  Initialize $\gamma_k$\\ 
 Calculate $g(z^k, \xi^k, \be^k)$ via \eqref{eq:grad_approx}\\
  $z^{k+1}  \leftarrow {\rm Prox}_{z^k}\left(\gamma_k g(z^k, \xi^k, \be^k)\right)$
  %\Comment*[r]{mirror descent step}
}
\KwResult{ $\hat z^N  \leftarrow \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^{N} \gamma_k z^k$}
\end{algorithm}
\vspace{-0.5cm}
    \end{minipage}
  \end{wrapfigure}

Algorithm \ref{alg:zoSPA} and its convergence analysis given in Theorem \ref{th:conv_rate} are based on the same proximal setups for spaces $\X$
and $\Y$. For the case,  when these setups are different we   replace the proximal step  $z^{k+1}  \leftarrow {\rm Prox}_{z^k}\left(\gamma_k g(z^k, \xi^k, \be^k)\right)$ on the  space $\Z\triangleq \X \times \Y$  by two proximal steps on spaces $\X$ and $\Y$. The convergence analysis in this case is given in  the Appendix  \ref{app:variablesep}.\\

\noindent
The next corollary presents our contribution. 
\begin{corollary}\label{cor:bound_noise}
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}, and 
let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement is true
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\E\left[\hat{\e}_{\rm sad}(\hat z^N)\right]\le\e$  after 
% \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\D^{-2}\e^2)^2 \right)\]
\[N =  \O\left( {da_q^2M_2^2\D^2}/{\e^{2}} \right)\]
iterations, where 
 $\sqrt{\E\left[ \|\be\|_q^4\right]}= \O\left( \min\{q,\log d \} d^{2/q-1} \right)  =a_q^2$ \cite{gorbunov2019upper}.  
% \begin{enumerate}
%     \item 
    % under Assumption \ref{ass:err_noise}
    % \[\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O \left( \frac{\e}{M_2} \right) \] 
  
    % \item under Assumption \ref{ass:Lip_noise}
    %   \[\delta(z) =\O\left( \frac{\e}{\D\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O\left( \frac{\e}{M_2} \right) \] 
%\end{enumerate}
% where $\e = \max\limits_{y\in \Y}  f(\hat x^N, y) - \min\limits_{x\in \X}   f(x, \hat y^N)$ and $(\hat x^N, \hat y^N,)$ are the outputs of the    Algorithm \ref{alg:zoSPA} after 
% \[N = \O\left( {M^2\D^2(1+ca_q^2d)^2}{\e^{-1}} \right)\]
% iterations.
\end{corollary}
Next we clarify the Corollary \ref{cor:bound_noise} in the two following special setups: the $\ell_2$-norm and the $\ell_1$-norm in the two following examples.
\begin{example}
Let $p=2$, then $q=2$ and  $\sqrt{\E \left[ \|\be\|_2^4\right]}   = 1$. Thus, $a_2^2=1$ and $\D^2 = \max\limits_{z,v\in \Z}\|z-v\|^2_2$. Consequently, the number of iterations in the Corollary \ref{cor:bound_noise} can be rewritten as follows
\[N =  \O\left( \frac{dM_2^2}{\e^{2}}\max\limits_{z,v\in \Z}\|z-v\|^2_2\right).\]
\end{example}
\begin{example}\citet[Lemma 4]{shamir2017optimal}
Let $p=1$ then, $q=\infty$ and $\sqrt{\E \left[ \|\be\|_\infty^4\right]}   = \O\left({\frac{\log d}{d}}\right)$. Thus, $a_\infty^2=\O\left({\frac{\log d}{d}}\right)$ and $\D^2 = \O\left(\log d \max\limits_{z,v\in \Z}\|z-v\|^2_1\right)$. Consequently, the number of iterations in the Corollary \ref{cor:bound_noise} can be rewritten as follows
\[N =  \O\left( \frac{M_2^2\log^2 d}{\e^{2}}\max\limits_{z,v\in \Z}\|z-v\|_1^2 \right).\]
\end{example}
% \begin{proof} 
%{\bf of the  Corollary \ref{cor:bound_noise}}
% The proof is based on equating Eq. \eqref{eq:convergrate0} 
% %and \eqref{eq:convergrate} 
% in Theorem \ref{th:conv_rate}  to $\e$. From that, the bounds for the number of iterations $N$, $\tau$ and $\Delta$ can be obtained. \\
% For instance, for $N$, we have
% \[N = \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})^2 \right) =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + da_q^2\D^{-2}\e^2)^2 \right).\]
% \end{proof}
% \noindent
% Under Assumption \ref{ass:Lip_noise}, the following corollary gives the maximum value for the Lipschitz constant of the adversarial noise  to sole the problem  \eqref{eq:min_max_problem} with accuracy $\e$ by Algorithm. \ref{alg:zoSPA}.


% \begin{corollary}\label{cor:Lip_noise}
% Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}, and let  Assumption \ref{ass:err_noise} hold. 
% Let \[M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O \left( \frac{\e}{M_2} \right). \] 
% Then for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}    after 
% % \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + c {d}a_q^2\D^{-2}\e^2)^2 \right)\]
% \[N =  \O\left( {da_q^2M_2^2\D^2}{\e^{-2}} \right)\]
% iterations, it holds $\E\left[\e_{\rm sad}(\hat z^N)\right]=\e$.  
% \end{corollary}

\begin{remark}
Corollary \ref{cor:bound_noise} bound for the Lipschitz constant given in the Corollary \ref{cor:bound_noise} is probably not the upper bound. In the Appendix \ref{app:upperbound}, we provide a natural analysis to prove  the bound from Corollary \ref{cor:bound_noise} being optimal but our arguments are based on the assumption that the points of the function evaluation were chosen regardless of the stochastic realizations $\xi_1,\xi_2,\xi_3,\dots$. Unfortunately, that is not the case of Algorithm \ref{alg:zoSPA} and many other practical algorithms.
\end{remark}

\begin{proof}[Proof of the  Theorem \ref{th:conv_rate}] 
By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align*}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) + \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2.   
\end{align*}
Taking the conditional  expectation w.r.t. $\xi, \be$ and summing for $k=1,\dots,N$  we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE}
 \sum_{k=1}^N \gamma_k  \E_{\be^k,\xi^k} \left[ \la g(z^k,\be^k,\xi^k), z^k-u\ra\right] 
   &\leq  V_{z^1}(u)  + \sum_{k=1}^N\frac{\gamma_k^2}{2} \E_{\be^k,\xi^k}\left[\|g(z^k,\be^k,\xi^k)\|_q^2 \right]. 
\end{align}
% where $\mathcal D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ is the diameter  of $\Z$. 

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE} we use Lemma \ref{lm:shamirEnabla} and obtain
 \begin{enumerate}[leftmargin=*]
     \item  under Assumption  \ref{ass:err_noise}:
     \begin{equation}\label{eq:inmainsqEtwo1}
        \E_{\be^k,\xi^k}\left[\|g(z^k,\xi^k,\be^k)\|^2_q\right] \leq c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}{\tau^{-2}}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise}: 
\begin{align}\label{eq:inmainsqEtwo}
    \E_{\be^k,\xi^k}\left[\|g(z^k,\xi^k,\be^k)\|^2_q\right] \leq c a^2_q d (M_2^2+M_{2,\delta}^2),
\end{align}
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E \left[ \|\be^k\|_q^4\right]} \leq a_q^2$.

{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE}, we use Lemma \ref{lm:expecapproxgrad}


 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz11}
     \sum_{k=1}^N \gamma_k \E_{\be^k,\xi^k}\left[\la g(z^k,\be^k,\xi^k), z^k-u\ra \right]
     &\geq  \sum_{k=1}^N \gamma_k \la \nabla f^\tau(z^k), z^k-u \ra  \notag \\ &+\sum_{k=1}^N \gamma_k  \E_{\be^k}\left[ \left|\la  {d\Delta}{\tau^{-1}}  \be^k, z^k-u  \ra \right|\right].
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz}
     \sum_{k=1}^N \gamma_k \E_{\be^k,\xi^k}\left[\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] 
     &\geq  \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \notag \\ 
     &+\sum_{k=1}^N \gamma_k \E_{\be^k}\left[ \left|\la  dM_{2,\delta} \be^k, z^k-u\ra\right| \right].
\end{align}
 \end{enumerate}
For the first term of the r.h.s. of Eq.\eqref{eq:eqrefeqffxyz11} and \eqref{eq:eqrefeqffxyz} we have 
\begin{align}\label{eq:eqexpfxy}
     \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra 
     &= \sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra \notag \\
     &=  \sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right) \notag \\
     &\geq  \sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y)) \notag \\
     &=  \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)),
\end{align}
where $u \triangleq (x^\top,y^\top)^\top$.
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq  f^\tau\left(\frac{\sum_{k=1}^N \gamma_k x^k}{\sum_{k=1}^{N}\gamma_k},y\right)  - f^\tau\left(x, \frac{\sum_{k=1}^N \gamma_k y^k}{\sum_{k=1}^{N}\gamma_k}\right)\notag \\
     &=  f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE}  for Eq. \eqref{eq:eqexpfxy} we get 
\begin{align}\label{eq:fpslff}
     \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra 
     &\geq \sum_{k=1}^{N}\gamma_k  f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) .
\end{align}
Next we estimate the term $\E_{\be^k} \left[    |\la \be^k, z^k-u\ra|  \right] $ in Eq. \eqref{eq:eqrefeqffxyz11} and \eqref{eq:eqrefeqffxyz},   by the Lemma  \ref{lm:dotprodvece} 
\begin{align}\label{eq:sectermErhs}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\|z^k-u\|_2}/{\sqrt{d}}. 
\end{align}
Now  we substitute  Eq. \eqref{eq:fpslff} and  \eqref{eq:sectermErhs} to Eq. \eqref{eq:eqrefeqffxyz11} and \eqref{eq:eqrefeqffxyz}, and get
 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz1122}
   \sum_{k=1}^N \gamma_k   \E_{\be^k,\xi^k}\left[ \la g(z^k,\be^k,\xi^k), z^k-u\ra \right] &\geq
     \sum_{k=1}^{N}\gamma_k  f^\tau\left( \hat x^N,y\right)- f^\tau\left(x, \hat y^N \right)  \notag \\
     &-  \sum_{k=1}^N \gamma_k {\sqrt{d}\Delta\|z^k-u\|_2}{\tau^{-1}}. 
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz22}
     \sum_{k=1}^N \gamma_k  \E_{\be^k,\xi^k}\left[\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] 
     &\geq  \sum_{k=1}^{N}\gamma_k  f^\tau\left( \hat x^N,y\right) - f^\tau\left(x, \hat y^N \right)  \notag \\
     &- \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta}\|z^k-u\|_2. 
\end{align}
 \end{enumerate}
 
{\bf Step 3.} (under Assumption \ref{ass:err_noise}) \\
Now we combine Eq. \eqref{eq:eqrefeqffxyz1122}   with  Eq. \eqref{eq:inmainsqEtwo1} for Eq. \eqref{eq:inmainsqE} and obtain under Assumption \ref{ass:err_noise} the following
     \begin{align}\label{eq:inmainsqEtwo133}
     \sum_{k=1}^{N}\gamma_k f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) 
     &-  \sum_{k=1}^N \gamma_k {\sqrt{d} \Delta \|z^k-u\|_2}{\tau^{-1}}  \leq  V_{z^1}(u) \notag \\
     &+  \sum_{k=1}^N \frac{\gamma_k^2}{2} \left(c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}{\tau^{-2}}\right).
     \end{align}
Using Lemma \ref{lm:shamirSmoothFun} we obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this we can rewrite \eqref{eq:inmainsqEtwo133} as follows
 \begin{align}\label{eq:exEeqE1}
       f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right) 
      &\leq 
     \frac{ V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q dM_2^2+ d^2 a_q^2\Delta^2\tau^{-2}}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  \notag \\
      &+{ \sqrt{d} \Delta \max_{k}\|z^k-u\|_2}{\tau^{-1}} +  2\tau M_2.
 \end{align}
  For the r.h.s. of \eqref{eq:exEeqE1}  we use the definition of  the $\omega$-diameter  of $\Z$:\\
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$.
 Using this for  \eqref{eq:exEeqE1} and   taking $(x,y) = (x_*,y_*)$,
%  the maximum in $(x,y) \in (\X,\Y)$,
 we obtain
 \begin{align}\label{eq:dghjsklslsl1}
    % \max_{y \in \Y} 
    f\left( \hat x^N,y_*\right) -  
    % \min_{x\in \X} 
    f\left(x_*, \hat y^N \right)
     &\leq \frac{ \D^2+ (c a^2_q d M_2^2 +
     d^2 a_q^2\Delta^2\tau^{-2})
    \sum_{k=1}^{N} {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
       \notag \\
    &+ {\sqrt{d}\Delta \D}{\tau^{-1}}
     +  2\tau M_2.  
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Then we use the definition of  the $\omega$-diameter  of $\Z$:
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$. Thus, taking the expectation of \eqref{eq:dghjsklslsl1} and choosing  learning rate $\gamma_k 
=\frac{\D}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl1} we get
 \begin{align*}
      \E\left[ 
    %   \max_{y \in \Y}
      f\left( \hat x^N,y_*\right) -  
    %   \min_{x\in \X} 
      f\left(x_*, \hat y^N \right)\right]
     &\leq  
     %\frac{\D(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     M_{\rm case1}\D\sqrt{{2}/{N}}
     + \frac{\Delta\D\sqrt{d}}{\tau} 
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 4.} (under Assumption \ref{ass:Lip_noise})\\
Now we combine Eq.  \eqref{eq:eqrefeqffxyz22}  with  Eq.  \eqref{eq:inmainsqEtwo} for Eq. \eqref{eq:inmainsqE} and obtain under Assumption \ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo334}
    \sum_{k=1}^{N}\gamma_k f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) 
    &- \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta}\|z^k-u\|_2 \leq V_{z^1}(u)\notag \\
    &+  \sum_{k=1}^N \frac{\gamma_k^2}{2} c a^2_q d (M_2^2+M_{2,\delta}^2).
\end{align}
Using Lemma \ref{lm:shamirSmoothFun} we obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this we  can rewrite \eqref{eq:inmainsqEtwo334} as follows
 \begin{align}\label{eq:exEeqE}
      f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  
      &\leq 
     \frac{ V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q d (M_2^2+M_{2,\delta}^2)}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2} \notag\\
      &+ \sqrt{d}M_{2,\delta} \max_{k} \|z^k-u\|_2  +  2\tau M_2. 
 \end{align}
   For the r.h.s. of \eqref{eq:exEeqE}  we use the definition of  the $\omega$-diameter  of $\Z$: \\
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$.
 Using this for  \eqref{eq:exEeqE} and   taking $(x,y) = (x_*,y_*)$,
%  the maximum in $(x,y) \in (\X,\Y)$, 
 we obtain
 \begin{align}\label{eq:dghjsklslsl}
    %   \max_{y \in \Y} 
      f\left( \hat x^N,y_*\right) -  
    %   \min_{x\in \X}
      f\left(x_*, \hat y^N \right)
     &\leq \frac{ \D^2+ c a^2_q d (M_2^2 +M_{2,\delta}^2)\sum_{k=1}^N {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
    \notag\\
     &+ M_{2,\delta}  \sqrt{d}\D
     +  2\tau M_2.  
 \end{align}
 Then we use the definition of  the $\omega$-diameter  of $\Z$:
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$. Thus, taking the expectation of \eqref{eq:dghjsklslsl1} and choosing  learning rate  $\gamma_k 
=\frac{\D}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl} we get
%   $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$  in Eq. \eqref{eq:dghjsklslsl} we obtain
%  \begin{align*}
%       \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
%      &\leq  \frac{\D(1+c a^2_q d M_2^2 + c a^2_q dM_{2,\delta}^2)}{\sqrt{2N}M}  + M_{2,\delta} \D \sqrt{d} 
%      +  2\tau M_2.  
%  \end{align*}
 \begin{align*}
      \E\left[ 
    %   \max_{y \in \Y} 
      f\left( \hat x^N,y_*\right) -  
    %   \min_{x\in \X} 
      f\left(x_*, \hat y^N \right)\right]
     &\leq  M_{\rm case2}\D\sqrt{{2}/{N}}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.  
 \end{align*}
\end{proof}

==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/intuition.tex <==
\section{Intuition of Smoothing}\label{sec:intuition}
In this section, we provide a motivation for smoothing a non-smooth function according to \eqref{eq:smoothedfunc}. 



Subgradients of a non-smooth function cannot be estimated by the  gradient-free approximation \eqref{eq:grad_approx}. 
 Indeed, let us consider the following example.
 



 




\begin{example}
Let us consider the one-dimensional ($d=1$) deterministic function $f(x)$ from Figure \ref{fig:non_smooth_funct}  with zeros noise ($\delta=0$) for simplicity.  Then, gradient-free approximation \eqref{eq:grad_approx} can be simplified as 
\begin{equation}\label{eq:simpgrad}
    g(x) = \frac{1}{2\tau}(f(x+\tau) - f(x-\tau)).
\end{equation}
Let us consider non-smooth function  $f(x) = |x|$.
For point $x>0$ taken close to $0$ we have
 \[g(x) = \frac{x}{\tau}, \]
 when $x \in [-\tau,\tau]$.
 However, for all $x>0$, $\nabla f(x)=1$. 
\end{example}




  \begin{figure}[h]
    \centering
   \includegraphics[width=0.5\linewidth]{approx2.png}
 \caption{Smooth approximation $f^{\tau}(x)$ of a non-smooth function $f(x)$}
 \label{fig:non_smooth_funct}
\end{figure}

\subsection{Differentiation of smooth approximation}
For simplicity, let us proof  Lemma \ref{lm:flax} in the 
one dimensional case $(d=1)$ 
    \[  f^\tau(x) \triangleq \E_{\tilde e} f(x+\tau \tilde e) = \frac{1}{2}\int_{-1}^1 f(x+\tau \tilde e)d \tilde e, \]
    where $\tilde e$ is a random vector from segment $[-1,1]$.\\
   We get for the derivative of $f$
    \[ \left( f^\tau(x)\right)_x' =  \frac{1}{2}\int_{-1}^1 f'_x(x+\tau \tilde e)d \tilde e. \]
    With the change of variable $y = x+\tau \tilde e$ we obtain
    \[
    \left( f^\tau(x)\right)_x' =  \frac{1}{2\tau}\int_{x-\tau}^{x+\tau} f'_y(y)dy = \frac{d}{2\tau} (f(x+\tau)-f(x-\tau))  = \E_{{e}}\left[\frac{d}{\tau}f(x+\tau {e})e\right],
    \]
    where $e$ is a random vector equal to 1 or -1 with probability $\nicefrac{1}{2}$.
 

% Smooth approximation
% a smooth approximation of a non-smooth function $f$ is
% \begin{equation*}
%     f^\tau(x) \triangleq \E_{\tilde \be} f(x+\tau \tilde \be),
% \end{equation*}
% where $\tau>0$ and $ \tilde\be$ is a random vector from the Euclidean unit ball.

% Whereas \[\E_{{\be}}\left[g(x,\be)\right] \neq \partial f(x).\]
%  Function  $f^\tau(x)$ is differentiable with the following gradient
% \[
% \nabla  f^\tau(x) = \E_{{\be}}\left[ \frac{d}{2\tau} (f(x+\tau {\be})-f(x-\tau {\be}))\be \right] = \E_{{\be}}\left[g(x,\be)\right],
% \]
% where $\be$ is a random vector from the Euclidean unit sphere.\\


% Main Idea: replace the original problem by
% \[
% \min_{x\in\X}f^\tau(x).
% \]




==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/lemmas.tex <==
\section{Auxiliary Results for Theorem \ref{th:conv_rate}}\label{sec:auxiliarylemmas}


This section presents auxiliary results to prove Theorem \ref{th:conv_rate} from Section \ref{sec:mainthero}.


\begin{lemma}\label{lm:dotprodvece}
Let vector $\be$ be a random unit vector from the Euclidean unit sphere $\{\be:\|\be\|_2=1\}$. Then it holds for all $r \in \R^d$
 \begin{equation*}
     \E_{ \be}\left[ \left|\la \be, r \ra \right| \right] \leq {\|r\|_2}/{\sqrt{d}}.
 \end{equation*}
\end{lemma}


\begin{lemma}\label{lm:shamirSmoothFun}
Let $f(z)$ be $M_2$-Lipschitz continuous function. Then for $f^\tau(z)$ from \eqref{eq:smoothedfunc}, it holds
\[
\sup_{z\in \Z}|f^\tau(z) - f(z)|\leq \tau M_2.
\]
\end{lemma}

\begin{proof}
By the definition of $f^\tau(z)$ from \eqref{eq:smoothedfunc} and Assumption \ref{ass:Lip_obj} we have
\begin{align*}
    |f^\tau(z) - f(z)|
    &= \left|\E_{\be}\left[f(z+\tau\be)\right]  -f(z)\right| = \E_{\be}\left[|f(z+\tau\be) - f(z)| \right] \leq \E\left[ M_2 \|\tau \be\|_2\right] =  M_2 \tau.  
\end{align*}
\end{proof}

\begin{lemma}\label{lm:flax}
 Function  $f^\tau(z)$ is differentiable with the following gradient
\[
\nabla  f^\tau(z) = \E_{{\be}}\left[ \frac{d}{\tau} f(z+\tau {\be})\be \right].
\]
\end{lemma}


\begin{lemma}\label{lm:expecapproxgrad}
   For $g(z,\xi,\be)$ from \eqref{eq:grad_approx} and $f^\tau(z)$ from \eqref{eq:smoothedfunc}, the following holds 
 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \[\E_{\xi, \be}\left[\la g(z,\xi,\be),r\ra\right] \geq \la \nabla f^\tau(z),r\ra  - {d\Delta}{\tau^{-1}} \E_{\be} \left[\left|\la \be, r \ra \right|\right],\]
     \item  under Assumption \ref{ass:Lip_noise}   \[\E_{\xi, \be}\left[\la g(z,\xi,\be),r\ra\right] \geq \la \nabla f^\tau(z),r\ra   - d M_{2,\delta} \E_{\be} \left[\left|\la  \be, r \ra \right|\right],\]
 \end{enumerate}
 \end{lemma}


\begin{proof} Let us consider
\begin{align*}
  \hspace{-0.3cm} g(z,\be,\xi) 
    &= \frac{d}{2\tau}   \left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be \notag \\
    &=\frac{d}{2\tau}  \left(f(z+\tau \be,\xi) +\delta(z+\tau \be) - f(z-\tau \be,\xi) - \delta(z-\tau \be) \right) \be\notag \\
   &=\frac{d}{2\tau} \left(\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi) \right) \be +     (\delta(z+\tau \be) - \delta(z-\tau \be)) \be\right).
\end{align*}
Using this we have the following \begin{align}\label{eq:sqprod}
    \E_{\xi, \be}\left[\la g(z,\xi,\be),r\ra\right]   &=\frac{d}{2\tau}  \E_{\xi, \be}\left[\la\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi) \right) \be, r \ra \right]\notag \\
    &+\frac{d}{2\tau}  \E_{ \be}\left[     \la (\delta(z+\tau \be) - \delta(z-\tau \be)) \be, r\ra\right].
\end{align}
Taking the expectation, w.r.t. $\be$, from  the first term of the r.h.s. of \eqref{eq:sqprod} and  using the symmetry of the distribution of $\be$, we have
 \begin{align}\label{eq:nablaeqfunc}
      \frac{d}{2\tau}\E_{\xi, \be} \left[  \left(\la f(z+\tau \be,\xi)  - f(z-\tau \be,\xi) \right) \be, r\ra \right] 
        &= \frac{d}{2\tau}\E_{\xi, \be}  \left[ \la f(z+\tau \be,\xi)\be, r\ra \right] +\frac{d}{2\tau}\E_{\xi, \be}  \left[  \la f(z-\tau \be,\xi)\be, r\ra \right]   \notag\\
         &= \frac{d}{\tau}\E_{\be} \left[ \la\E_{\xi} \left[ f(z+\tau \be,\xi)\right] \be, r\ra\right] = \frac{d}{\tau}\E_{\be} \left[ \la  f(z+\tau \be) \be, r\ra\right] \notag\\
         &=\la \nabla f^\tau(z),r\ra. \quad /*  \mbox{Lemma \ref{lm:flax}}  */ 
\end{align}
\begin{enumerate}[leftmargin=*]
    \item For the second term of the r.h.s. of \eqref{eq:sqprod} under the Assumption \ref{ass:err_noise} we obtain 
    \begin{align}\label{eq:secondtermlipschnass2}
    \frac{d}{2\tau}  \E_{ \be} \left[  \la(\delta(z+\tau \be) - \delta(z-\tau  \be)) \be, r\ra \right] \geq - \frac{d}{2\tau} 2\Delta \E_{\be} \left[ \left|\la \be, r \ra \right|\right] = -\frac{d\Delta}{\tau} \E_{\be} \left[ \left|\la \be, r \ra \right| \right].
\end{align}
    \item For the second term of the r.h.s. of \eqref{eq:sqprod} under the Assumption \ref{ass:Lip_noise} we obtain  
\begin{align}\label{eq:secondtermlipschn}
    \frac{d}{2\tau}  \E_{\be} \left[ \la (\delta(z+\tau \be) - \delta(z-\tau \be)) \be, r\ra\right] \geq - \frac{d}{2\tau} M_{2,\delta} 2\tau \E_{\be} \left[ \|\be\|_2 \left|\la\be, r\ra \right|\right] = -d M_{2,\delta}  \E_{\be} \left[ \left|\la\be, r\ra\right|\right].
\end{align}
\end{enumerate}


Using Eq. \eqref{eq:nablaeqfunc} and \eqref{eq:secondtermlipschnass2} (or Eq. \eqref{eq:secondtermlipschn}) for Eq. \eqref{eq:sqprod} we get the statement of the lemma.
% \begin{align}
%   \E\left[ g(z,\be,\xi)\right]  \geq  \nabla f^\tau (z)  - d M_{2,\delta} \E_{\be} \left[ \be\right]
% \end{align}

\end{proof}








\begin{lemma}\citet[Lemma 9]{shamir2017optimal}\label{lm:shamirLm9}
For any function $f(\be)$ which is $M$-Lipschitz w.r.t. the $\ell_2$-norm, it holds that if $\be$ is uniformly distributed on the Euclidean unit sphere, then
\[
\sqrt{\E\left[(f(\be) - \E f(\be))^4 \right]} \leq cM_2^2/d
\]
for some numerical constant $c$.
\end{lemma}






\begin{lemma}\label{lm:shamirEnabla}
 For $g(z,\xi,\be)$ from \eqref{eq:grad_approx}, the following holds
%  and $f^\tau(z)$ from \eqref{eq:smoothedfunc}, it holds that   $\E\left[g(z,\xi,\be)\right] = \nabla f^\tau(z)$. Moreover,  
 under Assumption \ref{ass:Lip_obj} 
 \begin{enumerate}
     \item  and Assumption  \ref{ass:err_noise}
     \[\E_{\xi,\be}\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}/{\tau^2},\]
     \item  and Assumption \ref{ass:Lip_noise} 
\[\E_{\xi,\be}\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q d (M_2^2+M_{2,\delta}^2),\] 
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E \left[ \|\be\|_q^4\right]} \leq a_q^2$.
\end{lemma}


% \begin{align}
%   \E\left[g(z,\xi,\be)\right] &= \E\left[ \frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be \right] \notag \\
%       &= \frac{d}{2\tau}\E \left[  \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right) \be \right] \notag\\
%         &= \frac{d}{2\tau}\E \left[ f(z+\tau \be,\xi)\be \right] + \frac{d}{2\tau}\E \left[\delta(z+\tau\be)\be \right]\notag \\
%         &+\frac{d}{2\tau}\E \left[  f(z-\tau \be,\xi)(-\be) \right]  +\frac{d}{2\tau}\E \left[\delta(z-\tau\be) (-\be) \right] \notag\\
%          &= \frac{d}{\tau}\E \left[ f(z+\tau \be,\xi)\be\right] + \frac{d}{\tau}\E \left[\delta(z+\tau\be)\be \right], \qquad /*\mbox{ the  distribution of $\be$ is symmetric } */  \notag\\
%          &=\nabla f^\tau (z)  + \frac{d}{\tau}\E \left[\delta(z+\tau\be)\be \right]. \qquad /* ~ \mbox{ Lemma \ref{lm:flax} } ~ */ 
% \end{align}

\begin{proof} Let us consider
\begin{align}\label{eq:sqnormE}
    &\E_{\xi,\be} \left[\|g(z,\xi,\be)\|^2_q \right] = \E_{\xi,\be}\left[ \left\|\frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be\right\|^2_q \right] \notag \\
    &= \frac{d^2}{4\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right)^2 \right] \notag\\
     &\leq \frac{d^2}{2\tau^2}\left(\E_{\xi,\be} \left[\|\be\|_q^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right] + \E_{\be} \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \right).
\end{align}
For the first term in the r.h.s. of Eq. \eqref{eq:sqnormE}, the following holds with an arbitrary parameter $\alpha$
\begin{align}\label{eq:fgkbbhgdddgh}
 & \frac{d^2}{2\tau^2}\E_{\xi,\be} \left[\|\be\|_q^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right]  \notag\\
  &= \frac{d^2}{2\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 \left((f(z+\tau \be,\xi) -\alpha) -(f(z-\tau \be,\xi) - \alpha)   \right)^2 \right] \notag\\
    &\leq \frac{d^2}{\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 + (f(z-\tau \be,\xi) -\alpha)^2 \right] \qquad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
     &=  \frac{d^2}{\tau^2}\left(\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] + \E_{\xi,\be} \left[\|\be\|_q^2(f(z-\tau \be,\xi) -\alpha)^2 \right] \right) \notag\\
    &= \frac{2d^2}{\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
\end{align}
Applying the Cauchy--Schwartz inequality for Eq. \eqref{eq:fgkbbhgdddgh} and using $\sqrt{\E \left[ \|\be\|_q^4\right]} \leq a_q^2$ we obtain 
\begin{align}\label{eq:funcsq}
     \frac{d^2}{\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] 
     &\leq \frac{d^2}{\tau^2} \E_{\xi} \left[\sqrt{\E \left[ \|\be\|_q^4\right]} \sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]} \right]\notag\\
     &\leq \frac{d^2 a_q^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right] . 
\end{align}
Then we assume $\alpha = \E_{\be}\left[f(z+\tau \be,\xi)\right]$
% , $\beta = \E\left[\delta(z+\tau \be)\right]$ 
and use Lemma \ref{lm:shamirLm9} along with the fact that $f(z+\tau\be,\xi)$ is $\tau M_2(\xi)$-Lipschitz, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus for Eq. \eqref{eq:funcsq}, it holds  
\begin{align}\label{eq:finlhkjfsvn}
    \frac{d^2 a_q^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right]
    &\leq \frac{d^2 a_q^2}{\tau^2} \cdot c\frac{\tau^2 \E M_2^2(\xi)}{d} = c d a_q^2 M_2^2.  
    %\red{\text{it seems should be} \leq}
\end{align}
\begin{enumerate}[leftmargin=*]
    \item Under the Assumption \ref{ass:err_noise}
     for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE}, the following holds
    \begin{align}\label{eq:fgkssssffdgh}
        &\frac{d^2}{4\tau^2}\E_{\be} \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \leq  \frac{d^2\Delta^2}{\tau^2} \E \left[ \|\be\|_q^2  \right]\leq \frac{d^2 a_q^2\Delta^2}{\tau^2}.
    \end{align}
   % where we used $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$.
    \item Under the Assumption \ref{ass:Lip_noise}
    for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE}, the following holds with an arbitrary parameter $\beta$
    \begin{align}\label{eq:fgklljgsdgh}
        &\frac{d^2}{4\tau^2}\E_{\be} \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \notag \\
     &= \frac{d^2}{2\tau^2}\E \left[ \|\be\|_q^2 \left((\delta(z+\tau\be) -\beta) -(\delta(z-\tau\be)  -\beta) \right)^2 \right] \notag\\
    &\leq \frac{d^2}{\tau^2}\E \left[ \|\be\|_q^2 \left((\delta(z+\tau\be)-\beta)^2  +(\delta(z-\tau\be) -\beta)^2 \right) \right] \quad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
    &= \frac{d^2}{2\tau^2}\left(\E \left[ \|\be\|_q^2 (\delta(z+\tau \be)-\beta)^2 \right] + \E \left[\|\be\|_q^2(\delta(z-\tau \be) -\beta)^2 \right] \right) \notag\\
    &= \frac{d^2}{\tau^2}\E \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
    \end{align}
\end{enumerate}
and for the second term in the Eq. \eqref{eq:sqnormE}, we get
\begin{align}\label{eq:noisesq}
   \frac{d^2}{\tau^2}\E_{\be}\left[ \|\be\|_q^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]
   &\leq \frac{d^2}{\tau^2}\sqrt{\E \left[ \|\be\|_q^4\right]} \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \notag \\
   &\leq \frac{d^2 a_q^2}{\tau^2} \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] }
\end{align}
Then we assume  $\beta = \E_{\be}\left[\delta(z+\tau \be)\right]$ and use Lemma \ref{lm:shamirLm9} together with the fact that $\delta(z+\tau\be)$ is $\tau M_{2,\delta}$-Lipschitz continuous, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus, Eq. \eqref{eq:noisesq} can be rewritten as 
\begin{align}\label{eq:fkssoomnbd}
    \frac{d^2 a_q^2}{\tau^2}  \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } 
    &\leq \frac{d^2 a_q^2}{\tau^2}  \cdot c\frac{\tau^2  M_{2,\delta}^2}{d} \leq c a^2_q d M_{2,\delta}^2. 
    %\red{\text{it seems should be} \leq}
\end{align}
Using Eq. \eqref{eq:finlhkjfsvn} and \eqref{eq:fgkssssffdgh} (or Eq. \eqref{eq:fkssoomnbd}) for Eq. \eqref{eq:sqnormE}, we get the statement of the theorem.
% \begin{align*}
%     \left[\|g(z,\xi,\be)\|^2_q \right] 
%     &\leq \frac{d^2 a_q^2}{\tau^2} \cdot c\frac{\tau^2 \E M_2^2(\xi)}{d} + \frac{d^2 a_q^2}{\tau^2}  \cdot c\frac{\tau^2 \E M_{2,\delta}^2(\xi)}{d} \leq c a^2_q d (M_2^2+M_{2,\delta}^2). 
%     %\red{\text{it seems should be} \leq}
% \end{align*}
\end{proof}

==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/noise.tex <==
\section{Infinite Noise Variance}
When the second moment of the  stochastic gradient  $\nabla f(z,\xi)$ is unbounded the rate of convergence may changes dramatically, see the next section. For such a case, we consider a more general inequality for  Assumptions~\ref{ass:Lip_obj}.  We suppose  that there exists a positive constant $\tilde{M_2}$ such that for   $M_2(\xi)$  Assumptions~\ref{ass:Lip_obj} the following holds 
\begin{equation*}
    \E \left[M_2(\xi)^{1+\kappa}\right]\le \tilde{M}_2^{1+\kappa},
\end{equation*}
where $\kappa \in \left(0,1\right]$. From  \citet[Lemmas 9 -- 11]{shamir2017optimal} the following can be obtained 
 \begin{enumerate}[leftmargin=*]
     \item  under Assumption  \ref{ass:err_noise}:
     \begin{equation}\label{eq:inmainsqEtwo1}
        \E\left[\|g(z,\xi,\be)\|^{1+\kappa}_q\right] \leq \tilde{c} a^2_q d^{(1+\kappa)/2}\tilde{M}_2^{1+\kappa} + 2^{1+\kappa}{d^{1+\kappa} a_q^2\Delta^2}{\tau^{-2}}=\tilde{M}_{case1}^{1+\kappa}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise}: 
\begin{align}\label{eq:inmainsqEtwo2}
    \E\left[\|g(z,\xi,\be)\|^{1+\kappa}_q\right] \leq \tilde{c} a^2_q d^{(1+\kappa)/2} (\tilde{M}_2^{1+\kappa}+M_{2,\delta}^{1+\kappa}) = \tilde{M}_{case2}^{1+\kappa},
\end{align}
 \end{enumerate}
 where    $\tilde{c}$ is some numerical constant and
 $\sqrt{\E_{\be} \left[ \|\be\|_q^{2+2\kappa}\right]} \leq \tilde{a}_q^2$. As a particular case: $\tilde{a}_{2}^2 = 1$, $\tilde{a}_{\infty}^2 = \O\left({\frac{\log^{(1+\kappa)/2} d}{d^{(1+\kappa)/2}}}\right)$. \\
Let us assume that $q \in \left[1+\kappa,\infty\right)$, $1/p + 1/q = 1$ and prox-function determined by
\[\omega(x) = K_q^{1/\kappa} \frac{\kappa}{1+\kappa}\|x\|_p^{\frac{1+\kappa}{\kappa}} \mbox{ with } K_q = 10\max\left\{1,(q-1)^{(1+\kappa)/2}\right\}.  \]
Based on \cite{vural2022mirror} one can prove the first part of Theorem~\ref{th:conv_rate_restarts} with $M_2$ replaced by $\tilde{M_2}$, stepsize is chosen as
\[\gamma_k = \frac{\left((1+\kappa)V_{z^1}(z^{\star})/\kappa\right)^{\frac{1}{1+\kappa}}}{\tilde{M}_{case}}N^{-\frac{1}{1+\kappa}}\]
and the first terms in the r.h.s. of \eqref{eq:convergrate0_restarts}, \eqref{eq:convergrate_restarts} is determined as follows 
\[\tilde{M}_{case}\left(\frac{1+\kappa}{\kappa}V_{z^1}(z^{\star})\right)^{\frac{\kappa}{1+\kappa}} N^{-\frac{\kappa}{1+\kappa}}.\]
These results can be further generalized to $r-$growth condition for duality gap ($r\ge 2$), see Assumption~\ref{ass:strongly_convex}.


==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/probability_convergence.tex <==
\section{High-probability bound}
\label{H-PB}
\begin{assumption}[Uniformly Lischitz continuity of the objective]\label{ass:uni_Lip_obj}
 Function $f(z,\xi)$ is uniformly $M_2$-Lipschitz continuous in $z\in \Z$ w.r.t. the $\ell_2$-norm, i.e.,   for all  $z_1,z_2\in \Z$ and $\xi \in \Xi$, 
 \[|f(z_1, \xi)- f(z_2,\xi)| \leq M_2 \|z_1- z_2\|_2.\] 
\end{assumption}



Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
% Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$.
%, where  $N$ is the number of iterations and $M^2 \triangleq  (M_2^2+M_{2,\delta}^2)$. 
\begin{theorem}\label{th:conv_rate_prob}
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:uni_Lip_obj}. Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
=\frac{\D}{M}\sqrt{\frac{2}{N}}$, where  $N$ is the number of iterations and $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$. Then for the output $  (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, under Assumption \ref{ass:err_noise} for some constant $c$ the following holds
% \begin{align}
%       \text{Prob} & \left\{ \e_{\rm sad} (\hat z^N)  \geq \frac{4 \Omega^2 \sqrt{d} \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2 d^2}{M}   + \right. \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 d^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
%       & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} 
% \end{align}

\begin{align}
       &\text{Prob}  \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{ \sqrt{V_{z^1}(u)} M  }{\sqrt{N}}  +  \Omega \frac{2 \sqrt{2} M \sqrt{V_{z^1}(u)}}{c N} +\right. \nonumber\\
      & \left.  + 2 \tau M_2 + \frac{ \Omega \D \sqrt{d} \Delta }{\tau }    \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} \label{eq:convergrate_prob}.
\end{align}

where 
$ \e_{\rm sad}  \triangleq \max\limits_{y\in \Y}  f(\hat x^N, y) - \min\limits_{x\in \X}   f(x, \hat y^N)$.
%is the `saddle point residual'.
\end{theorem}


















\begin{proof}[Proof of the  Theorem \ref{th:conv_rate_prob}]
By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) + \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_2^2/2   \notag
\end{align}
Summing for $k=1,\dots,N$ we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE_prob}
   \sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra 
   &\leq V_{z^1}(u)  + \sum_{k=1}^N\gamma_k^2\|g(z^k,\be^k,\xi^k)\|_2^2/2  \notag\\
   &\leq  V_{z^1}(u) + \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_2^2, 
\end{align}
For the next steps we provide the new definition of gradient approximation of $\nabla f(z, \xi)$ following the Eq. $\eqref{eq:grad_approx}$:
\begin{equation}\label{eq:grad_approx_f}
    g_f(z,\xi, \be) = \frac{d}{2\tau}\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix},
\end{equation}
{\bf Step 1.}\\
In this step we will estimate the second term in the r.h.s of inequality \eqref{eq:inmainsqE_prob}. We can rewrite this term in the form :
\begin{align}\label{eq:prob_var}
    & \|g(z^k,\be^k,\xi^k)\|_2^2  = \frac{d^2}{4\tau^2}  \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right)^2 \leq \notag\\
     &\hspace{4cm}\leq 2 \|g_f(z^k,\be^k,\xi^k)\|_2^2 + \frac{d^2}{2\tau^2} \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2  
\end{align}
\begin{enumerate}
\item To estimate the first term in the r.h.s of Eq. \eqref{eq:prob_var} we invoke the Assumtion \ref{ass:uni_Lip_obj} and the Eq.\eqref{eq:grad_approx_f}. We observe that the function $g_f(z^k,\be^k,\xi^k)$ is uniformly $M_2 d$-Lipschitz continious and $\E_{\be^k} g_f(z^k,\be^k,\xi^k) = 0$. Thus we can use Lemma 9 from  \cite{shamir2017optimal} and obtain for some constant $c$: 
\begin{align}\label{eq:estim_of_g_f}
    \text{Prob} \left\{ \| g_f(z^k,\be^k,\xi^k) \|_2 > t  \right\} \leq \exp \left\{ - \frac{c t^2}{M_2^2 d} \right\} 
\end{align}
Invoking the last inequality and  Assumtion \ref{ass:uni_Lip_obj}, the random variables \\
$\phi_k = \gamma_k^2 \|g_f(z^k,\be^k,\xi^k)\|_2^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$ satisfy the premise of case B of Lemma 2 from \cite{lan2012validation} with $\sigma_k = \frac{2 d M_2^2}{c} \gamma_k^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$:
\begin{align*}
     \E_{|t-1} \left[ \exp \{|\phi_k|/\sigma_k\} \right] & = \E_{|t-1} \left[ \exp \{ \|g_f(z^k,\be^k,\xi^k)\|_2^2/4  M_2^2 d\} \right] = \\
     &= \int_0^{\infty} \text{Prob} \left\{ \exp \{ \|g_f(z^k,\be^k,\xi^k)\|_2^2/4  M_2^2 d\} \geq \tilde{t}  \right\} d \tilde{t} \leq \int_0^{1} 1 d \tilde{t} +\\
     & + \int_1^{\infty} \underbrace{\text{Prob} \left\{ \exp \{ \|g_f(z^k,\be^k,\xi^k)\|_2^2/4  M_2^2 d\} \geq \tilde{t}  \right\}}_{\text{by } \eqref{eq:estim_of_g_f} : \text{ }\leq \exp \left\{ - \frac{c \sigma_k^2  \ln \tilde{t}}{M_2^2 d} \right\} \leq \left(\frac{1}{\tilde{t}} \right)^{\frac{c \sigma_k^2}{d M_2^2}} = \left(\frac{1}{\tilde{t}} \right)^{2}} d \tilde{t} \leq 1 + 1 \leq  \exp \{1\}
\end{align*}

Invoking case B of Lemma 2 from \cite{lan2012validation}, we get
\small{
\begin{align}
    &\text{Prob} \left\{ \left| \sum_{k=1}^N \gamma_k^2 \|g_f(z^k,\be^k,\xi^k)\|_2^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1} \right| > \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c  \sum_{k=1}^N \gamma_k } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c  \sum_{k=1}^N \gamma_k } \right\} \nonumber \\
    & \hspace{8 cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} \label{eq:first_step_var}
\end{align}}
\normalsize 
\item Under the Assumption \ref{ass:err_noise}
     for the third term in the r.h.s. of Eq. \eqref{eq:prob_var}, the following holds
    \begin{align}\label{eq:first_step_var_delta}
        &\frac{d^2}{2\tau^2}  \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2  \leq  \frac{d^2\Delta^2}{2\tau^2} .
    \end{align}
\end{enumerate}

Thus using Eq.\eqref{eq:first_step_var} and \eqref{eq:first_step_var_delta}  we can estimate the second term in the r.h.s of inequality \eqref{eq:inmainsqE_prob} as follow:
\begin{align}
    &\text{Prob} \left\{ \left| \sum_{k=1}^N \gamma_k^2/2 \|g(z^k,\be^k,\xi^k)\|_2^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1} \right| > \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c  \sum_{k=1}^N \gamma_k } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c  \sum_{k=1}^N \gamma_k }+   \right. \nonumber \\
    &\hspace{4 cm} \left. +  \frac{d^2\Delta^2 \sum_{k=1}^N \gamma_k^2}{2 \tau^2 \sum_{k=1}^N \gamma_k } \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} \label{eq:first_step_second_term}
\end{align}
{\bf Step 2.}\\
Using the notation \eqref{eq:grad_approx_f} we rewrite the l.h.s. of  Eq. \eqref{eq:inmainsqE_prob} as following:

\begin{align}
    &\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra =\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \nonumber\\
    & + \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra + \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra \label{eq:step2_rewriten}
\end{align}
\begin{enumerate}
    \item For the first term in r.h.s. of  Eq. \eqref{eq:step2_rewriten}, we provide the following notions:
% $$\sigma_k = \gamma_k M_2 2 \mathcal D,$$
$$\sigma_k = 2 \gamma_k \sqrt{d} M_2  \sqrt{V_{z^1}(u)} \Omega ,$$
$$\phi_k (\xi_k)= \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra .$$
For applying the case A of Lemma 2 from \cite{lan2012validation} we need to estimate the module of function $\gamma_k\la g_f(z^k,\be^k,\xi^k) , z^k-u\ra$. Using Assumption \ref{ass:uni_Lip_obj} we obtain:
\begin{align}
    &\left| \gamma_k\la g_f(z^k,\be^k,\xi^k) , z^k-u\ra \right| \stackrel{\eqref{eq:grad_approx_f}}{=}  \left| \gamma_k\la \frac{d}{2\tau}\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix} , z^k-u\ra \right|\nonumber\\
    & \stackrel{Ass. \ref{ass:uni_Lip_obj}}{\leq} \gamma_k d M_2 \left| \la  \be , z^k-u\ra \right| \label{eq:estim_of_scalar_product}
\end{align}
Now we need to estimate the term $\left| \la  \be , z^k-u\ra \right|$. To do this, using the Poincaré's lemma from \cite{lifshits2012lectures} paragraph 6.3 we rewrite $\be$ in different form:
\begin{align}\label{eq:poincare_def_e}
    \be \stackrel{D}{=} \frac{\eta}{\sqrt{\eta_1^2 + \dots + \eta_d^2}},
\end{align}

where $\eta = \left( \eta_1, \eta_2, \dots , \eta_d \right)^T = \mathcal{N} \left( 0 , I_d \right)$. 
Using Lemma 1 \cite{laurent2000adaptive}
% \cite{boucheron2013concentration} 
it follows:
\begin{align}
    \text{Prob} \left\{  \sum_{k=1}^d \left|\eta_k\right|^2 \le d -  2 \sqrt{\Omega d} \right\} \leq  \exp \{- \Omega \} . \label{eq:step2_sphere_rewriten}
\end{align}
Using the definition of $\eta$ we obtain:
\begin{align}
    \la \eta, z^k-u \ra \stackrel{D}{=} \mathcal{N} \left( 0 , \|z^k - u\|_2^2 \right). \label{eq:step2_poincare}
\end{align}
Using Eq. \eqref{eq:step2_sphere_rewriten}, \eqref{eq:step2_poincare} and \eqref{eq:poincare_def_e} we can estimate the r.h.s of Eq. \eqref{eq:estim_of_scalar_product}:
\begin{align}
    \text{Prob} &\left\{     \left| \la \be, z^k-u \ra \right| > \frac{ \Omega V_{z^k}(u)}{\sqrt{d}} \right\} \leq 3 \exp \{-\Omega/4 \} . \label{eq:step1_sphere_rewriten_2}
\end{align}










Moreover, using Eq. \eqref{eq:estim_of_scalar_product}, Eq. \eqref{eq:step1_sphere_rewriten_2} and the fact that $V_{z^k}(u) = \O ( V_{z^1}(u)) \text{  } \forall k \geq 1$ from \cite{gorbunov2021gradient} we have:

\begin{align*}
    \text{Prob} \left\{\exp \left\{ \left(\gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra \right)^2/ \sigma_k^2 \right\}  \geq \exp \{1\}\right\} \leq 3 \exp \{-\Omega/4 \}
\end{align*}
It follows by case A of Lemma 2 from \cite{lan2012validation} that
\begin{align}
    & \text{Prob} \left\{ \left| \frac{\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra}{\sum_{k=1}^{N}\gamma_k}  \right| > \frac{4 \sqrt{d} \Omega^2 \sqrt{V_{z^1}(u)} M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} \right\} \leq \\
    & \hspace{8cm}\leq  2 \exp \{-\Omega^2/3 \} + 3 \exp \{-\Omega/4 \}. \label{eq:step2_martingale_rewriten}
\end{align}
\item For the second term in r.h.s of Eq. \eqref{eq:step2_rewriten} under the Assumption \ref{ass:err_noise} we obtain :
\begin{align}
    & \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra \geq - \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left|\la \be, z^k-u \ra \right| \label{eq:step2_delta_rewriten}
\end{align}

Using Eq. \eqref{eq:step1_sphere_rewriten_2} we can estimate the r.h.s of Eq. \eqref{eq:step2_delta_rewriten}:
\begin{align}
    \text{Prob} &\left\{   \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left| \la \be, z^k-u \ra \right| > \frac{ \Omega \D \sqrt{d} \Delta \sum_{k=1}^N \gamma_k}{\tau} \right\} \leq 3 \exp \{-\Omega/4 \} . \label{eq:step2_sphere_rewriten_2}
\end{align}
\item We rewrite the third term in r.h.s. of  Eq. \eqref{eq:step2_rewriten} in the following form: 
\begin{align} 
    \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra & =  \sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra  \notag \\
     &=  \sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right) \notag \\
     &\geq  \sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y)) \notag \\
     &=  \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \label{eq:eqexpfxy_prob}.
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE_prob}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq  f^\tau\left(\frac{\sum_{k=1}^N \gamma_k x^k}{\sum_{k=1}^{N}\gamma_k},y\right)  - f^\tau\left(x, \frac{\sum_{k=1}^N \gamma_k y^k}{\sum_{k=1}^{N}\gamma_k}\right)\notag \\
     &=  f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE_prob}  for Eq. \eqref{eq:eqexpfxy_prob} we get 
\begin{align}\label{eq:fpslff_prob}
      \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra  
     &\geq \left( \sum_{k=1}^{N}\gamma_k \right) \left( f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right) .
\end{align}
\end{enumerate}









{\bf Step 3.} \\
Then we use this with  Eq. \eqref{eq:step2_rewriten}, \eqref{eq:step2_delta_rewriten} and \eqref{eq:fpslff_prob} for Eq. \eqref{eq:inmainsqE_prob} and obtain
\begin{align}
      &f^\tau\left( \hat x^N,y\right)   - f^\tau\left(x, \hat y^N \right)  \leq   \frac{V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k } + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_2^2  \nonumber \\
    & - \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \la \be, z^k-u \ra \label{eq:exEeqE_prob}
\end{align}


 For the l.h.s. of Eq. \eqref{eq:exEeqE_prob} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2 \label{eq:f_tau_to_f}
 \end{align}
 Using Eq. \eqref{eq:first_step_second_term}, \eqref{eq:step2_martingale_rewriten}, \eqref{eq:step2_sphere_rewriten_2}, \eqref{eq:f_tau_to_f} and taking the maximum in $(x,y) \in (\X,\Y)$, we obtain we can rewrite Eq. \eqref{eq:exEeqE_prob} as follow:
 
 \begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \sqrt{V_{z^1}(u)} M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c \sum_{k=1}^N \gamma_k }  \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c \sum_{k=1}^N \gamma_k } +  \frac{d^2\Delta^2 \sum_{k=1}^N \gamma_k^2}{2 \tau^2 \sum_{k=1}^N \gamma_k } + \frac{V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
      & \hspace{3cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \}\label{eq:dghjsklslsl_proba}
\end{align}
%  \begin{align}
%       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } +\frac{d \D \Delta}{\tau} \right. \nonumber\\
%       & \left.+ \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
%       & \hspace{5cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} \label{eq:dghjsklslsl_proba}
% \end{align}

 Choosing the learning rate $\gamma_k 
=\frac{\sqrt{V_{z^1}(u)}}{M}\sqrt{\frac{2}{N}}$ with $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl_proba} we obtain
\begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \sqrt{V_{z^1}(u)} M_2  }{\sqrt{N}} + \frac{2 \sqrt{2}  \sqrt{V_{z^1}(u)} M_2^2 d}{c M\sqrt{N}}   + \right. \nonumber\\
      & \hspace{2cm}\left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2 \sqrt{2} M_2^2 d \sqrt{V_{z^1}(u)}}{c M N} +  \frac{d^2\Delta^2 \sqrt{2} \sqrt{V_{z^1}(u)}}{2 \tau^2 M \sqrt{N} }+ \frac{\sqrt{V_{z^1}(u)} M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
      & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .
\end{align}

Using the notation of $M$ we obtain:
\begin{align}
       &\text{Prob}  \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{  \sqrt{V_{z^1}(u)} M  }{\sqrt{N}}   + \frac{ \Omega \D \sqrt{d} \Delta }{\tau }  + \right. \nonumber\\
      & \left.+2 \tau M_2 + \Omega \frac{2 \sqrt{2} M \sqrt{V_{z^1}(u)}}{c N}    \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .
\end{align}

% \begin{align}
%       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2}{M}  +\frac{d \D \Delta}{\tau} + \right. \nonumber\\
%       & \left. \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} 
% \end{align}
\end{proof}




==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/restarts.tex <==
\section{Restarts and Linear Convergence Rate}\label{sec:rest}
In this section we apply restart-technique \cite{juditsky2014deterministic} to  Algorithm\ref{alg:zoSPA} in the case when we additionally have $\gamma-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems). 
\begin{assumption}\label{ass:strongly_convex}
There is $\gamma \geq 1$ and $\mu_{\gamma} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
$$ \frac{\mu_{\gamma}}{2} \|z-z^{\star}\|_p^{\gamma} 
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right).
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
$$
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
Then for the output $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA},  the following holds for $ \e_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \e_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \e_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $a_q^2$ is such that $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, if Assumption \ref{ass:strongly_convex} is satisfied we can apply restarts and to achieve $\E[\e_{\rm sad}] \leq \varepsilon$ one need $N$ iterations where $N$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N &= \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right),\\
     N &=  \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right),
 \end{align}
 where $B$ is an inaccuracy associated with the $\tau$-smoothing and inexactness of the oracle. 
 Constants $A, B$ depend on noise conditions and are given by the following equality
 \begin{enumerate}
    \item under Assumption \ref{ass:err_noise} 
 \begin{align}\label{eq:err_noise_AB}
      A = \sqrt{2} M_{\rm case1}, \;\;\; B = {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2,
 \end{align}
    \item under Assumption \ref{ass:Lip_noise} 
    \begin{align}\label{eq:err_noise_AB_2}
      A = \sqrt{2} M_{\rm case2}, \;\;\; B = M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.
 \end{align}
\end{enumerate}
Thus, from \eqref{eq:err_noise_AB} $\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon^2/\left(\D M_2\sqrt{d}\right)\right)$ and from \eqref{eq:err_noise_AB_2}
$\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon/\left(\D\sqrt{d}\right)\right)$.
\end{theorem}

\begin{remark}
An important particular case of Theorem~\ref{th:conv_rate_restarts} is when $\gamma = 1$. Under this assumption the estimate on the number of iteration $\eqref{eq:estim_iter_restart}$ can be rewritten in the following form:
 \begin{align}
     N = \widetilde \O\left(\frac{64 \cdot A^2}{\mu_{1}^2 } \right) = \widetilde \O\left(\frac{A^2}{\mu_{1}^{2} } \right).
 \end{align}
As a result, it leads us to the linear convergence of the algorithm for non-smooth convex-concave saddle points problems with sharp saddle-point. For convex optimization problems with sharp minimum this effect was known \cite{juditsky1993stochastic}.
\end{remark}



%  \iffalse

\begin{proof}[Proof of the  Theorem \ref{th:conv_rate_restarts}]
By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) - \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2   \notag
\end{align}
Summing for $k=1,\dots,N$  and taking the expectation, we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE_restarts}
   \E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right]
   &\leq \E [V_{z^1}(u)]  - \E\left[\sum_{k=1}^N\frac{\gamma_k^2}{2}\|g(z^k,\be^k,\xi^k)\|_q^2 \right] \notag\\
   &\leq  \E[V_{z^1}(u)] + \sum_{k=1}^N \frac{\gamma_k^2}{2} \E\left[\|g(z^k,\be^k,\xi^k)\|_q^2\right],
\end{align}
where we took into account that $z^1$ can be chosen in stochastic way.

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE_restarts} we use Lemma \ref{lm:shamirEnabla} and obtain
 \begin{enumerate}[leftmargin=*]
     \item  under Assumption  \ref{ass:err_noise}:
     \begin{equation}\label{eq:inmainsqEtwo1_restarts}
        \E\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}{\tau^{-2}}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise}: 
\begin{align}\label{eq:inmainsqEtwo_restarts}
    \E\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q d (M_2^2+M_{2,\delta}^2),
\end{align}
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$.

{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE_restarts}, we use Lemma \ref{lm:expecapproxgrad}


 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz11_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] =  \E\left[\sum_{k=1}^N \gamma_k\left\la \E_{\be^k}\left[g(z^k,\be^k,\xi^k) \right], z^k-u\right\ra \right] \notag\\
     &\hspace{2cm}\geq  \E\left[\sum_{k=1}^N \gamma_k \la \nabla f^\tau(z^k), z^k-u \ra \right] - \E\left[\sum_{k=1}^N \gamma_k\left|\la  {d\Delta}{\tau^{-1}}  \be^k, z^k-u  \ra \right|\right].
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] =  \E\left[\sum_{k=1}^N \gamma_k\left\la \E_{\be^k}\left[g(z^k,\be^k,\xi^k) \right], z^k-u\right\ra \right] \notag\\
     &\hspace{2cm}\geq  \E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right]-\E\left[\sum_{k=1}^N \gamma_k\left|\la  dM_{2,\delta} \be^k, z^k-u\ra\right| \right].
\end{align}
 \end{enumerate}
For the first term of the r.h.s. of Eq.\eqref{eq:eqrefeqffxyz11_restarts} and \eqref{eq:eqrefeqffxyz_restarts} we have 
\begin{align}\label{eq:eqexpfxy_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right]
     =  \E\left[\sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra \right] \notag \\
     &=  \E\left[\sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right)\right] \notag \\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y))\right] \notag \\
     &=  \E\left[\sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \right].
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE_restarts}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq    f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE_restarts}  for Eq. \eqref{eq:eqexpfxy_restarts} we get 
\begin{align}\label{eq:fpslff_restarts}
      \E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right] 
     &\geq \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right].
\end{align}
Next we estimate the term $\E_{\be^k} \left[    |\la \be^k, z^k-u\ra|  \right] $ in Eq. \eqref{eq:eqrefeqffxyz11_restarts} and \eqref{eq:eqrefeqffxyz_restarts},   by the Lemma~\ref{lm:dotprodvece} 
\begin{align}\label{eq:sectermErhs_restarts}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\D}/{\sqrt{d}}. 
\end{align}
Now  we substitute  Eq. \eqref{eq:fpslff_restarts} and  \eqref{eq:sectermErhs_restarts} to Eq. \eqref{eq:eqrefeqffxyz11_restarts} and \eqref{eq:eqrefeqffxyz_restarts}, and get
 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz1122_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right]
    \geq 
     \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)- f^\tau\left(x, \hat y^N \right) \right] -  \sum_{k=1}^N \gamma_k \frac{\sqrt{d}\Delta\D}{\tau}.  
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz22_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] \geq  \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right) - f^\tau\left(x, \hat y^N \right) \right] - \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta}\D. 
\end{align}
 \end{enumerate}
 
{\bf Step 3.} (under Assumption \ref{ass:err_noise}) \\
Now we combine Eq. \eqref{eq:eqrefeqffxyz1122_restarts}   with  Eq. \eqref{eq:inmainsqEtwo1_restarts} for Eq. \eqref{eq:inmainsqE_restarts} and obtain under Assumption \ref{ass:err_noise} the following
     \begin{align}\label{eq:inmainsqEtwo133_restarts}
    & \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
     -  \sum_{k=1}^N \gamma_k \frac{\Delta\D\sqrt{d}}{\tau} \notag\\
     &\leq \E [V_{z^1}(u)] +  \sum_{k=1}^N \frac{\gamma_k^2}{2} \left(c a^2_q dM_2^2 + \frac{d^2 a_q^2\Delta^2}{\tau^2}\right).
     \end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE1_restarts}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      &\leq 
     \frac{ \E [V_{z^1}(u)]}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q dM_2^2+ d^2 a_q^2\Delta^2\tau^{-2}}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  +\frac{\Delta\D\sqrt{d}}{\tau}.
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE1_restarts} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE1_restarts} and  choosing $(x,y) = (x^{\star}, y^{\star})$, we obtain
 \begin{align}\label{eq:dghjsklslsl1_restarts}
     \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq \frac{ \E [V_{z^1}(z^{\star})]+ (c a^2_q d M_2^2 +
     d^2 a_q^2\Delta^2\tau^{-2})
    \sum_{k=1}^{N} {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
       \notag \\
    &+ {\Delta\D\sqrt{d}}{\tau^{-1}}
     +  2\tau M_2.
 \end{align}
%  where $D^2(z^1, z^{\star}) = V_{z^1}(z^{\star})$.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Choosing  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl1_restarts} we get
 \begin{align*}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  
     %\frac{V_{z^1}(u)(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E [V_{z^1}(z^{\star})]}
     + \frac{\Delta\D\sqrt{d}}{\tau} 
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 4.} (under Assumption \ref{ass:Lip_noise})\\
Now we combine Eq.  \eqref{eq:eqrefeqffxyz22_restarts}  with  Eq.  \eqref{eq:inmainsqEtwo_restarts} for Eq. \eqref{eq:inmainsqE_restarts} and obtain under Assumption~\ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo334_restarts}
    &\sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
    - \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta} \D \leq \E [V_{z^1}(u)] +  \sum_{k=1}^N \frac{\gamma_k^2}{2} c a^2_q d (M_2^2+M_{2,\delta}^2).
\end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE_restarts}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      &\leq 
     \frac{ \E [V_{z^1}(u)]}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q d (M_2^2+M_{2,\delta}^2)}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  + M_{2,\delta} \D \sqrt{d}. 
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE_restarts} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE_restarts} and   chooosing $(x,y) = (x^{\star}, y^{\star})$, we obtain
 \begin{align}\label{eq:dghjsklslsl_restarts}
     \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq \frac{ \E [V_{z^1}(z^{\star})] + c a^2_q d (M_2^2+M_{2,\delta}^2)\sum_{k=1}^N {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
    \notag \\
    &+ M_{2,\delta}  \sqrt{d}\D
     +  2\tau M_2.
 \end{align}
 Choosing the learning rate 
%   $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$  in Eq. \eqref{eq:dghjsklslsl} we obtain
%  \begin{align*}
%       \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
%      &\leq  \frac{\D(1+c a^2_q d M_2^2 + c a^2_q dM_{2,\delta}^2)}{\sqrt{2N}M}  + M_{2,\delta} \D \sqrt{d} 
%      +  2\tau M_2.  
%  \end{align*}
 $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl_restarts} we obtain
 \begin{align*}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E [V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 5.} (Restart)
 At the previous step, we obtained the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq  \frac{A\sqrt{\E [V_{z^1}(z^{\star})]}}{\sqrt{N_1}}  + B,  
 \end{align}
 with an appropriate choice of constants $A, B$. Here $B$ is an inaccuracy associated with the stochastic setting of the problem and inexactness of the oracle. In this step we will employ the restart technique that is generalization of technique proposed in \cite{juditsky2014deterministic}.
 
 For the r.h.s. of Eq. \eqref{restart:rate} we use Assumption \ref{ass:strongly_convex} and the fact of remark 3 from \cite{gasnikov2018universal} that $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$ for the l.h.s 
 \begin{align}\label{restart:norms}
 \underbrace{\frac{\mu_{\gamma}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{\gamma}\right]}_{\geq\frac{\mu_{\gamma}}{2} \E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}
 \leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= A\widetilde \O(\underbrace{\E[\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}  + B.
 \end{align}
 Then by choosing ${N_1} = \frac{A^2\widetilde \O(R_0^2)}{B^2}$ and applying the Jensen inequality for l.h.s of Eq. \eqref{restart:norms} we get
 \begin{align}
 \frac{\mu_{\gamma}}{2} \underbrace{\E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}_{R_1^{\gamma}} \leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= 2A\widetilde \O(\underbrace{\E [\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}.
 \end{align}
 And finally taking ${N_1}$ so as to reduce the distance to the solution by half, we obtain
 $$ {N_1} = \widetilde \O \left( \frac{64A^2}{\mu_{\gamma}^2 R_1^{2(\gamma-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ from a similar condition for reducing the distance to the solution by a factor of $2$, and so on. 
 
 Thus, after $k$ of such restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N = N_1 +\dots + N_k = \widetilde \O \left(\frac{64 \cdot 2^{2(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}}\left(1+2^{2(\gamma-1)} + \dots + 2^{2(k-1)(\gamma-1)}\right) \right).
 \end{align} 
 It remains for us to determine the number of restarts, for this we fix the desired accuracy in terms of $\E[\e_{\rm sad}] \leq \varepsilon$ and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\e_{\rm sad}] = \widetilde \O \left(\frac{\mu_{\gamma} R_k^{\gamma}}{2}\right)=   \frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{\gamma}R_0^{\gamma}}{2^{k\gamma}}\right) \leq \varepsilon.
 \end{align} 
 Then to fulfill this condition one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{\gamma}R_0^{\gamma}/\varepsilon\right)) / \gamma$ and using Eq. \eqref{restart:N} we get the total number of iterations
 $$ N = \widetilde \O\left(\frac{64 \cdot 2^{2k(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}} \right) = \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right).$$
 Moreover, using ${N_k} = \frac{A^2\widetilde \O(R_{k-1}^2)}{B^2}$ and $\frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  \leq \varepsilon$ from Eq. \eqref{restart:epsilon} we have $B = \tilde{O}(\varepsilon)$.  This condition imposes restrictions on the final accuracy $\varepsilon$ and, as a consequence, on the choice of $N$, given by Eq. \eqref{restart:N}
 \begin{align*}
     N = \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right).
 \end{align*}
\end{proof}




\begin{remark}
The estimations on the noise $B$ in Eq. \eqref{eq:err_noise_AB} and \eqref{eq:err_noise_AB_2} can be improved in the following way: it is possible to obtain the better evaluation on the r.h.s of Eq. \eqref{eq:sectermErhs_restarts} as
\begin{align}\label{eq:sectermErhs_restarts_new}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|_2  \right] \leq {\|z^k - u\|}/{\sqrt{d}}. 
\end{align}
Choosing $u = (x^*, y^*)$ we provide exponentially decreasing sequence of $\D_2^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate}. It leads us to the more precise estimation on the noise $B$. We use this estimation on $B$ when we employ the restart technique in the proof of Theorem~\ref{th:conv_rate_restarts} and, thanks to this, we obtain the better estimate on the maximal level of noise: under Assumption \ref{ass:err_noise} $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{2-1/\gamma}}{M_2\sqrt{d}}$$  and 
under Assumption \ref{ass:Lip_noise} 
$$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{1-1/\gamma}}{\sqrt{d}}.$$
\end{remark}

\begin{remark}\label{hpb}
Based on high-probability bound from Appendix~\ref{H-PB} we can obtain high-probability bound by using the same restart-technique \cite{juditsky2014deterministic}. In the case $\gamma = 2$ it is probably possible to improve this bound in $\log \varepsilon^{-1}$ factor by using alternative algorithm \cite{harvey2019tight}. Moreover, based on stochastic-gradient clipping trick \cite{gorbunov2021near} we can obtain the result in Appendix~\ref{H-PB} in the case when the second moment of stochastic gradient is bounded (subgaussian tails are not required). When the variance of noise is not bounded (the second moment of stochastic gradient is non bounded) the rate of convergence may changes drastically, see the next section.
\end{remark}
% \fi



==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/restarts_MOTOR.tex <==
\section{Restarts}\label{sec:rest}
In this section, we assume that we  additionally have the $r-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems).  For such a case, we apply the restart technique \cite{juditsky2014deterministic} to  Algorithm \ref{alg:zoSPA} 
\begin{assumption}[$r-$growth condition]\label{ass:strongly_convex}
There is $r \geq 1$ and $\mu_{r} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
\[\frac{\mu_{r}}{2} \|z-z^{\star}\|_p^{r}
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right),
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
\]
where $(x^*,y^*)$ is a solution of problem \eqref{eq:min_max_problem}.
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy Assumption \ref{ass:Lip_obj}. 
Then the following holds for $ \e_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$, where   $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ is the output of   Algorithm \ref{alg:zoSPA} 
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \e_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \e_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If the Assumption \ref{ass:strongly_convex} is satisfied for $r \geq 2$  and one of the two following statement is true
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, we can apply restart technique  to achieve $\E[\e_{\rm sad}] \leq \e$ in $N_{acc}$ iterations, where $N_{acc}$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N_{acc} = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \e^{2(r-1)/r}} \right).
 \end{align}
\end{theorem}
\textit{Proof of  Theorem \ref{th:conv_rate_restarts}.}
~We repeat the proof of Theorem \ref{th:conv_rate}, except that now $z^1$ can be chosen in a stochastic way. Moreover, now we use a rougher inequality instead of \eqref{eq:sectermErhs}
\begin{align}\label{eq:sectermErhs_restarts}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\D}/{\sqrt{d}}.
\end{align}
{\bf Step 1.} (under Assumption \ref{ass:err_noise}) \\
Taking the expectation in \eqref{eq:dghjsklslsl1}, choosing $(x,y) = (x^{\star}, y^{\star})$, and
 learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$  we get
 \begin{align} \label{rate:restarts1}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  
     %\frac{V_{z^1}(u)(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E [V_{z^1}(z^{\star})]}
     + \frac{\Delta\D\sqrt{d}}{\tau} 
     +  2\tau M_2.  
 \end{align}
 {\bf Step 2.} (under Assumption \ref{ass:Lip_noise})\\
Taking the mathematical expectation in \eqref{eq:dghjsklslsl1}, choosing $(x,y) = (x^{\star}, y^{\star})$, and  learning rate 
 $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$  we obtain
 \begin{align} \label{rate:restarts2}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E [V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.  
 \end{align}
{\bf Step 3.} (Restarts)\\
Now let $\tau$ be chosen as $\tau = \O\left(\e/M_2\right)$, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement holds
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then using \eqref{rate:restarts1} we obtain the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= \widetilde \O\left(\  a_q M_2 \sqrt{2d}\sqrt{\frac{\E [V_{z^1}(z^{\star})]}{N_1}}\right).
 \end{align}
  In this step we will employ the restart technique that is a generalization of technique proposed in \cite{juditsky2014deterministic}.\\
 For the l.h.s. of Eq. \eqref{restart:rate} we use the Assumption \ref{ass:strongly_convex}. For the r.h.s. of Eq. \eqref{restart:rate} we use $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$  from  \cite[Remark 3]{gasnikov2018universal}  
 \begin{align}\label{restart:norms}
 \frac{\mu_{r}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{r}\right]
 &\leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] \notag \\
     &= \frac{a_q M_2 \sqrt{2d}}{\sqrt{{N_1}}}\widetilde \O\left(\sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
 Then the l.h.s of Eq. \eqref{restart:norms} we  use the Jensen inequality and  get the following
 \begin{align}
 \frac{\mu_{r}}{2} \underbrace{\left(\sqrt{\E\left[\|z^{N_1} - z^{\star}\|_p^2\right]}\right)^{r}}_{R_1^{r}} &\leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] \notag\\
     &= \frac{a_q M_2 \sqrt{2d}}{\sqrt{{N_1}}}\widetilde \O\left(\sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
Finally taking ${N_1}$ so as to halve the distance to the solution, we get
 $$ {N_1} = \widetilde \O \left( \frac{a_q^2 M_2^2 d}{\mu_{r}^2 R_1^{2(r-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ similarly: we halve the distance $R_1$ to the solution, and so on. \\
 Thus, after $k$  restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N_{acc} = N_1 +\dots + N_k = \widetilde \O \left(\frac{ 2^{2(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}}\left(1+2^{2(r-1)} + \dots + 2^{2(k-1)(r-1)}\right) \right).
 \end{align} 
 Now we need  to determine the number of restarts. To do  this, we fix the desired accuracy  and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\e_{\rm sad}] = \widetilde \O \left(\frac{\mu_{r} R_k^{r}}{2}\right)=   \frac{2 a_q M_2 \sqrt{d} \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{r}R_0^{r}}{2^{kr}}\right) \leq \e.
 \end{align} 
 Then to fulfill this condition, one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{r}R_0^{r}/\e\right)) / r$ and using Eq. \eqref{restart:N} we get the total number of iterations
\[ N_{acc} = \widetilde \O\left(\frac{32 \cdot 2^{2k(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}} \right) = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \e^{2(r-1)/r}} \right).\]
\qed



\begin{remark}
If in Theorem \ref{th:conv_rate_restarts} we use a tighter inequality   \eqref{eq:sectermErhs} instead of
\eqref{eq:sectermErhs_restarts} (as in Theorem \ref{th:conv_rate}), then
the estimations on the $\Delta$ and $M_{2,\delta}$   can be improved.
Choosing $u = (x^*, y^*)$ we can provide exponentially decreasing sequence of $\D^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate} and get 
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} $\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\e^{2-1/\gamma}}{M_2\sqrt{d}}$
    \item under Assumption \ref{ass:Lip_noise} 
$M_{2,\delta} \lesssim \frac{\mu_{\gamma}^{1/\gamma}\e^{1-1/\gamma}}{\sqrt{d}}$.
\end{enumerate}

\end{remark}







==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/restarts_new.tex <==
\section{Restarts}\label{sec:rest}
In this section, we assume that we  additionally have the $r-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems).  For such a case, we apply the restart technique \cite{juditsky2014deterministic} to  Algorithm \ref{alg:zoSPA} 
\begin{assumption}[$r-$growth condition]\label{ass:strongly_convex}
There is $r \geq 1$ and $\mu_{r} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
\[\frac{\mu_{r}}{2} \|z-z^{\star}\|_p^{r}
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right),
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
\]
where $(x^*,y^*)$ is a solution of problem \eqref{eq:min_max_problem}.
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
Then the following holds for $ \hat{\e}_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$, where   $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ is the output of   Algorithm \ref{alg:zoSPA},  
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \hat{\e}_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \hat{\e}_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement is true
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\E\left[\hat{\e}_{\rm sad}(\hat z^N)\right]\leq\e$  after 
% \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\D^{-2}\e^2)^2 \right)\]
\[N =  \O\left( {da_q^2M_2^2\D^2}/{\e^{2}} \right)\]
iterations. If also Assumption \ref{ass:strongly_convex} is satisfied for $r \geq 2$ we can apply restarts and to achieve $\E[\hat{\e}_{\rm sad}] \leq \varepsilon$ in $N_{acc}$ iterations where $N_{acc}$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N_{acc} = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \varepsilon^{2(r-1)/r}} \right).
 \end{align}
\end{theorem}


% \begin{corollary}\label{cor:bound_noise_restarts}
% Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}, and 
% let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement is true
% \begin{enumerate}
%     \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
%     \item Assumption \ref{ass:Lip_noise} holds and 
%  $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
% \end{enumerate}
% then 
% for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\E\left[\e_{\rm sad}(\hat z^N)\right]=\e$  after 
% % \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\D^{-2}\e^2)^2 \right)\]
% \[N =  \O\left( {da_q^2M_2^2\D^2}/{\e^{2}} \right)\]
% iterations, where 
%  $\sqrt{\E \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
% % \begin{enumerate}
% %     \item 
%     % under Assumption \ref{ass:err_noise}
%     % \[\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O \left( \frac{\e}{M_2} \right) \] 
  
%     % \item under Assumption \ref{ass:Lip_noise}
%     %   \[\delta(z) =\O\left( \frac{\e}{\D\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O\left( \frac{\e}{M_2} \right) \] 
% %\end{enumerate}
% % where $\e = \max\limits_{y\in \Y}  f(\hat x^N, y) - \min\limits_{x\in \X}   f(x, \hat y^N)$ and $(\hat x^N, \hat y^N,)$ are the outputs of the    Algorithm \ref{alg:zoSPA} after 
% % \[N = \O\left( {M^2\D^2(1+ca_q^2d)^2}{\e^{-1}} \right)\]
% % iterations.
% \end{corollary}

% \begin{remark}
% An important particular case of Theorem~\ref{th:conv_rate_restarts} is when $\gamma = 1$. Under this assumption the estimate on the number of iteration $\eqref{eq:estim_iter_restart}$ can be rewritten in the following form:
%  \begin{align}
%      N = \widetilde \O\left(\frac{64 \cdot A^2}{\mu_{1}^2 } \right) = \widetilde \O\left(\frac{A^2}{\mu_{1}^{2} } \right).
%  \end{align}
% As a result, it leads us to the linear convergence of the algorithm for non-smooth convex-concave saddle points problems with sharp saddle-point. For convex optimization problems with sharp minimum this effect was known \cite{juditsky1993stochastic}.
% \end{remark}



%  \iffalse

\textit{Proof of  Theorem \ref{th:conv_rate_restarts}}
~We repeat the proof of Theorem \ref{th:conv_rate}, except that now $z^1$ can be chosen in a stochastic way. Moreover, now we use a rougher inequality instead of \eqref{eq:sectermErhs}
\begin{align}\label{eq:sectermErhs_restarts}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\D}/{\sqrt{d}}.
\end{align}
{\bf Step 1.} (under Assumption \ref{ass:err_noise}) \\
Taking the expectation in \eqref{eq:exEeqE1}, choosing $(x,y) = (x^{\star}, y^{\star})$, and
 learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$  we get
 \begin{align} \label{rate:restarts1}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  
     %\frac{V_{z^1}(u)(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E [V_{z^1}(z^{\star})]}
     + \frac{\sqrt{d}\Delta\D}{\tau} 
     +  2\tau M_2.  
 \end{align}
 {\bf Step 2.} (under Assumption \ref{ass:Lip_noise})\\
Taking the expectation in \eqref{eq:exEeqE}, choosing $(x,y) = (x^{\star}, y^{\star})$, and  learning rate 
 $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$  we obtain
 \begin{align} \label{rate:restarts2}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E [V_{z^1}(z^{\star})]}  + M_{2,\delta}\sqrt{d} \D  
     +  2\tau M_2.  
 \end{align}
{\bf Step 3.} (Restarts)\\
Now let $\tau$ be chosen as $\tau = \O\left(\e/M_2\right)$, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement holds
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then using \eqref{rate:restarts1} we obtain the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= \widetilde \O\left(\frac{a_q M_2 \sqrt{d}}{\sqrt{N_1}}\sqrt{\E [V_{z^1}(z^{\star})]}\right).
 \end{align}
  In this step we will employ the restart technique that is a generalization of the technique proposed in \cite{juditsky2014deterministic}.\\
 For the l.h.s. of Eq. \eqref{restart:rate} we use the Assumption \ref{ass:strongly_convex}. For the r.h.s. of Eq. \eqref{restart:rate} we use $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$  from  \citet[Remark 3]{gasnikov2018universal}  
 \begin{align}\label{restart:norms}
 \frac{\mu_{r}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{r}\right]
 &\leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] = \widetilde \O\left(\frac{a_q M_2 \sqrt{d}}{\sqrt{{N_1}}} \sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
 Then the l.h.s of Eq. \eqref{restart:norms} we  use the Jensen inequality and  get the following
 \begin{align}
 \frac{\mu_{r}}{2} \left({\E\left[\|z^{N_1} - z^{\star}\|_p^2\right]}\right)^{r/2} &\leq   \frac{\mu_{r}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{r}\right] \leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] \notag\\
     &= \widetilde \O\left( \frac{a_q M_2 \sqrt{d}}{\sqrt{{N_1}}} \sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
Finally, 
let us introduce $R_k \triangleq \sqrt{\E\left[\|z^{N_k} - z^{\star}\|_p^2\right]}$ and $R_0 \triangleq \sqrt{\E\left[\|z^{1} - z^{\star}\|_p^2\right]}$. Then we
take ${N_1}$ so as to halve the distance to the solution and get
 $$ {N_1} = \widetilde \O \left( \frac{a_q^2 M_2^2 d}{\mu_{r}^2 R_1^{2(r-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ similarly: we halve the distance $R_1$ to the solution, and so on. \\
 Thus, after $k$  restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N_{acc} = N_1 +\dots + N_k = \widetilde \O \left(\frac{ 2^{2(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}}\left(1+2^{2(r-1)} + \dots + 2^{2(k-1)(r-1)}\right) \right).
 \end{align} 
 Now we need  to determine the number of restarts. To do  this, we fix the desired accuracy  and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\hat{\e}_{\rm sad}] =  \widetilde \O \left(\frac{\mu_{r} R_k^{r}}{2}\right)=   \widetilde \O\left( \frac{ a_q M_2 \sqrt{d} }{\sqrt{N_k}}  R_{k-1}\right) = \widetilde \O \left(\frac{\mu_{r}R_0^{r}}{2^{kr}}\right)  \leq \e.
 \end{align} 
 Then to fulfill this condition, one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{r}R_0^{r}/\e\right)) / r$ and using Eq. \eqref{restart:N} we get the total number of iterations
\[ N_{acc} = \widetilde \O\left(\frac{ 2^{2k(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}} \right) = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \e^{2(r-1)/r}} \right).\]
\qed


\begin{remark}
If in Theorem \ref{th:conv_rate_restarts}, we use a tighter inequality   \eqref{eq:sectermErhs} instead of
\eqref{eq:sectermErhs_restarts} (as in Theorem \ref{th:conv_rate}), then
the estimations on the $\Delta$ and $M_{2,\delta}$   can be improved.
Choosing $u = (x^*, y^*)$ we can provide exponentially decreasing sequence of $\D^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate} and get 
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} $\Delta \lesssim \frac{\mu_{r}^{1/r}\e^{2-1/r}}{M_2\sqrt{d}}$
    \item under Assumption \ref{ass:Lip_noise} 
$M_{2,\delta} \lesssim \frac{\mu_{r}^{1/r}\e^{1-1/r}}{\sqrt{d}}$.
\end{enumerate}

\end{remark}

% \begin{remark}
% The estimations on the noise $B$ in Eq. \eqref{eq:err_noise_AB} and \eqref{eq:err_noise_AB_2} can be improved in the following way: it is possible to obtain the better evaluation on the r.h.s of Eq. \eqref{eq:sectermErhs_restarts} as
% \begin{align}\label{eq:sectermErhs_restarts_new}
%   \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|_2  \right] \leq {\|z^k - u\|}/{\sqrt{d}}. 
% \end{align}
% Choosing $u = (x^*, y^*)$ we provide exponentially decreasing sequence of $\D_2^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate}. It leads us to the more precise estimation on the noise $B$. We use this estimation on $B$ when we employ the restart technique in the proof of Theorem~\ref{th:conv_rate_restarts} and, thanks to this, we obtain the better estimate on the maximal level of noise: under Assumption \ref{ass:err_noise} $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{2-1/\gamma}}{M_2\sqrt{d}}$$  and 
% under Assumption \ref{ass:Lip_noise} 
% $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{1-1/\gamma}}{\sqrt{d}}.$$
% \end{remark}

\begin{remark}\label{hpb}
Based on high-probability bound  we can obtain high-probability bound by using the same restart-technique \cite{juditsky2014deterministic}. In the case $r = 2$ it is probably possible to improve this bound in $\log \varepsilon^{-1}$ factor by using alternative algorithm \cite{harvey2019tight}. 
\end{remark}
% \fi

\begin{theorem}\label{th:conv_rate_restarts_prob} 
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:uni_Lip_obj} and Assumption \ref{ass:err_noise} for some constant $c$. Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
=\frac{\D}{M}\sqrt{\frac{2}{N}}$, where  $N$ is the number of iterations and $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$. Then for the output $  (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA},  the following holds
% \begin{align}
%       \Prob & \left\{ \e_{\rm sad} (\hat z^N)  \geq \frac{4 \Omega^2 \sqrt{d} \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2 d^2}{M}   + \right. \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 d^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
%       & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} 
% \end{align}
\begin{align}
       &\Prob  \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{  \mathcal D M  }{\sqrt{N}}   + \frac{ \Omega \D \sqrt{d} \Delta }{\tau } +2 \tau M_2 + \right. \nonumber\\
      & \left.  + \Omega \frac{2 \sqrt{2} M \D}{c N}   \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} \label{eq:convergrate_prob_restarts}.
\end{align}

 Let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If also Assumption \ref{ass:err_noise} holds true with $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$ after 
\[N =  \O\left( {d M_2^2\D^2}/{\e^{2}} \right)\]
iterations. If moreover Assumption \ref{ass:strongly_convex} is satisfied we can apply restarts and to achieve $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$ in $N_{acc}$ iterations where $N_{acc}$ is given by
 \begin{align}\label{eq:estim_iter_restart_prob}
     N_{acc} = \widetilde \O\left(\frac{M_2^2 d}{\mu_{r}^{2/r} \varepsilon^{2(r-1)/r}} \right).
 \end{align}
\end{theorem}

\begin{proof}
We recall inequality \eqref{eq:dghjsklslsl_proba} from Theorem \ref{th:conv_rate_prob}:
\begin{align}
       &\Prob  \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \|z^1 -z^{\star}\|_p M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c \sum_{k=1}^N \gamma_k }  \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c \sum_{k=1}^N \gamma_k } +  \frac{d^2\Delta^2 \sum_{k=1}^N \gamma_k^2}{2 \tau^2 \sum_{k=1}^N \gamma_k } + \frac{ \|z^1 -z^{\star}\|_p^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
      & \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \}\label{eq:dghjsklslsl_proba_restarts}.
\end{align}
%  \begin{align}
%       \Prob & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } +\frac{d \D \Delta}{\tau} \right. \nonumber\\
%       & \left.+ \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
%       & \hspace{5cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} \label{eq:dghjsklslsl_proba}
% \end{align}
 Choosing  learning rate $\gamma_k 
=\frac{\|z^1 -z^{\star}\|_p}{M}\sqrt{\frac{2}{N}}$ with $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl_proba_restarts} we obtain

\begin{align}
       \Prob & \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \|z^1 -z^{\star}\|_p M_2  }{\sqrt{N}} + \frac{2 \sqrt{2}  \|z^1 -z^{\star}\|_p M_2^2 d}{c M\sqrt{N}}   + \right. \nonumber\\
      & \hspace{3cm}\left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2 \sqrt{2} M_2^2 d\|z^1 -z^{\star}\|_p}{c M N} +  \frac{d^2\Delta^2 \sqrt{2} \D}{2 \tau^2 M \sqrt{N} }+ \frac{\|z^1 -z^{\star}\|_p M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
      & \hspace{2cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .
\end{align}
Using the notation of $M$ we obtain:
\begin{align}
       &\Prob  \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{\|z^1 -z^{\star}\|_p M  }{\sqrt{N}}   + \frac{ \Omega \D \sqrt{d} \Delta }{\tau } +2 \tau M_2 + \right. \nonumber\\
      & \left. + \Omega \frac{2 \sqrt{2} M \|z^1 -z^{\star}\|_p}{c N}    \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .\label{eq:conv_proba}
\end{align}
{\bf Step 3.} (Restarts)\\
In this step we will employ the restart technique that is generalization of technique proposed in \cite{juditsky2014deterministic}.
Before we need to get a more compact convergence result in the form $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$. For this we fix $\sigma > 0$ and let $\tau$ be chosen as $\tau = \O\left(\e/M_2\right)$. If moreover Assumption \ref{ass:err_noise} holds true with $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$, then using \eqref{eq:conv_proba} we obtain 
 \begin{align}\label{restart:rate_prob}
     \Prob & \left\{ f\left( \hat x^{N_1},y^{\star}\right) -  f\left(x^{\star}, \hat y^{N_1} \right) = \widetilde \O_1\left(\ M_2 \sqrt{d}\frac{\|z^1 -z^{\star}\|_p }{\sqrt{N_1}}  \right)   \right\}  \geq 1 - \sigma_1.
 \end{align}
 We note that now the notation $\widetilde \O_1$ contains the factor $\log \sigma_1^{-1}$.
 
  For the l.h.s. of Eq. \eqref{restart:rate_prob} we use Assumption \ref{ass:strongly_convex} then with probability at least $1 - \sigma_1$ 
 \begin{align}\label{restart:norms_prob}
 \frac{\mu_{r}}{2} \underbrace{\|z^{N_1} - z^{\star}\|_p^{r}}_{R_1^r}
 &\leq
     f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right) = \widetilde \O\left(\ M_2 \sqrt{d}\frac{\|z^1 -z^{\star}\|_p }{\sqrt{N_1}} \right).
 \end{align}
 Then taking ${N_1}$ so as to reduce the distance to the solution by half, we obtain
 $$ {N_1} = \widetilde \O_1 \left( \frac{M_2^2 d}{\mu_{r}^2 R_1^{2(r-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ from a similar condition for reducing the distance $R_1$ to the solution by a factor of $2$, and so on.  We remind that at each restart step $i \in \{1,k\}$, the resulting formula \eqref{restart:norms_prob} is valid only with probability $1 - \sigma_i$. Thus, we choose $\sigma_i = \sigma/k$ and then by the union bound inequality all inequalities are satisfied simultaneously with probability at least $1 - \sigma$. We will determine the number of restarts further, but at this stage we use the fact that $k$ depends on the accuracy only logarithmically, which entails that $\forall i\in \{1,k\} \;\;  \widetilde \O_i = \widetilde \O$.
 
 Thus, after $k$ of such restarts, the total number of iterations will be
 \begin{align} \label{restart:N_prob}
     N_{acc} = N_1 +\dots + N_k = \widetilde \O \left(\frac{ 2^{2(r-1)}M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}}\left(1+2^{2(r-1)} + \dots + 2^{2(k-1)(r-1)}\right) \right).
 \end{align} 
 It remains for us to determine the number of restarts, for this we fix the desired accuracy in terms of $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$ and using the inequality \eqref{restart:norms_prob} we obtain 
 \begin{align}\label{restart:epsilon_prob}
     \hat{\e}_{\rm sad} = \widetilde \O \left(\frac{\mu_{r} R_k^{r}}{2}\right)=   \frac{ M_2 \sqrt{d} \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{r}R_0^{r}}{2^{kr}}\right) \leq \varepsilon.
 \end{align} 
 Then to fulfill this condition one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{r}R_0^{r}/\varepsilon\right)) / r$ and using Eq. \eqref{restart:N} we get the total number of iterations
\[ N_{acc} = \widetilde \O\left(\frac{2^{2k(r-1)}M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}} \right) = \widetilde \O\left(\frac{M_2^2 d}{\mu_{r}^{2/r} \varepsilon^{2(r-1)/r}} \right).\]
  


\end{proof}




==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/restarts_prob.tex <==
\section{Restarts and Linear Convergence Rate}\label{sec:rest}
In this section we apply restart-technique \cite{juditsky2014deterministic} to  Algorithm\ref{alg:zoSPA} in the case when we additionally have $r-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems). 
\begin{assumption}\label{ass:strongly_convex}
There is $r \geq 1$ and $\mu_{r} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
$$ \frac{\mu_{r}}{2} \|z-z^{\star}\|_p^{r} 
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right).
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
$$
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
Then for the output $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA},  the following holds for $ \e_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \e_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \e_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $a_q^2$ is such that $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, if Assumption \ref{ass:strongly_convex} is satisfied we can apply restarts and to achieve $\E[\e_{\rm sad}] \leq \varepsilon$ one need $N$ iterations where $N$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N &= \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right),\\
     N &\leq  \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right),
 \end{align}
 where $B$ is an inaccuracy associated with the $\tau$-smoothing and inexactness of the oracle. 
 Constants $A, B$ depend on noise conditions and are given by the following equality
 \begin{enumerate}
    \item under Assumption \ref{ass:err_noise} 
 \begin{align}\label{eq:err_noise_AB}
      A = \sqrt{2} M_{\rm case1}, \;\;\; B = {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2,
 \end{align}
    \item under Assumption \ref{ass:Lip_noise} 
    \begin{align}\label{eq:err_noise_AB_2}
      A = \sqrt{2} M_{\rm case2}, \;\;\; B = M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.
 \end{align}
\end{enumerate}
Thus, from \eqref{eq:err_noise_AB} $\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon^2/\left(\D M_2\sqrt{d}\right)\right)$ and from \eqref{eq:err_noise_AB_2}
$\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon/\left(\D\sqrt{d}\right)\right)$.
\end{theorem}

\begin{remark}
An important particular case of Theorem~\ref{th:conv_rate_restarts} is when $\gamma = 1$. Under this assumption the estimate on the number of iteration $\eqref{eq:estim_iter_restart}$ can be rewritten in the following form:
 \begin{align}
     N = \widetilde \O\left(\frac{64 \cdot A^2}{\mu_{1}^2 } \right) = \widetilde \O\left(\frac{A^2}{\mu_{1}^{2} } \right).
 \end{align}
As a result, it leads us to the linear convergence of the algorithm for non-smooth convex-concave saddle points problems with sharp saddle-point. For convex optimization problems with sharp minimum this effect was known \cite{juditsky1993stochastic}.
\end{remark}



%  \iffalse

\begin{proof}[Proof of the  Theorem \ref{th:conv_rate_restarts}]

The proof is based on the proof of Theorem~\ref{th:conv_rate_prob}. In the first $3$ steps, we obtain an estimate of type \eqref{eq:convergrate_prob} with a more detailed  dependence on the choice of the initial point $z_1$. Then we apply the restart technique to the obtained convergence rate.

By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) - \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2   \notag
\end{align}
Summing for $k=1,\dots,N$ we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE_prob:rst}
   \sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra 
   &\leq V_{z^1}(u)  - \sum_{k=1}^N\gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2  \notag\\
   &\leq  V_{z_1}(u) + \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_q^2.
\end{align}
where $z^1$ can be chosen in stochastic way.

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE_prob:rst}, invoking Assumtion \ref{ass:uni_Lip_obj}, the random variables $\phi_k = \gamma_k^2 \|g(z^k,\be^k,\xi^k)\|_q^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$ satisfy the premise of case B of Lemma 2 from \cite{lan2012validation} with $\sigma_k = 4 N^{2/q -1} M_2^2 \gamma_k^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$:
\begin{align*}
    & \E_{|t-1} \left[ \exp \{|\phi_k|/\sigma_k\} \right] = \E_{|t-1} \left[ \exp \{ \|g(z^k,\be^k,\xi^k)\|_q^2/4 N^{2/q -1} M_2^2\} \right] \leq  /* \mbox{ Holder's inequality} */ \\
    & \leq \E_{|t-1} \left[ \exp \{ 
    \|g(z^k,\be^k,\xi^k)\|_2^2/4M_2^2\} \right] \leq \exp \{1\}
\end{align*}

Invoking case B of Lemma 2 from \cite{lan2012validation}, we get
\small{
\begin{align}
    &\text{Prob} \left\{ \left| \sum_{k=1}^N \gamma_k^2 \|g(z^k,\be^k,\xi^k)\|_q^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1} \right| > \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } + \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } \right\} \nonumber \\
    & \hspace{8 cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} \label{eq:first_step_var:rst}
\end{align}}





{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE_prob:rst}, we provide the new definition of gradient approximation of $\nabla f(z, \xi)$ following the Eq. $\eqref{eq:grad_approx}$:
\begin{equation}\label{eq:grad_approx_f:rst}
    g_f(z,\xi, \be) = \frac{d}{2\tau}\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix},
\end{equation}

Using the notation \eqref{eq:grad_approx_f:rst} we rewrite the l.h.s. of  Eq. \eqref{eq:inmainsqE_prob:rst} as following:

\begin{align}
    &\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra =\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \nonumber\\
    & + \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra + \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra \label{eq:step2_rewriten:rst}
\end{align}
\begin{enumerate}
    \item For the first term in r.h.s. of  Eq. \eqref{eq:step2_rewriten:rst}, we use Assumption \ref{ass:uni_Lip_obj} and provide the following notions:
$$\sigma_k = \gamma_k M_2 2 \mathcal D,$$
$$\phi_k (\xi_k)= \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra .$$
Moreover, using the notion of $\omega$-diameter of $\Z$ we have that:
\begin{align*}
  \E_{|k-1} &\left[ \exp \left\{ \phi_k^2/ \sigma_k^2 \right\} \right] = \underbrace{\E_{|k-1} \left[ \exp \left\{ \left(\gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra \right)^2/ \left(  \gamma_k M_2 2 \mathcal D \right)^2 \right\} \right]}_{\leq \exp \{1\}}.  
\end{align*}
It follows by case A of Lemma 2 from \cite{lan2012validation} that
\begin{align}
    \text{Prob} \left\{ \left| \frac{\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra}{\sum_{k=1}^{N}\gamma_k}  \right| > \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} \right\} \leq 2 \exp \left\{ -\frac{\Omega^2}{3} \right\} . \label{eq:step2_martingale_rewriten:rst}
\end{align}
\item For the second term in r.h.s of Eq. \eqref{eq:step2_rewriten:rst} under the Assumption \ref{ass:err_noise} we obtain :
\begin{align}
    & \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra \geq - \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left|\la \be, z^k-u \ra \right| \label{eq:step2_delta_rewriten:rst}
\end{align}
Using the Poincaré's lemma from \cite{lifshits2012lectures} paragraph 6.3 we rewrite $\be$ in different form:
\begin{align}\label{eq:poincare_def_e:rst}
    \be \stackrel{D}{=} \frac{\eta}{\sqrt{\eta_1^2 + \dots + \eta_d^2}},
\end{align}

where $\eta = \left( \eta_1, \eta_2, \dots , \eta_d \right)^T = \mathcal{N} \left( 0 , I_d \right)$. 
Using Lemma 1 \cite{laurent2000adaptive}
% \cite{boucheron2013concentration} 
it follows:
\begin{align}
    \text{Prob} \left\{  \sum_{k=1}^d \left|\eta_k\right|^2 \le d -  2 \sqrt{\Omega d} \right\} \leq  \exp \{- \Omega \} . \label{eq:step2_sphere_rewriten:rst}
\end{align}
Using the definition of $\eta$ we obtain:
\begin{align}
    \la \eta, z^k-u \ra \stackrel{d}{=} \mathcal{N} \left( 0 , \|z^k - u\|^2 \right). \label{eq:step2_poincare:rst}
\end{align}
Using Eq. \eqref{eq:step2_sphere_rewriten:rst}, \eqref{eq:step2_poincare:rst} and \eqref{eq:poincare_def_e:rst} we can estimate the r.h.s of Eq. \eqref{eq:step2_delta_rewriten:rst}:
\begin{align}
    \text{Prob} &\left\{   \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left| \la \be, z^k-u \ra \right| > \frac{ \Omega \D \sqrt{d} \Delta \sum_{k=1}^N \gamma_k}{\tau} \right\} \nonumber\\
    &\leq 3 \exp \{-\Omega/4 \} . \label{eq:step2_sphere_rewriten_2:rst}
\end{align}
\item We rewrite the third term in r.h.s. of  Eq. \eqref{eq:step2_rewriten:rst} in the following form: 
\begin{align} 
    \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra & =  \sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra  \notag \\
     &=  \sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right) \notag \\
     &\geq  \sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y)) \notag \\
     &=  \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \label{eq:eqexpfxy_prob:rst}.
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE_prob:rst}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq  f^\tau\left(\frac{\sum_{k=1}^N \gamma_k x^k}{\sum_{k=1}^{N}\gamma_k},y\right)  - f^\tau\left(x, \frac{\sum_{k=1}^N \gamma_k y^k}{\sum_{k=1}^{N}\gamma_k}\right)\notag \\
     &=  f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE_prob}  for Eq. \eqref{eq:eqexpfxy_prob:rst} we get 
\begin{align}\label{eq:fpslff_prob:rst}
      \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra  
     &\geq  \sum_{k=1}^{N}\gamma_k \left( f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right) .
\end{align}
\end{enumerate}









{\bf Step 3.} \\
Then we use this with  Eq. \eqref{eq:step2_rewriten:rst}, \eqref{eq:step2_delta_rewriten} and \eqref{eq:fpslff_prob:rst} for Eq. \eqref{eq:inmainsqE_prob:rst} and obtain
\begin{align}
      &f^\tau\left( \hat x^N,y\right)   - f^\tau\left(x, \hat y^N \right)  \leq   \frac{\D^2}{\sum_{k=1}^{N}\gamma_k } + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_q^2  \nonumber \\
    & - \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \la \be, z^k-u \ra \label{eq:exEeqE_prob:rst}
\end{align}


 For the l.h.s. of Eq. \eqref{eq:exEeqE_prob:rst} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2 \label{eq:f_tau_to_f:rst}
 \end{align}
 Using Eq. \eqref{eq:f_tau_to_f:rst}, \eqref{eq:step2_martingale_rewriten:rst},  \eqref{eq:first_step_var:rst}, \eqref{eq:step2_sphere_rewriten_2:rst} and taking the maximum in $(x,y) \in (\X,\Y)$, we obtain we can rewrite Eq. \eqref{eq:exEeqE_prob:rst} as follow:
 
 \begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k }  \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
      & \hspace{3cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} + 3 \exp \{-\Omega/4 \}. \label{eq:dghjsklslsl_proba:rst}
\end{align}
%  \begin{align}
%       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } +\frac{d \D \Delta}{\tau} \right. \nonumber\\
%       & \left.+ \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
%       & \hspace{5cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} \label{eq:dghjsklslsl_proba}
% \end{align}

 Choosing the learning rate $\gamma_k 
=\frac{\D}{M}\sqrt{\frac{2}{N}}$ with $M^2 \triangleq (M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl_proba:rst} we obtain
\begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2}{M}   + \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
      & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 3 \exp \{-\Omega/4 \} 
\end{align}









 {\bf Step 5.} (Restart)
 At the previous step, we obtained the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq  \frac{A\sqrt{\E [V_{z^1}(z^{\star})]}}{\sqrt{N_1}}  + B,  
 \end{align}
 with an appropriate choice of constants $A, B$. Here $B$ is an inaccuracy associated with the stochastic setting of the problem and inexactness of the oracle. In this step we will employ the restart technique that is generalization of technique proposed in \cite{juditsky2014deterministic}.
 
 For the r.h.s. of Eq. \eqref{restart:rate} we use Assumption \ref{ass:strongly_convex} and the fact of remark 3 from \cite{gasnikov2018universal} that $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$ for the l.h.s 
 \begin{align}\label{restart:norms}
 \underbrace{\frac{\mu_{\gamma}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{\gamma}\right]}_{\geq\frac{\mu_{\gamma}}{2} \E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}
 \leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq A\widetilde \O(\underbrace{\E[\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}  + B.
 \end{align}
 Then by choosing ${N_1} \leq \frac{A^2\widetilde \O(R_0^2)}{B^2}$ and applying the Jensen inequality for l.h.s of Eq. \eqref{restart:norms} we get
 \begin{align}
 \frac{\mu_{\gamma}}{2} \underbrace{\E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}_{R_1^{\gamma}} \leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq 2A\widetilde \O(\underbrace{\E [\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}.
 \end{align}
 And finally taking ${N_1}$ so as to reduce the distance to the solution by half, we obtain
 $$ {N_1} = \widetilde \O \left( \frac{64A^2}{\mu_{\gamma}^2 R_1^{2(\gamma-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ from a similar condition for reducing the distance to the solution by a factor of $2$, and so on. 
 
 Thus, after $k$ of such restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N = N_1 +\dots + N_k = \widetilde \O \left(\frac{64 \cdot 2^{2(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}}\left(1+2^{2(\gamma-1)} + \dots + 2^{2(k-1)(\gamma-1)}\right) \right).
 \end{align} 
 It remains for us to determine the number of restarts, for this we fix the desired accuracy in terms of $\E[\e_{\rm sad}] \leq \varepsilon$ and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\e_{\rm sad}] = \widetilde \O \left(\frac{\mu_{\gamma} R_k^{\gamma}}{2}\right)=   \frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{\gamma}R_0^{\gamma}}{2^{k\gamma}}\right) \leq \varepsilon.
 \end{align} 
 Then to fulfill this condition one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{\gamma}R_0^{\gamma}/\varepsilon\right)) / \gamma$ and using Eq. \eqref{restart:N} we get the total number of iterations
 $$ N = \widetilde \O\left(\frac{64 \cdot 2^{2k(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}} \right) = \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right).$$
 Moreover, using ${N_k} \leq \frac{A^2\widetilde \O(R_{k-1}^2)}{B^2}$ and $\frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  \leq \varepsilon$ from Eq. \eqref{restart:epsilon} we have $B = \tilde{O}(\varepsilon)$.  This condition imposes restrictions on the final accuracy $\varepsilon$ and, as a consequence, on the choice of $N$, given by Eq. \eqref{restart:N}
 \begin{align*}
     N \leq  \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right).
 \end{align*}
\end{proof}




\begin{remark}
The estimations on the noise $B$ in Eq. \eqref{eq:err_noise_AB} and \eqref{eq:err_noise_AB_2} can be improved in the following way: it is possible to obtain the better evaluation on the r.h.s of Eq. \eqref{eq:sectermErhs_restarts} as
\begin{align}\label{eq:sectermErhs_restarts_new}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq {\|z^k - u\|_2}/{\sqrt{d}}. 
\end{align}
Choosing $u = (x^*, y^*)$ we provide exponentially decreasing sequence of $\D_2^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate}. It leads us to the more precise estimation on the noise $B$. We use this estimation on $B$ when we employ the restart technique in the proof of Theorem~\ref{th:conv_rate_restarts} and, thanks to this, we obtain the better estimate on the maximal level of noise: under Assumption \ref{ass:err_noise} $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{2-1/\gamma}}{M_2\sqrt{d}}$$  and 
under Assumption \ref{ass:Lip_noise} 
$$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{1-1/\gamma}}{\sqrt{d}}.$$
\end{remark}

\begin{remark}\label{hpb}
Based on high-probability bound from Appendix~\ref{H-PB} we can obtain high-probability bound by using the same restart-technique \cite{juditsky2014deterministic}. In the case $\gamma = 2$ it is probably possible to improve this bound in $\log \varepsilon^{-1}$ factor by using alternative algorithm \cite{harvey2019tight}. Moreover, based on stochastic-gradient clipping trick \cite{gorbunov2021near} we can obtain the result in Appendix~\ref{H-PB} in the case when the second moment of stochastic gradient is bounded (subgaussian tails are not required). When the variance of noise is not bounded (the second moment of stochastic gradient is non bounded) the rate of convergence may changes drastically, see the next section.
\end{remark}
% \fi



==> Gradient-Free Optimization for Non-Smooth Minimax Problems 2022/variable_separation.tex <==
\section{Variable Separation}
In this section, 
we assume  proximal setups for spaces $\X$ and $\Y$ can be different.  Thus,  
 we replace the proximal step  $z^{k+1}  \leftarrow {\rm Prox}_{z^k}\left(\gamma_k g(z^k, \xi^k, \be^k)\right)$ on the  space $\Z\triangleq \X \times \Y$ from Algorithm \ref{alg:zoSPA} by two proximal steps on spaces $\X$ and $\Y$:
\begin{align*}
    x^{k+1}  &\leftarrow {\rm Prox}_{x^k}\left(\gamma_k g_x(z^k, \xi^k, \be^k)\right),\\
    y^{k+1}  &\leftarrow {\rm Prox}_{y^k}\left(\gamma_k g_y(z^k, \xi^k, \be^k)\right).
\end{align*}
We also note that we have different Bregman divergence for each space $\X, \Y$ and the step is taken according to the corresponding divergence.



\begin{lemma}\label{lm:shamirEnabla:separated}
 For $g(z,\xi,\be)$ from \eqref{eq:grad_approx}, the following holds
 under Assumption \ref{ass:Lip_obj} 
 \begin{enumerate}
     \item  and Assumption  \ref{ass:err_noise}
     \[\E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} dM_2^2 + {d^2 a_{q_x}^2\Delta^2}{\tau^{-2}},\]
     \item  and Assumption \ref{ass:Lip_noise} 
\[\E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} d (M_2^2+M_{2,\delta}^2),\] 
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E_{\be_x} \left[ \|\be_x\|_{q_x}^4\right]} \leq a_{q_x}^2$.
\end{lemma}

\begin{proof}
\begin{align}\label{eq:sqnormE:separated}
    &\E \left[\|g_x(z,\xi,\be)\|^2_{q_x} \right] = \E\left[ \left\|\frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be_x\right\|^2_{q_x} \right] \notag \\
    &= \frac{d^2}{4\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right)^2 \right] \notag\\
     &= \frac{d^2}{4\tau^2}\left(\E \left[\|\be_x\|_{q_x}^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right] + \E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \right) 
\end{align}
For the first term in the r.h.s. of Eq. \eqref{eq:sqnormE:separated}, the following holds with an arbitrary parameter $\alpha$
\begin{align}\label{eq:fgkbbhgdddgh:separated}
 & \frac{d^2}{4\tau^2}\E \left[\|\be_x\|_{q_x}^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right]  \notag\\
  &= \frac{d^2}{2\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left((f(z+\tau \be,\xi) -\alpha) -(f(z-\tau \be,\xi) - \alpha)   \right)^2 \right] \notag\\
    &\leq \frac{d^2}{2\tau^2}\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 + (f(z-\tau \be,\xi) -\alpha)^2 \right] \quad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
     &=  \frac{d^2}{2\tau^2}\left(\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] + \E \left[\|\be_x\|_{q_x}^2(f(z-\tau \be,\xi) -\alpha)^2 \right] \right) \notag\\
    &= \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
\end{align}
Applying the Cauchy--Schwartz inequality for Eq. \eqref{eq:fgkbbhgdddgh:separated} and using $\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \leq a_{q_x}^2$ we obtain 
\begin{align}\label{eq:funcsq:separated}
     \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] 
     &\leq \frac{d^2}{\tau^2}\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \sqrt{\E \left[ f(z+\tau \be,\xi)-\alpha)^4\right]} \notag\\
     &\leq \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right] . 
\end{align}
Then we assume $\alpha = \E\left[f(z+\tau \be,\xi)\right]$, $\beta = \E\left[\delta(z+\tau \be)\right]$ and use Lemma \ref{lm:shamirLm9} along with the fact that $f(z+\tau\be,\xi)$ is $\tau M_2(\xi)$-Lipschitz continuous, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus, it holds for the Eq. \eqref{eq:funcsq:separated}  
\begin{align}\label{eq:finlhkjfsvn:separated}
    \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right]
    &\leq \frac{d^2 a_{q_x}^2}{\tau^2} \cdot c\frac{\tau^2 \E M_2^2(\xi)}{d} = c d a_{q_x}^2 M_2^2.  
    %\red{\text{it seems should be} \leq}
\end{align}
\begin{enumerate}
    \item Under the Assumption \ref{ass:err_noise}
     for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE:separated}, the following holds
    \begin{align}\label{eq:fgkssssffdgh:separated}
        &\frac{d^2}{4\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \leq  \frac{d^2\Delta^2}{\tau^2} \E \left[ \|\be_x\|_{q_x}^2  \right]\leq \frac{d^2 a_{q_x}^2\Delta^2}{\tau^2}.
    \end{align}
   % where we used $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$.
    \item Under the Assumption \ref{ass:Lip_noise}
    for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE:separated}, the following holds with an arbitrary parameter $\beta$
    \begin{align}\label{eq:fgklljgsdgh:separated}
        &\frac{d^2}{4\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \notag \\
     &= \frac{d^2}{2\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left((\delta(z+\tau\be) -\beta) -(\delta(z-\tau\be)  -\beta) \right)^2 \right] \notag\\
    &\leq \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left((\delta(z+\tau\be)-\beta)^2  +(\delta(z-\tau\be) -\beta)^2 \right) \right] \qquad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
    &= \frac{d^2}{2\tau^2}\left(\E \left[ \|\be_x\|_{q_x}^2 (\delta(z+\tau \be)-\beta)^2 \right] + \E \left[\|\be_x\|_{q_x}^2(\delta(z-\tau \be) -\beta)^2 \right] \right) \notag\\
    &= \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
    \end{align}
\end{enumerate}





and for the second term in the Eq. \eqref{eq:sqnormE:separated}, we get
\begin{align}\label{eq:noisesq:separated}
   \frac{d^2}{\tau^2}\E\left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]
   &\leq \frac{d^2}{\tau^2}\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \sqrt{\E \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \notag \\
   &\leq \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[ \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \right]
\end{align}

Then we assume  $\beta = \E\left[\delta(z+\tau \be)\right]$ and use Lemma \ref{lm:shamirLm9} together with the fact that $\delta(z+\tau\be)$ is $\tau M_{2,\delta}$-Lipschitz continuous, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus, Eq. \eqref{eq:noisesq:separated} can be rewritten as 
\begin{align}\label{eq:fkssoomnbd:separated}
    \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[ \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \right]
    &\leq \frac{d^2 a_{q_x}^2}{\tau^2}  \cdot c\frac{\tau^2  M_{2,\delta}^2}{d} \leq c a^2_{q_x} d M_{2,\delta}^2. 
    %\red{\text{it seems should be} \leq}
\end{align}

Using Eq. \eqref{eq:finlhkjfsvn:separated} and \eqref{eq:fgkssssffdgh:separated} (or Eq. \eqref{eq:fkssoomnbd:separated}) for Eq. \eqref{eq:sqnormE:separated}, we get the statement of the lemma.
\end{proof}







\begin{proof}[Proof of the  Theorem \ref{th:conv_rate}]
By the definitions 
$$x^{k+1}= {\rm Prox}_{x^k}\left(\gamma_k g_x(z^k,\be^k,\xi^k) \right),$$ 
$$y^{k+1}= {\rm Prox}_{y^k}\left(\gamma_k g_y(z^k,\be^k,\xi^k) \right)$$
we get  \cite{ben2001lectures}, for all $u = (x, y) \in \X \times \Y$
\begin{align}
   \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \leq V_{x^k}(x) - V_{x^{k+1}}(x) - \gamma_k^2\|g_x(z^k,\be^k,\xi^k)\|_{q_x}^2/2   \notag
\end{align}
\begin{align}
   \gamma_k\la g_y(z^k,\be^k,\xi^k), y^k-y\ra \leq V_{y^k}(y) - V_{y^{k+1}}(y) - \gamma_k^2\|g_y(z^k,\be^k,\xi^k)\|_{q_y}^2/2   \notag
\end{align}
where $V_x, V_y$ are Bregman divergences in $\X$ and $\Y$ spaces respectively.
Summing for $k=1,\dots,N$  and taking the expectation, we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE:separated}
   \E\left[\sum_{k=1}^N \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \right]
   &\leq V_{x^1}(x)  - \E\left[\sum_{k=1}^N\gamma_k^2\|g_x(z^k,\be^k,\xi^k)\|_{q_x}^2/2 \right] \notag\\
   &\leq  \D_x^2 + \sum_{k=1}^N \frac{\gamma_k^2}{2} \E\left[\|g_x(z^k,\be^k,\xi^k)\|_{q_x}^2\right], 
\end{align}
\begin{align}\label{eq:inmainsqE_y:separated}
   \E\left[\sum_{k=1}^N \gamma_k\la g_y(z^k,\be^k,\xi^k), y^k-y\ra \right]
   &\leq V_{y^1}(y)  - \E\left[\sum_{k=1}^N\gamma_k^2\|g_y(z^k,\be^k,\xi^k)\|_{q_y}^2/2 \right] \notag\\
   &\leq  \D_y^2 + \sum_{k=1}^N \frac{\gamma_k^2}{2} \E\left[\|g_y(z^k,\be^k,\xi^k)\|_{q_y}^2\right], 
\end{align}
where $\mathcal D_x = \max_{x, \xi\in \X}\sqrt{2V_{x}(\xi)}$, $\mathcal D_x = \max_{y , \zeta \in \Y}\sqrt{2V_{y}(\zeta)}$ are the diameters  of $\X, \Y$. In what follows, we deal only with the variable $x$, taking into account the fact that the calculations for the other variable are similar.

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE:separated} we use Lemma \ref{lm:shamirEnabla:separated} and obtain
 \begin{enumerate}
     \item  under Assumption  \ref{ass:err_noise}
     \begin{equation}\label{eq:inmainsqEtwo1:separated}
        \E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} dM_2^2 + \frac{d^2 a_{q_x}^2\Delta^2}{\tau^2}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo:separated}
    \E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} d (M_2^2+M_{2,\delta}^2),
\end{align}
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \leq a_{q_x}^2$.

{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE:separated}, we use Lemma \ref{lm:expecapproxgrad}


 \begin{enumerate}
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz11:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \right] &=  \E\left[\sum_{k=1}^N \gamma_k\la \E\left[g_x(z^k,\be^k,\xi^k)\mid z^k \right], x^k-x\ra \right] \notag\\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k\left\la \nabla_x f^\tau(z^k) - \frac{d\Delta}{\tau}  \be^k_x, x^k-x\right\ra \right].
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \right] &=  \E\left[\sum_{k=1}^N \gamma_k\la \E\left[g_x(z^k,\be^k,\xi^k)\mid z^k \right], x^k-x\ra \right] \notag\\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(z^k) - dM_{2,\delta} \be^k_x, x^k-x\ra \right].
\end{align}
 \end{enumerate}



For the first term of the r.h.s. of Eq.\eqref{eq:eqrefeqffxyz11:separated} and \eqref{eq:eqrefeqffxyz:separated} we have 
\begin{align}\label{eq:eqexpfxy:separated_x}
     \E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(z^k), x^k-x\ra \right]
     &=  \E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(x^k,y^k), x^k-x \ra\right] \notag \\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))\right].
\end{align}
By exactly the same calculations, we get the inequality for dual variable $y$
\begin{align}\label{eq:eqexpfxy:separated_y}
     \E\left[\sum_{k=1}^N \gamma_k\la \nabla_y f^\tau(z^k), y^k-y\ra \right]
     &=  \E\left[\sum_{k=1}^N \gamma_k\la -\nabla_y f^\tau(x^k,y^k), y^k-y \ra\right] \notag \\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k (  - f^\tau(x^k,y^k) + f^\tau(x^k,y))\right]. 
\end{align}

Summing up the inequalities \eqref{eq:eqexpfxy:separated} and \eqref{eq:eqexpfxy:separated_y} we have
\begin{align}\label{eq:eqexpfxy:separated}
\E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(z^k), x^k-x\ra \right] \notag &+ \E\left[\sum_{k=1}^N \gamma_k\la \nabla_y f^\tau(z^k), y^k-y\ra \right] \notag \\
&\geq \E\left[\sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \right].
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE:separated}
     &\E\left[\frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \right] \notag \\
     &\hspace{2cm}\leq \E\left[ f^\tau\left(\frac{1}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \gamma_k x^k,y\right)  - f^\tau\left(x, \frac{1}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \gamma_k y^k\right) \right]\notag \\
     &\hspace{2cm}= \E\left[ f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right],
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm. 
Using Eq. \eqref{eq:fineqE:separated}  for Eq. \eqref{eq:eqexpfxy:separated} we get 
\begin{align}\label{eq:fpslff:separated}
      \E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right] 
     &\geq \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right].
\end{align}
Next we estimate the term $\E_{\be_x^k} \left[   \left| \la \be_x^k, x^k-x\ra \right| \right] $ in Eq. \eqref{eq:eqrefeqffxyz11:separated} and \eqref{eq:eqrefeqffxyz:separated}  by the Lemma  \ref{lm:dotprodvece}  
\begin{align}\label{eq:sectermErhs:separated}
  \E_{\be_x^k} \left[    \left|\la \be_x^k, x^k-x\ra \right| \right] \leq  \frac{\D_x}{\sqrt{d_x}},
\end{align}
and similarly 
\begin{align}\label{eq:sectermErhs:separated_y}
  \E_{\be_x^k} \left[   \left| \la \be_y^k, y^k-y\ra \right| \right] \leq  \frac{\D_y}{\sqrt{d_y}}.
\end{align}
Now  we substitute  Eq. \eqref{eq:fpslff:separated}, \eqref{eq:sectermErhs:separated_y} and  \eqref{eq:sectermErhs:separated} to Eq. \eqref{eq:eqrefeqffxyz11:separated} and \eqref{eq:eqrefeqffxyz:separated} summed with similar ones for the variable $y$, and get
 \begin{enumerate}
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz1122:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] &\geq 
     \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)- f^\tau\left(x, \hat y^N \right) \right] \notag \\ 
     &-  \sum_{k=1}^N \gamma_k \Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right).  
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz22:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] &\geq  \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right) - f^\tau\left(x, \hat y^N \right) \right] \notag\\
     &- \sum_{k=1}^N \gamma_k M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right). 
\end{align}
 \end{enumerate}
 
{\bf Step 3.} (under Assumption \ref{ass:err_noise}) \\
Now we combine Eq. \eqref{eq:eqrefeqffxyz1122:separated}   with  Eq. \eqref{eq:inmainsqEtwo1:separated} for sum of Eq. \eqref{eq:inmainsqE:separated}, \eqref{eq:inmainsqE_y:separated} and obtain under Assumption \ref{ass:err_noise} the following
     \begin{align}\label{eq:inmainsqEtwo133:separated}
     &\sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
     -  \sum_{k=1}^N \gamma_k \Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)  \notag \\
     &\leq \D_x^2 + \D_y^2 +  \sum_{k=1}^N \frac{\gamma_k^2}{2} \left(c a^2_{q_x} dM_2^2 + c a^2_{q_y} dM_2^2 + \frac{d^2 a_{q_x}^2\Delta^2}{\tau^2} + \frac{d^2 a_{q_y}^2\Delta^2}{\tau^2}\right).
     \end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE1:separated}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      \leq 
     \frac{ \D^2}{\sum_{k=1}^{N}\gamma_k}
      &+\frac{c (a^2_{q_x}+a^2_{q_y}) dM_2^2+ d^2 (a^2_{q_x}+a^2_{q_y})\Delta^2\tau^{-2}}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  \notag\\
      &+\Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right).
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE1:separated} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE1:separated} and   taking $(x,y) = (x_*,y_*)$
%  the maximum in $(x,y) \in (\X,\Y)$,
 we obtain
 \begin{align}\label{eq:dghjsklslsl1:separated}
     \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
     &\leq \frac{ \D^2+ (c d M_2^2 +
     d^2\Delta^2\tau^{-2}) (a^2_{q_x}+a^2_{q_y})
    \sum_{k=1}^{N} {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
       \notag \\
    &+ \Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Choosing the learning rate $\gamma_k 
=\frac{\D}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq (c d M_2^2 +
     d^2\Delta^2\tau^{-2}) (a^2_{q_x}+a^2_{q_y})$ in Eq. \eqref{eq:dghjsklslsl1:separated} we obtain
 \begin{align*}
      \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
     &\leq  
     %\frac{\D(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\D
     + \Delta\left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 4.} (under Assumption \ref{ass:Lip_noise})\\
Now we combine Eq.  \eqref{eq:eqrefeqffxyz22:separated}  with  Eq.  \eqref{eq:inmainsqEtwo:separated} for sum of Eq. \eqref{eq:inmainsqE:separated}, \eqref{eq:inmainsqE_y:separated} and obtain under Assumption \ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo334:separated}
    \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
    &- \sum_{k=1}^N \gamma_k M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)\notag \\ &\leq \D^2 
    +  \sum_{k=1}^N \frac{\gamma_k^2}{2} c (a^2_{q_x} + a^2_{q_y}) d (M_2^2+M_{2,\delta}^2).
\end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE:separated}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      &\leq 
     \frac{ \D^2}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c (a^2_{q_x} + a^2_{q_y}) d (M_2^2+M_{2,\delta}^2)}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2} \notag \\ &+ M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right). 
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE:separated} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE:separated} and   taking $(x,y) =(x_*,y_*)$
%  the maximum in $(x,y) \in (\X,\Y)$,
 we obtain
 \begin{align}\label{eq:dghjsklslsl:separated}
     \E\left[ 
    %  \max_{y \in \Y}
     f\left( \hat x^N,y_*\right) -  
    %  \min_{x\in \X}
     f\left(x_*, \hat y^N \right)\right]
     &\leq \frac{ \D^2+ c (a^2_{q_x} + a^2_{q_y}) d (M_2^2+M_{2,\delta}^2)\sum_{k=1}^N {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
    \notag \\&+ M_{2,\delta}  \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align}
 Choosing the learning rate 
%   $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$  in Eq. \eqref{eq:dghjsklslsl} we obtain
%  \begin{align*}
%       \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
%      &\leq  \frac{\D(1+c a^2_q d M_2^2 + c a^2_q dM_{2,\delta}^2)}{\sqrt{2N}M}  + M_{2,\delta} \D \sqrt{d} 
%      +  2\tau M_2.  
%  \end{align*}
 $\gamma_k 
=\frac{\D}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d (a^2_{q_x} + a^2_{q_y})(M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl1:separated} we obtain
 \begin{align*}
      \E\left[ 
    %   \max_{y \in \Y} 
      f\left( \hat x^N,y_*\right) - 
    %   \min_{x\in \X} 
      f\left(x_*, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\D  + M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align*}
\end{proof}


==> gas_upper.tex <==
\section{``Upper'' bound in the case of Lipschitz noise}
Now let us consider a stochastic convex optimization problem of the form
\begin{equation}\label{eq:conv_prob}
    \min_{x \in \X} F(x) \triangleq \mathds{E}_{\xi} f(x,\xi),
\end{equation}
where  $X \subseteq \R^{d}$ is a convex set, and for all $\xi$, $f(x,\xi)$ is convex in $x\in\X$  and satisfies Assumption \ref{ass:Lip_obj}. The empirical counterpart of this problem \eqref{eq:conv_prob} is
% for all $\xi$ 
%and for all $x,y \in \X$, $\xi$
% \begin{equation}\label{M}
%      \left|f(y,\xi) - f(x,\xi)\right| \le M_2 \|y-x\|_2.
% \end{equation}
% where $p\ge 1$.  
% Consider Monte Carlo (also known as Sample Average Approximation) approach for \eqref{eq:conv_prob} \cite{shapiro2021lectures}:
\begin{equation}\label{emp_prob}
    \min_{x \in \X} \hat{F}(x)\triangleq \frac{1}{N}\displaystyle\sum_{k = 1}^{N} f(x, \xi^k).
\end{equation}
The exact solution ($\nicefrac{\e}{2}$-solution)  of \eqref{emp_prob} is an $\e$-solution of \eqref{eq:conv_prob} if the sample size $N$ is taken as follows  \cite{shapiro2005complexity,feldman2016generalization}
\begin{equation}\label{LB}
   N=\widetilde{ \Omega}\left(d {M_2^2 \D_2^2}/{\e^{2}}\right),
\end{equation}
where $\D_2$ is the diameter of $X$ in the $\ell_2$-norm. This lower bound is tight \cite{shapiro2005complexity,shapiro2021lectures}.

On the other hand,  $\hat{F}(x)$ from \eqref{emp_prob} can be considered as an inexact zeroth-order oracle for $F(x)$ from \eqref{eq:conv_prob}. If $\delta(x) = F(x) - \hat{F}(x)$ then  in $\text{Poly}\left(d,1/\e\right)$ points $y,x$ with probability $1 - \beta$ the following holds 
$$\left|\delta(y) - \delta(x)\right| = \O\left(\frac{M_2\|y-x\|_2}{\sqrt{N}}\ln\left(\frac{\text{Poly}\left(d,1/\e\right)}{\beta}\right)\right)= \widetilde{\O}\left(\frac{M_2\|y-x\|_2}{\sqrt{N}}\right),$$
i.e., $\delta(x)$ is a Lipschitz function with Lipschitz constant 
\begin{equation}\label{delta}
    {M_{2,\delta}} = \widetilde{\O}\left({M_2}/{\sqrt{N}}\right).
\end{equation}

Let us assume there exists a zeroth-order algorithm that can solve \eqref{eq:conv_prob} with accuracy  $\e$ in $\text{Poly}\left(d,1/\e\right)$ oracle calls, where an oracle returns an inexact value of $F(x)$ with a noise that has the following Lipschitz constant 
$$M_{2,\delta}  \gg \frac{\e}{\D_2\sqrt{d}}.$$ 
We can use this algorithm to solve problem \eqref{eq:conv_prob} with $N$ determines from (see \eqref{delta})
$$\frac{M_2}{\sqrt{N}} \gg \frac{\e}{\D_2\sqrt{d}},$$
i.e.
$$N \ll d{M_2^2 \D_2^2}/{\e^2},$$
that contradicts  the lower bound \eqref{LB}. 

Thereby it is impossible in general to solve with accuracy $\e$ (in function value) Lipschitz convex  optimization problem via $\text{Poly}\left(d,1/\e\right)$ inexact zero-order oracle calls if Lipschitz constant of noise is greater than  
\begin{equation}\label{LBN}
   {\e}/({\D_2\sqrt{d}}).
\end{equation}

Unfortunately, we obtain this upper bound assuming that $\text{Poly}\left(d,1/\e\right)$ points were chosen regardless of $\left\{\xi^k\right\}_{k=1}^N$. That is not the case for the most of practical algorithms, in particular, considered above. But the dependence of these points from $\left\{\xi^k\right\}_{k=1}^N$ is significantly weakened by randomization we use in zero-order methods. So we may expect that nevertheless this upper bound still takes place. 

For arbitrary $\text{Poly}\left(d,1/\e\right)$ points (possibly that could depend on $\left\{\xi^k\right\}_{k=1}^N$) we can guarantee only (see \cite{shapiro2021lectures})
\begin{equation}\label{delta_}
    M_{2,\delta}  = \widetilde{\O}\left(\sqrt{d}{M_2}/{\sqrt{N}}\right).
\end{equation}
That is large than \eqref{delta}. Consequently, the upper bound \eqref{LBN} should be 
rewritten as
\begin{equation}\label{LBN_}
    {\e}/{\D_2}.
\end{equation}

We believe that \eqref{LBN_} is not tight upper bound, rather than \eqref{LBN}. That is, there exists algorithm (see Algorithm \ref{alg:zoSPA}) that can solve \eqref{eq:conv_prob} with accuracy $\e$ (in function value) via $\simeq dM_2^2\D_2^2/\e^2$ inexact zero-order oracle calls if Lipschitz constant of noise is bounded from above by $M_{2,\delta}  \lesssim \e/(\D_2\sqrt{d})$. But there are no algorithms reaching the same accuracy $\e$ by using $\text{Poly}\left(d,1/\e\right)$ inexact zero-order oracle calls if Lipschitz constant of noise is bounded from above by $M_{2,\delta}  \gg \e/(\D_2\sqrt{d})$, in particular, for $M_{2,\delta} $ given by \eqref{LBN_}.

Note, that \eqref{LB} holds  also if $f(x,\xi)$ has Lipschitz $x$-gradient \cite{feldman2016generalization}. So we can expect that obtained above lower bounds take place also for smooth problems. Known maximal level of noise bounds for concrete algorithms confirm this \cite{gasnikov2017stochastic,berahas2021theoretical,vasin2021stopping}.

==> intro_main.tex <==
\section{Introduction}\label{sec:intro}
In this paper, we consider a stochastic non-smooth \textit{saddle point} problem of the form
\begin{equation}\label{eq:min_max_problem}
    \min_{x\in \X} \max_{y\in \Y} ~f(x,y),
\end{equation}
where $f(x,y) \triangleq \E_\xi \left[f(x,y,\xi)\right]$ is the expectation, w.r.t. $\xi \in \Xi$,  $f: \X \times\Y \to \R $   is convex-concave and Lipschitz continuous, and  $\X \subseteq \R^{d_x}$, $\Y \subseteq \R^{d_y}$ are  convex compact sets. We will denote $z_* = (x_*,y_*)$ a solution of the problem \eqref{eq:min_max_problem}. The standard interpretation of such min-max problems is the antagonistic game between a learner and an adversary, where the equilibria are the saddle points  \cite{neumann1928theorie}.
Now the interest in   saddle point problems 
is renewed due to the popularity of generative adversarial networks (GANs), whose training involves solving  min-max problems \cite{goodfellow2014generative,chen2017zoo}. 

Motivated by  many applications in the field of  reinforcement learning \cite{choromanski2018structured,mania2018simple} and statistics,  where only a  black-box access to the function values of the objective is available, we consider \textit{zeroth-order} oracle (also known as gradient-free oracle).  Particularly, we mention the classical problem of adversarial multi-armed bandit \cite{flaxman2004online,bartlett2008high,bubeck2012regret}, where a learner receives a feedback  given by the function evaluations from an adversary. Thus, zeroth-order methods  \cite{conn2009introduction}  are the workhorse technique when the    gradient information is prohibitively expensive or even  not available and optimization is performed based only on the function evaluations.


\paragraph{Related Work and Contribution.}

Zeroth-order methods in the non-smooth setup were developed in a wide range of works  \cite{polyak1987introduction,spall2003introduction,conn2009introduction,duchi2015optimal,shamir2017optimal,nesterov2017random,gasnikov2017stochastic,beznosikov2020gradient,gasnikov2022power}.  Particularly, in \cite{shamir2017optimal}, an optimal algorithm  was provided as an improvement to the work \cite{duchi2015optimal} for a non-smooth case but Lipschitz continuous  in stochastic convex optimization problems.
However, this algorithm uses the exact function evaluations that can be infeasible in some applications. 
Indeed, an objective $f(z,\xi)$    can be not directly observed but instead, its noisy approximation $\vp(z,\xi) \triangleq f(z,\xi) + \delta(z)$ can be queried, where $\delta(z)$ is some adversarial noise.
This noisy-corrupted setup was considered in
many works \dd{\cite{polyak1987introduction,granichin2003randomized}}, however, such an algorithm that is optimal in terms of the number of oracle calls complexity and the maximum value of adversarial noise has not been proposed.
For instance,   in \cite{bayandina2018gradient,beznosikov2020gradient},  optimal algorithms in terms of oracle calls complexity were proposed, however, they are not optimal in terms of the maximum value of the noise. 
%Namely, the bounds contain non-optimal term $1/d$ and$1/\sqrt{d}$  respectively, where  $d \triangleq d_x + d_y$ is the problem size.
 In papers \cite{risteski2016algorithms,vasin2021stopping},   algorithms are optimal in terms of the maximum value of the noise, however, they are not optimal in terms of the oracle calls complexity.  
In this paper, we provide an accurate analysis of a gradient-free version of the mirror descent method with an inexact oracle that shows that  the method is optimal both in terms of the inexact  oracle calls complexity and the maximum admissible noise.  We consider two possible scenarios for the nature of the adversarial noise arising in different applications: the noise is bounded by a small value or  is Lipschitz.  Table \ref{Table1} demonstrates our contribution by comparing our results with the existing optimal bounds. Finally, we consider the case when the objective satisfies the $\gamma$-growth condition and restate the results.



\begin{table}[!h]
   \centering
    \small
    \vspace{-0.3cm}
    \caption{Summary of the Contribution}
    \label{Table1}
    \begin{threeparttable}
    \begin{tabular}{|c|c|c|c|c|c|}
         \hline
         \scriptsize \textsc{Paper} 
        %&\begin{tabular}{c}\bf Supports \\ \bf distributed \\ \bf setup? \end{tabular}
        & \begin{tabular}{c} 
        %  \scriptsize \textsc{$\min$}
        % \scriptsize \textsc{or} \\ 
        %   \scriptsize \textsc{ $\mathbf  \min\max$ }
          \scriptsize \textsc{Problem}\tnote{{\color{blue}(1)}}
        \end{tabular} 
        & \begin{tabular}{c}
      \scriptsize \textsc{Expectation}  \\ 
        \scriptsize \textsc{or Large } \\
          \scriptsize \textsc{ Deviation }
        \end{tabular}  
        & \begin{tabular}{c}
      \scriptsize \textsc{Is the  Noise} \\ 
      \scriptsize \textsc{Lipschitz?}
        \end{tabular} 
         & \begin{tabular}{c}
         \scriptsize \textsc{Number of} \\  \scriptsize \textsc{Oracle Calls} \\ 
        \end{tabular} 
            & \begin{tabular}{c}
      \scriptsize \textsc{Maximum Noise}  
        \end{tabular} \\
    \hline\hline
% \tiny{\citet{gasnikov2017stochastic}}\tnote{{\color{blue}(1)}}  & 
%   \scriptsize{ convex optimization} & $\E$ & \xmark &  $\nicefrac{n}{\e^2}$ & $\min\left\{ \nicefrac{\e^{3/2}}{\sqrt{n}}, \nicefrac{\e}{n}\right\}$\\
  %%%%%%%             
\tiny{\citet{bayandina2018gradient}}   &   \scriptsize{ convex}  & $\E$& \xmark   &   $\nicefrac{d}{\e^2}$ & $\nicefrac{\e^2}{d^{3/2}}$\\   
  %%%%%%%     
    \tiny{\citet{beznosikov2020gradient}}   &   \scriptsize{ saddle point} & $\E$ & \xmark  &  $\nicefrac{d}{\e^2}$ & $\nicefrac{\e^2}{d}$\\ 
    %%%%%%%    
    \tiny{\citet{vasin2021stopping}}   &   \scriptsize{ convex} & $\E$ & \xmark   &  ${\rm Poly}\left(d, \nicefrac{1}{\e}\right)$ & $\nicefrac{\e^2}{\sqrt d}$\\\ 
%%%%%%%    
 
\tiny{\citet{risteski2016algorithms}}   &   \scriptsize{ convex} & $\E$ & \xmark   & $ {\rm Poly}\left(d, \nicefrac{1}{\e}\right)$ & $\max\left\{ \nicefrac{\e^{2}}{\sqrt{d}}, \nicefrac{\e}{d}\right\}$\tnote{{\color{blue}(2)}}~ ~\\ 
%%%%%%%      
    \hline
    { \scriptsize \textsc{ This work}}     &  \scriptsize{  saddle point}  &  $\E$~ and ~$\Prob$ & \xmark   & $\nicefrac{d}{\e^2}$ & $\nicefrac{\e^2}{\sqrt d}$\\    
    
       { \scriptsize \textsc{This work}}     &  \scriptsize{  saddle point}   & $\E$~ and ~$\Prob$ & \cmark  & $\nicefrac{d}{\e^2}$ & $\nicefrac{\e}{\sqrt d}$\tnote{{\color{blue}(3)}} \\    
      \hline
    \end{tabular} 
    
    %%%%%%%%%%%
\begin{tablenotes}
{\scriptsize
 \item[{\color{blue}(1)}] The results obtained for saddle point problems are also valid for convex optimization problems.
}\\
 {\scriptsize
 \item[{\color{blue}(2)}] Notice, that this bound (up to a logarithmic factor) is also an upper bound for maximum possible value of noise. It is  important to note, that $ \e/d\lesssim \e^2/\sqrt{d}$, when $\e^{-2}\lesssim d$. That is in the large-dimension regime, when subgradient method is better than center of gravity types methods \cite{nemirovskij1983problem}, the upper bound on the value of admissible noise (that allows one to solve the problem with accuracy $\e$) will be $\e^2/\sqrt{d}$. 
}

{\scriptsize
 \item[{\color{blue}(3)}] This estimate is for the Lipschitz constant of the noise and  it possibly is tight. However,  we prove that the upper bound (possibly not tight) for the Lipschitz-noise constant is $\e$ (see Appendix~\ref{app:upperbound} for details).
}
\end{tablenotes}    
\end{threeparttable}

\end{table}

% \paragraph{Contribution.} 


% \begin{itemize}[leftmargin=*]
%   \setlength\itemsep{-0.2em}
%     \item 
%     \item
%     \item
% \end{itemize}

 \vspace{-0.2cm}
\paragraph{Paper Organization.} This paper is organized as follows. In Section \ref{sec:prelim}, we begin with background material, notation, and assumptions.   In Section \ref{sec:mainthero}, we present  the main results of the paper: the algorithm and the analysis of its convergence. 
In Section \ref{sec:rest}, we consider  an additional assumption of $\gamma$-growth condition and restate the results.
%In Section \ref{sec:generalization}, we give some possible generalizations for our results. 
In Section \ref{sec:auxiliarylemmas}, we provide some of the key technical components used to prove the main results from Section \ref{sec:mainthero}.  

\section{Preliminaries: Notation, Setup and Assumptions}\label{sec:prelim}
In this section, we give some key notation, background material and assumptions.

\paragraph{Notation.} We use $\la x,y\ra \triangleq \sum_{i=1}^d x_i y_i$ to define the inner product of $x,y \in \R^d$, where $x_i$ is
  the $i$-th component of $x$. By  norm  $\|\cdot\|_p$ we mean  the $\ell_p$-norm. Then the dual norm of the norm $\|\cdot\|_p$ is $\|\lm\|_q \triangleq \max\{\la x,\lm \ra \mid \|x\|_p \leq 1 \} $. Operator $\E[\cdot]$  is the full  expectation and operator $\E_{\xi}[\cdot]$ is the conditional expectation, w.r.t. $\xi$.   
  
  
  
\paragraph{Setup.}
Let us introduce the embedding space $\Z \triangleq \X \times \Y$, and then  some $z\in \Z$ means $z \triangleq (x,y)$, where $x\in \X, y \in \Y$.
% Let us introduce the embedding space $\Z = \X \times \Y$ and introduce functions $f(z)$ and $f(z,\xi)$ by rewriting the objectives from Eq. \eqref{eq:min_max_problem} as follows
% \[
% f(z)\triangleq f(x,y) 
% \]
% where $z \triangleq (x,y) \in \Z$ and $x\in \X, y \in \Y$.
On this embedding space, we introduce  the $\ell_p$-norm
and  a prox-function $\omega(z)$ compatible with this norm. Then we define the  Bregman divergence associated with $\omega(z)$ as
\[V_z( v) \triangleq \omega(z) -\omega(v) - \la  \nabla \omega(v), z - v \ra \geq \|z-v\|_p^2/2, \quad \mbox{ for all } z,v \in Z.\] 
We also introduce a prox-operator as follows
\[ {\rm Prox}_z(\xi) \triangleq \arg\min_{v\in Z} \left(V_z(v) + \la \xi, v \ra\right), \quad \mbox{ for all } z \in Z.\]
Finally, we denote the $\omega$-diameter  of $\Z$ by 
$\D \triangleq \max\limits_{z,v\in \Z}\sqrt{2V_{z}(v)}= \widetilde{\O}\left(\max\limits_{z,v\in \Z}\|z-v\|_p\right)$. Here $\widetilde \O\left(\cdot\right)$ is $\O\left(\cdot\right)$ up to a $\sqrt{\log d}$-factor.




\begin{assumption}[Lischitz continuity of the objective]\label{ass:Lip_obj}
%  Function $f(x,y)$ is $M_x$-Lipschitz continuous w.r.t. $x\in \X$ and $M_y$-Lipschitz continuous w.r.t. $y\in \Y$, i.e., 
%  \begin{align*}
%      |f(x_1,\cdot)- f(x_2,\cdot)| &\leq M_x \|x_1- x_2\|_p, \quad \mbox{ for all } x_1,x_2\in \X,\\
%      |f(\cdot, y_1)- f(\cdot,y_2)| &\leq M_y \|y_1- y_2\|_p, \quad \mbox{ for all } y_1,y_2 \in \Y.
%  \end{align*}
 Function $f(z,\xi)$ is $M_2$-Lipschitz continuous in $z\in \Z$ w.r.t. the $\ell_2$-norm, i.e.,   for all  $z_1,z_2\in \Z$ and $\xi \in \Xi$, 
 \[|f(z_1, \xi)- f(z_2,\xi)| \leq M_2(\xi) \|z_1- z_2\|_2.\] 
 Moreover, there exists a positive constant $ M_2$ such that  $\E\left[M^2_2(\xi)\right] \leq M_2^2$.
%  \begin{align*}
%      |f(z_1)- f(z_2)| &\leq M_2 \|z_1- z_2\|_2, \quad \mbox{ for all } z_1,z_2\in \Z.
%  \end{align*}
\end{assumption}



\begin{assumption}\label{ass:err_noise}
For all  $z \in \Z$, it holds $|\delta(z)| \leq \Delta.$
\end{assumption}


\begin{assumption}[Lischitz continuity of the noise]\label{ass:Lip_noise}
Function $\delta(z)$ is $M_{2,\delta}$-Lipschitz continuous in $z\in \Z$ w.r.t. the $\ell_2$-norm, i.e., for all $z_1, z_2 \in \Z$, \[|\delta(z_1)- \delta(z_2)| \leq M_{2,\delta} \|z_1- z_2\|_2.\]
\end{assumption}





% The smoothing was introduced so that for a smoothed problem  it was possible to obtain an unbiased estimate of the subgradient.






\section{Main Results}\label{sec:mainthero}
In this section, we present one of the main results of the paper. For problem \eqref{eq:min_max_problem}, we present an
algorithm (see Algorithm \ref{alg:zoSPA}) that is optimal in terms of the number of inexact zeroth-order oracle calls and the maximum adversarial noise.  The algorithm  is based on a gradient-free version of the stochastic  mirror descent (SMD) \cite{ben2001lectures}. 

\paragraph{Black-box oracle.} We assume that we can query   zeroth-order oracle corrupted by an adversarial noise $\delta(z)$: 
\begin{equation}\label{eq:zerothorder}
    \vp(z,\xi) \triangleq f(z,\xi) + \delta(z).
\end{equation}
We will consider two cases:
\begin{enumerate}[leftmargin=*]
   \setlength\itemsep{-0.1em}
    \item Noise $\delta(z)$ is bounded (Assumption \ref{ass:err_noise})
    \item Noise $\delta(z)$ is Lipschitz (Assumption \ref{ass:Lip_noise})
\end{enumerate}
% Here $f(z,\xi)$ is the objective in the problem \eqref{eq:min_max_problem}.
% \paragraph{Zeroth-order oracle.}
% We assume that we can query biased zeroth-order oracle returning  \[\vp(z,\xi) \triangleq f(z,\xi) + \delta(z),\]
% where random variable $\xi$ is responsible for  unbiased stochastic noise and $\delta(z)$ is biased deterministic noise



\paragraph{Gradient approximation.}  The gradient of $\vp(z,\xi)$ from \eqref{eq:zerothorder}, w.r.t. $z$, can be approximated by the function evaluations in two random points closed to $z$. To do so, we define  vector $\be$ picked uniformly at random from the Euclidean unit sphere $\{\be:\|\be\|_2= 1\}$. Let $\be \triangleq (\be_x^\top, -\be_y^\top)^\top$, where ${\rm dim}(\be_x) \triangleq d_x$, ${\rm dim}(\be_y) \triangleq d_y$ and ${\rm dim}(\be) \triangleq d = d_x+d_y$. Then the gradient  of $ \vp(z,\xi)$ can be estimated by the following approximation with a  small variance \cite{shamir2017optimal}:
\begin{equation}\label{eq:grad_approx}
    g(z,\xi, \be) = \frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix},
\end{equation}
where $\tau$ is some constant. 
% In the one-dimensional ($d=1$), the estimate \eqref{eq:grad_approx} is trivial:
% when $\vp(z,\xi)$ is differentiable at $z$ and $\tau$  is sufficiently small, then the estimator \eqref{eq:grad_approx} approximates  the true gradient $\nabla \vp(z,\xi)$ well.





\paragraph{Randomized smoothing.}
For a non-smooth objective $f(z)$, we define the following function  
\begin{equation}\label{eq:smoothedfunc}
    f^\tau(z) \triangleq \E_{\tilde \be} f(z+\tau \tilde \be),
\end{equation}
where $\tau>0$ and $ \tilde\be$ is a vector picked uniformly at random from the Euclidean unit ball: $\{\tilde\be:\|\tilde\be\|_2\leq 1\}$. Function  $f^\tau(z)$ can be referred as a smooth approximation of $f(z)$. Here $f(z)\triangleq \E f(z,\xi)$. We notice that function $f^\tau(z)$ is introduced only for proof.\\

\noindent The next theorem presents the convergence rates for Algorithm \ref{alg:zoSPA} in terms of the expectation. For the convergence results in large deviation, we refer to the Appendix \ref{app:probab_converg}.

\begin{theorem}\label{th:conv_rate} 
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
% Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$.
%, where  $N$ is the number of iterations and $M^2 \triangleq  (M_2^2+M_{2,\delta}^2)$. 
Then  the following holds for\footnote{All the results obtained in this paper (except Section~\ref{sec:rest}) will have the same form for $\e_{\rm sad}  \triangleq \max_{y\in \Y}  f(\hat x^N, y) - \min_{x\in \X}   f(x, \hat y^N)$, but this required more accurate analysis, based on special trick from \cite{juditsky2011solving,beznosikov2020gradient}.} $\hat{\e}_{\rm sad}  \triangleq
% \max_{y\in \Y}  f(\hat x^N, y) - \min_{x\in \X}   f(x, \hat y^N)$ } $ \hat{\e}_{\rm sad}  \triangleq
f(\hat x^N, y_*) -  f(x_*, \hat y^N)$
% \max_{y\in \Y}  f(\hat x^N, y) - \min_{x\in \X}   f(x, \hat y^N)$,
where  $\hat z^N \triangleq (\hat x^N, \hat y^N)$ is the output of   Algorithm \ref{alg:zoSPA}:
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\D}{M_{\rm case1}}\sqrt{\frac{2 }{N}}$ with \\  $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + {d^2a_q^2\Delta^2}{\tau^{-2}}\right)$ 
 \begin{align}\label{eq:convergrate0}
      \E\left[ \hat{\e}_{\rm sad}\right]
     &\leq  M_{\rm case1}\D\sqrt{{2 }/{N}}
     + {\sqrt{d}\Delta \D}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\D}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\  $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate}
     \E\left[ \hat{\e}_{\rm sad}\right]
     \leq M_{\rm case2} \D   \sqrt{{2 }/{N}} + M_{2,\delta} \sqrt{d}  \D
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $\sqrt{\E\left[ \|\be\|_q^4\right]}= \O\left( \min\{q,\log d \} d^{2/q-1} \right)  =a_q^2$ \cite{gorbunov2019upper}. 
\end{theorem}

  \begin{wrapfigure}{L}{0.5\textwidth}
    \begin{minipage}{0.5\textwidth}
    \vspace{-0.7cm}
\begin{algorithm}[H]
 \caption{\textit{Zeroth-order} \textsc{SMD}}
\label{alg:zoSPA}
\KwData{ iteration number $N$}\\
$z^1  \leftarrow \arg\min_{z\in \Z} d(z)$
\For{$k=1,\dots, N$}{
  Sample $\be^k, \xi^k$ independently\\
  Initialize $\gamma_k$\\ 
 Calculate $g(z^k, \xi^k, \be^k)$ via \eqref{eq:grad_approx}\\
  $z^{k+1}  \leftarrow {\rm Prox}_{z^k}\left(\gamma_k g(z^k, \xi^k, \be^k)\right)$
  %\Comment*[r]{mirror descent step}
}
\KwResult{ $\hat z^N  \leftarrow \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^{N} \gamma_k z^k$}
\end{algorithm}
\vspace{-0.5cm}
    \end{minipage}
  \end{wrapfigure}

Algorithm \ref{alg:zoSPA} and its convergence analysis given in Theorem \ref{th:conv_rate} are based on the same proximal setups for spaces $\X$
and $\Y$. For the case,  when these setups are different we   replace the proximal step  $z^{k+1}  \leftarrow {\rm Prox}_{z^k}\left(\gamma_k g(z^k, \xi^k, \be^k)\right)$ on the  space $\Z\triangleq \X \times \Y$  by two proximal steps on spaces $\X$ and $\Y$. The convergence analysis in this case is given in  the Appendix  \ref{app:variablesep}.\\

\noindent
The next corollary presents our contribution. 
\begin{corollary}\label{cor:bound_noise}
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}, and 
let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement is true
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\E\left[\hat{\e}_{\rm sad}(\hat z^N)\right]\le\e$  after 
% \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\D^{-2}\e^2)^2 \right)\]
\[N =  \O\left( {da_q^2M_2^2\D^2}/{\e^{2}} \right)\]
iterations, where 
 $\sqrt{\E\left[ \|\be\|_q^4\right]}= \O\left( \min\{q,\log d \} d^{2/q-1} \right)  =a_q^2$ \cite{gorbunov2019upper}.  
% \begin{enumerate}
%     \item 
    % under Assumption \ref{ass:err_noise}
    % \[\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O \left( \frac{\e}{M_2} \right) \] 
  
    % \item under Assumption \ref{ass:Lip_noise}
    %   \[\delta(z) =\O\left( \frac{\e}{\D\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O\left( \frac{\e}{M_2} \right) \] 
%\end{enumerate}
% where $\e = \max\limits_{y\in \Y}  f(\hat x^N, y) - \min\limits_{x\in \X}   f(x, \hat y^N)$ and $(\hat x^N, \hat y^N,)$ are the outputs of the    Algorithm \ref{alg:zoSPA} after 
% \[N = \O\left( {M^2\D^2(1+ca_q^2d)^2}{\e^{-1}} \right)\]
% iterations.
\end{corollary}
Next we clarify the Corollary \ref{cor:bound_noise} in the two following special setups: the $\ell_2$-norm and the $\ell_1$-norm in the two following examples.
\begin{example}
Let $p=2$, then $q=2$ and  $\sqrt{\E \left[ \|\be\|_2^4\right]}   = 1$. Thus, $a_2^2=1$ and $\D^2 = \max\limits_{z,v\in \Z}\|z-v\|^2_2$. Consequently, the number of iterations in the Corollary \ref{cor:bound_noise} can be rewritten as follows
\[N =  \O\left( \frac{dM_2^2}{\e^{2}}\max\limits_{z,v\in \Z}\|z-v\|^2_2\right).\]
\end{example}
\begin{example}\citet[Lemma 4]{shamir2017optimal}
Let $p=1$ then, $q=\infty$ and $\sqrt{\E \left[ \|\be\|_\infty^4\right]}   = \O\left({\frac{\log d}{d}}\right)$. Thus, $a_\infty^2=\O\left({\frac{\log d}{d}}\right)$ and $\D^2 = \O\left(\log d \max\limits_{z,v\in \Z}\|z-v\|^2_1\right)$. Consequently, the number of iterations in the Corollary \ref{cor:bound_noise} can be rewritten as follows
\[N =  \O\left( \frac{M_2^2\log^2 d}{\e^{2}}\max\limits_{z,v\in \Z}\|z-v\|_1^2 \right).\]
\end{example}
% \begin{proof} 
%{\bf of the  Corollary \ref{cor:bound_noise}}
% The proof is based on equating Eq. \eqref{eq:convergrate0} 
% %and \eqref{eq:convergrate} 
% in Theorem \ref{th:conv_rate}  to $\e$. From that, the bounds for the number of iterations $N$, $\tau$ and $\Delta$ can be obtained. \\
% For instance, for $N$, we have
% \[N = \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})^2 \right) =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + da_q^2\D^{-2}\e^2)^2 \right).\]
% \end{proof}
% \noindent
% Under Assumption \ref{ass:Lip_noise}, the following corollary gives the maximum value for the Lipschitz constant of the adversarial noise  to sole the problem  \eqref{eq:min_max_problem} with accuracy $\e$ by Algorithm. \ref{alg:zoSPA}.


% \begin{corollary}\label{cor:Lip_noise}
% Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}, and let  Assumption \ref{ass:err_noise} hold. 
% Let \[M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O \left( \frac{\e}{M_2} \right). \] 
% Then for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}    after 
% % \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + c {d}a_q^2\D^{-2}\e^2)^2 \right)\]
% \[N =  \O\left( {da_q^2M_2^2\D^2}{\e^{-2}} \right)\]
% iterations, it holds $\E\left[\e_{\rm sad}(\hat z^N)\right]=\e$.  
% \end{corollary}

\begin{remark}
Corollary \ref{cor:bound_noise} bound for the Lipschitz constant given in the Corollary \ref{cor:bound_noise} is probably not the upper bound. In the Appendix \ref{app:upperbound}, we provide a natural analysis to prove  the bound from Corollary \ref{cor:bound_noise} being optimal but our arguments are based on the assumption that the points of the function evaluation were chosen regardless of the stochastic realizations $\xi_1,\xi_2,\xi_3,\dots$. Unfortunately, that is not the case of Algorithm \ref{alg:zoSPA} and many other practical algorithms.
\end{remark}

\begin{proof}[Proof of the  Theorem \ref{th:conv_rate}] 
By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align*}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) + \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2.   
\end{align*}
Taking the conditional  expectation w.r.t. $\xi, \be$ and summing for $k=1,\dots,N$  we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE}
 \sum_{k=1}^N \gamma_k  \E_{\be^k,\xi^k} \left[ \la g(z^k,\be^k,\xi^k), z^k-u\ra\right] 
   &\leq  V_{z^1}(u)  + \sum_{k=1}^N\frac{\gamma_k^2}{2} \E_{\be^k,\xi^k}\left[\|g(z^k,\be^k,\xi^k)\|_q^2 \right]. 
\end{align}
% where $\mathcal D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ is the diameter  of $\Z$. 

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE} we use Lemma \ref{lm:shamirEnabla} and obtain
 \begin{enumerate}[leftmargin=*]
     \item  under Assumption  \ref{ass:err_noise}:
     \begin{equation}\label{eq:inmainsqEtwo1}
        \E_{\be^k,\xi^k}\left[\|g(z^k,\xi^k,\be^k)\|^2_q\right] \leq c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}{\tau^{-2}}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise}: 
\begin{align}\label{eq:inmainsqEtwo}
    \E_{\be^k,\xi^k}\left[\|g(z^k,\xi^k,\be^k)\|^2_q\right] \leq c a^2_q d (M_2^2+M_{2,\delta}^2),
\end{align}
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E \left[ \|\be^k\|_q^4\right]} \leq a_q^2$.

{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE}, we use Lemma \ref{lm:expecapproxgrad}


 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz11}
     \sum_{k=1}^N \gamma_k \E_{\be^k,\xi^k}\left[\la g(z^k,\be^k,\xi^k), z^k-u\ra \right]
     &\geq  \sum_{k=1}^N \gamma_k \la \nabla f^\tau(z^k), z^k-u \ra  \notag \\ &+\sum_{k=1}^N \gamma_k  \E_{\be^k}\left[ \left|\la  {d\Delta}{\tau^{-1}}  \be^k, z^k-u  \ra \right|\right].
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz}
     \sum_{k=1}^N \gamma_k \E_{\be^k,\xi^k}\left[\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] 
     &\geq  \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \notag \\ 
     &+\sum_{k=1}^N \gamma_k \E_{\be^k}\left[ \left|\la  dM_{2,\delta} \be^k, z^k-u\ra\right| \right].
\end{align}
 \end{enumerate}
For the first term of the r.h.s. of Eq.\eqref{eq:eqrefeqffxyz11} and \eqref{eq:eqrefeqffxyz} we have 
\begin{align}\label{eq:eqexpfxy}
     \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra 
     &= \sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra \notag \\
     &=  \sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right) \notag \\
     &\geq  \sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y)) \notag \\
     &=  \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)),
\end{align}
where $u \triangleq (x^\top,y^\top)^\top$.
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq  f^\tau\left(\frac{\sum_{k=1}^N \gamma_k x^k}{\sum_{k=1}^{N}\gamma_k},y\right)  - f^\tau\left(x, \frac{\sum_{k=1}^N \gamma_k y^k}{\sum_{k=1}^{N}\gamma_k}\right)\notag \\
     &=  f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE}  for Eq. \eqref{eq:eqexpfxy} we get 
\begin{align}\label{eq:fpslff}
     \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra 
     &\geq \sum_{k=1}^{N}\gamma_k  f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) .
\end{align}
Next we estimate the term $\E_{\be^k} \left[    |\la \be^k, z^k-u\ra|  \right] $ in Eq. \eqref{eq:eqrefeqffxyz11} and \eqref{eq:eqrefeqffxyz},   by the Lemma  \ref{lm:dotprodvece} 
\begin{align}\label{eq:sectermErhs}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\|z^k-u\|_2}/{\sqrt{d}}. 
\end{align}
Now  we substitute  Eq. \eqref{eq:fpslff} and  \eqref{eq:sectermErhs} to Eq. \eqref{eq:eqrefeqffxyz11} and \eqref{eq:eqrefeqffxyz}, and get
 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz1122}
   \sum_{k=1}^N \gamma_k   \E_{\be^k,\xi^k}\left[ \la g(z^k,\be^k,\xi^k), z^k-u\ra \right] &\geq
     \sum_{k=1}^{N}\gamma_k  f^\tau\left( \hat x^N,y\right)- f^\tau\left(x, \hat y^N \right)  \notag \\
     &-  \sum_{k=1}^N \gamma_k {\sqrt{d}\Delta\|z^k-u\|_2}{\tau^{-1}}. 
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz22}
     \sum_{k=1}^N \gamma_k  \E_{\be^k,\xi^k}\left[\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] 
     &\geq  \sum_{k=1}^{N}\gamma_k  f^\tau\left( \hat x^N,y\right) - f^\tau\left(x, \hat y^N \right)  \notag \\
     &- \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta}\|z^k-u\|_2. 
\end{align}
 \end{enumerate}
 
{\bf Step 3.} (under Assumption \ref{ass:err_noise}) \\
Now we combine Eq. \eqref{eq:eqrefeqffxyz1122}   with  Eq. \eqref{eq:inmainsqEtwo1} for Eq. \eqref{eq:inmainsqE} and obtain under Assumption \ref{ass:err_noise} the following
     \begin{align}\label{eq:inmainsqEtwo133}
     \sum_{k=1}^{N}\gamma_k f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) 
     &-  \sum_{k=1}^N \gamma_k {\sqrt{d} \Delta \|z^k-u\|_2}{\tau^{-1}}  \leq  V_{z^1}(u) \notag \\
     &+  \sum_{k=1}^N \frac{\gamma_k^2}{2} \left(c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}{\tau^{-2}}\right).
     \end{align}
Using Lemma \ref{lm:shamirSmoothFun} we obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this we can rewrite \eqref{eq:inmainsqEtwo133} as follows
 \begin{align}\label{eq:exEeqE1}
       f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right) 
      &\leq 
     \frac{ V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q dM_2^2+ d^2 a_q^2\Delta^2\tau^{-2}}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  \notag \\
      &+{ \sqrt{d} \Delta \max_{k}\|z^k-u\|_2}{\tau^{-1}} +  2\tau M_2.
 \end{align}
  For the r.h.s. of \eqref{eq:exEeqE1}  we use the definition of  the $\omega$-diameter  of $\Z$:\\
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$.
 Using this for  \eqref{eq:exEeqE1} and   taking $(x,y) = (x_*,y_*)$,
%  the maximum in $(x,y) \in (\X,\Y)$,
 we obtain
 \begin{align}\label{eq:dghjsklslsl1}
    % \max_{y \in \Y} 
    f\left( \hat x^N,y_*\right) -  
    % \min_{x\in \X} 
    f\left(x_*, \hat y^N \right)
     &\leq \frac{ \D^2+ (c a^2_q d M_2^2 +
     d^2 a_q^2\Delta^2\tau^{-2})
    \sum_{k=1}^{N} {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
       \notag \\
    &+ {\sqrt{d}\Delta \D}{\tau^{-1}}
     +  2\tau M_2.  
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Then we use the definition of  the $\omega$-diameter  of $\Z$:
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$. Thus, taking the expectation of \eqref{eq:dghjsklslsl1} and choosing  learning rate $\gamma_k 
=\frac{\D}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl1} we get
 \begin{align*}
      \E\left[ 
    %   \max_{y \in \Y}
      f\left( \hat x^N,y_*\right) -  
    %   \min_{x\in \X} 
      f\left(x_*, \hat y^N \right)\right]
     &\leq  
     %\frac{\D(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     M_{\rm case1}\D\sqrt{{2}/{N}}
     + \frac{\Delta\D\sqrt{d}}{\tau} 
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 4.} (under Assumption \ref{ass:Lip_noise})\\
Now we combine Eq.  \eqref{eq:eqrefeqffxyz22}  with  Eq.  \eqref{eq:inmainsqEtwo} for Eq. \eqref{eq:inmainsqE} and obtain under Assumption \ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo334}
    \sum_{k=1}^{N}\gamma_k f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) 
    &- \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta}\|z^k-u\|_2 \leq V_{z^1}(u)\notag \\
    &+  \sum_{k=1}^N \frac{\gamma_k^2}{2} c a^2_q d (M_2^2+M_{2,\delta}^2).
\end{align}
Using Lemma \ref{lm:shamirSmoothFun} we obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this we  can rewrite \eqref{eq:inmainsqEtwo334} as follows
 \begin{align}\label{eq:exEeqE}
      f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  
      &\leq 
     \frac{ V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q d (M_2^2+M_{2,\delta}^2)}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2} \notag\\
      &+ \sqrt{d}M_{2,\delta} \max_{k} \|z^k-u\|_2  +  2\tau M_2. 
 \end{align}
   For the r.h.s. of \eqref{eq:exEeqE}  we use the definition of  the $\omega$-diameter  of $\Z$: \\
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$.
 Using this for  \eqref{eq:exEeqE} and   taking $(x,y) = (x_*,y_*)$,
%  the maximum in $(x,y) \in (\X,\Y)$, 
 we obtain
 \begin{align}\label{eq:dghjsklslsl}
    %   \max_{y \in \Y} 
      f\left( \hat x^N,y_*\right) -  
    %   \min_{x\in \X}
      f\left(x_*, \hat y^N \right)
     &\leq \frac{ \D^2+ c a^2_q d (M_2^2 +M_{2,\delta}^2)\sum_{k=1}^N {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
    \notag\\
     &+ M_{2,\delta}  \sqrt{d}\D
     +  2\tau M_2.  
 \end{align}
 Then we use the definition of  the $\omega$-diameter  of $\Z$:
$\D \triangleq \max_{z,v\in \Z}\sqrt{2V_{z}(v)}$ and estimate $\|z^k-u\|_2 \leq \D$ for all $z^1,\dots, Z^k$ and all $u\in \Z$. Thus, taking the expectation of \eqref{eq:dghjsklslsl1} and choosing  learning rate  $\gamma_k 
=\frac{\D}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl} we get
%   $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$  in Eq. \eqref{eq:dghjsklslsl} we obtain
%  \begin{align*}
%       \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
%      &\leq  \frac{\D(1+c a^2_q d M_2^2 + c a^2_q dM_{2,\delta}^2)}{\sqrt{2N}M}  + M_{2,\delta} \D \sqrt{d} 
%      +  2\tau M_2.  
%  \end{align*}
 \begin{align*}
      \E\left[ 
    %   \max_{y \in \Y} 
      f\left( \hat x^N,y_*\right) -  
    %   \min_{x\in \X} 
      f\left(x_*, \hat y^N \right)\right]
     &\leq  M_{\rm case2}\D\sqrt{{2}/{N}}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.  
 \end{align*}
\end{proof}

==> intuition.tex <==
\section{Intuition of Smoothing}\label{sec:intuition}
In this section, we provide a motivation for smoothing a non-smooth function according to \eqref{eq:smoothedfunc}. 



Subgradients of a non-smooth function cannot be estimated by the  gradient-free approximation \eqref{eq:grad_approx}. 
 Indeed, let us consider the following example.
 



 




\begin{example}
Let us consider the one-dimensional ($d=1$) deterministic function $f(x)$ from Figure \ref{fig:non_smooth_funct}  with zeros noise ($\delta=0$) for simplicity.  Then, gradient-free approximation \eqref{eq:grad_approx} can be simplified as 
\begin{equation}\label{eq:simpgrad}
    g(x) = \frac{1}{2\tau}(f(x+\tau) - f(x-\tau)).
\end{equation}
Let us consider non-smooth function  $f(x) = |x|$.
For point $x>0$ taken close to $0$ we have
 \[g(x) = \frac{x}{\tau}, \]
 when $x \in [-\tau,\tau]$.
 However, for all $x>0$, $\nabla f(x)=1$. 
\end{example}




  \begin{figure}[h]
    \centering
   \includegraphics[width=0.5\linewidth]{approx2.png}
 \caption{Smooth approximation $f^{\tau}(x)$ of a non-smooth function $f(x)$}
 \label{fig:non_smooth_funct}
\end{figure}

\subsection{Differentiation of smooth approximation}
For simplicity, let us proof  Lemma \ref{lm:flax} in the 
one dimensional case $(d=1)$ 
    \[  f^\tau(x) \triangleq \E_{\tilde e} f(x+\tau \tilde e) = \frac{1}{2}\int_{-1}^1 f(x+\tau \tilde e)d \tilde e, \]
    where $\tilde e$ is a random vector from segment $[-1,1]$.\\
   We get for the derivative of $f$
    \[ \left( f^\tau(x)\right)_x' =  \frac{1}{2}\int_{-1}^1 f'_x(x+\tau \tilde e)d \tilde e. \]
    With the change of variable $y = x+\tau \tilde e$ we obtain
    \[
    \left( f^\tau(x)\right)_x' =  \frac{1}{2\tau}\int_{x-\tau}^{x+\tau} f'_y(y)dy = \frac{d}{2\tau} (f(x+\tau)-f(x-\tau))  = \E_{{e}}\left[\frac{d}{\tau}f(x+\tau {e})e\right],
    \]
    where $e$ is a random vector equal to 1 or -1 with probability $\nicefrac{1}{2}$.
 

% Smooth approximation
% a smooth approximation of a non-smooth function $f$ is
% \begin{equation*}
%     f^\tau(x) \triangleq \E_{\tilde \be} f(x+\tau \tilde \be),
% \end{equation*}
% where $\tau>0$ and $ \tilde\be$ is a random vector from the Euclidean unit ball.

% Whereas \[\E_{{\be}}\left[g(x,\be)\right] \neq \partial f(x).\]
%  Function  $f^\tau(x)$ is differentiable with the following gradient
% \[
% \nabla  f^\tau(x) = \E_{{\be}}\left[ \frac{d}{2\tau} (f(x+\tau {\be})-f(x-\tau {\be}))\be \right] = \E_{{\be}}\left[g(x,\be)\right],
% \]
% where $\be$ is a random vector from the Euclidean unit sphere.\\


% Main Idea: replace the original problem by
% \[
% \min_{x\in\X}f^\tau(x).
% \]




==> lemmas.tex <==
\section{Auxiliary Results for Theorem \ref{th:conv_rate}}\label{sec:auxiliarylemmas}


This section presents auxiliary results to prove Theorem \ref{th:conv_rate} from Section \ref{sec:mainthero}.


\begin{lemma}\label{lm:dotprodvece}
Let vector $\be$ be a random unit vector from the Euclidean unit sphere $\{\be:\|\be\|_2=1\}$. Then it holds for all $r \in \R^d$
 \begin{equation*}
     \E_{ \be}\left[ \left|\la \be, r \ra \right| \right] \leq {\|r\|_2}/{\sqrt{d}}.
 \end{equation*}
\end{lemma}


\begin{lemma}\label{lm:shamirSmoothFun}
Let $f(z)$ be $M_2$-Lipschitz continuous function. Then for $f^\tau(z)$ from \eqref{eq:smoothedfunc}, it holds
\[
\sup_{z\in \Z}|f^\tau(z) - f(z)|\leq \tau M_2.
\]
\end{lemma}

\begin{proof}
By the definition of $f^\tau(z)$ from \eqref{eq:smoothedfunc} and Assumption \ref{ass:Lip_obj} we have
\begin{align*}
    |f^\tau(z) - f(z)|
    &= \left|\E_{\be}\left[f(z+\tau\be)\right]  -f(z)\right| = \E_{\be}\left[|f(z+\tau\be) - f(z)| \right] \leq \E\left[ M_2 \|\tau \be\|_2\right] =  M_2 \tau.  
\end{align*}
\end{proof}

\begin{lemma}\label{lm:flax}
 Function  $f^\tau(z)$ is differentiable with the following gradient
\[
\nabla  f^\tau(z) = \E_{{\be}}\left[ \frac{d}{\tau} f(z+\tau {\be})\be \right].
\]
\end{lemma}


\begin{lemma}\label{lm:expecapproxgrad}
   For $g(z,\xi,\be)$ from \eqref{eq:grad_approx} and $f^\tau(z)$ from \eqref{eq:smoothedfunc}, the following holds 
 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \[\E_{\xi, \be}\left[\la g(z,\xi,\be),r\ra\right] \geq \la \nabla f^\tau(z),r\ra  - {d\Delta}{\tau^{-1}} \E_{\be} \left[\left|\la \be, r \ra \right|\right],\]
     \item  under Assumption \ref{ass:Lip_noise}   \[\E_{\xi, \be}\left[\la g(z,\xi,\be),r\ra\right] \geq \la \nabla f^\tau(z),r\ra   - d M_{2,\delta} \E_{\be} \left[\left|\la  \be, r \ra \right|\right],\]
 \end{enumerate}
 \end{lemma}


\begin{proof} Let us consider
\begin{align*}
  \hspace{-0.3cm} g(z,\be,\xi) 
    &= \frac{d}{2\tau}   \left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be \notag \\
    &=\frac{d}{2\tau}  \left(f(z+\tau \be,\xi) +\delta(z+\tau \be) - f(z-\tau \be,\xi) - \delta(z-\tau \be) \right) \be\notag \\
   &=\frac{d}{2\tau} \left(\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi) \right) \be +     (\delta(z+\tau \be) - \delta(z-\tau \be)) \be\right).
\end{align*}
Using this we have the following \begin{align}\label{eq:sqprod}
    \E_{\xi, \be}\left[\la g(z,\xi,\be),r\ra\right]   &=\frac{d}{2\tau}  \E_{\xi, \be}\left[\la\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi) \right) \be, r \ra \right]\notag \\
    &+\frac{d}{2\tau}  \E_{ \be}\left[     \la (\delta(z+\tau \be) - \delta(z-\tau \be)) \be, r\ra\right].
\end{align}
Taking the expectation, w.r.t. $\be$, from  the first term of the r.h.s. of \eqref{eq:sqprod} and  using the symmetry of the distribution of $\be$, we have
 \begin{align}\label{eq:nablaeqfunc}
      \frac{d}{2\tau}\E_{\xi, \be} \left[  \left(\la f(z+\tau \be,\xi)  - f(z-\tau \be,\xi) \right) \be, r\ra \right] 
        &= \frac{d}{2\tau}\E_{\xi, \be}  \left[ \la f(z+\tau \be,\xi)\be, r\ra \right] +\frac{d}{2\tau}\E_{\xi, \be}  \left[  \la f(z-\tau \be,\xi)\be, r\ra \right]   \notag\\
         &= \frac{d}{\tau}\E_{\be} \left[ \la\E_{\xi} \left[ f(z+\tau \be,\xi)\right] \be, r\ra\right] = \frac{d}{\tau}\E_{\be} \left[ \la  f(z+\tau \be) \be, r\ra\right] \notag\\
         &=\la \nabla f^\tau(z),r\ra. \quad /*  \mbox{Lemma \ref{lm:flax}}  */ 
\end{align}
\begin{enumerate}[leftmargin=*]
    \item For the second term of the r.h.s. of \eqref{eq:sqprod} under the Assumption \ref{ass:err_noise} we obtain 
    \begin{align}\label{eq:secondtermlipschnass2}
    \frac{d}{2\tau}  \E_{ \be} \left[  \la(\delta(z+\tau \be) - \delta(z-\tau  \be)) \be, r\ra \right] \geq - \frac{d}{2\tau} 2\Delta \E_{\be} \left[ \left|\la \be, r \ra \right|\right] = -\frac{d\Delta}{\tau} \E_{\be} \left[ \left|\la \be, r \ra \right| \right].
\end{align}
    \item For the second term of the r.h.s. of \eqref{eq:sqprod} under the Assumption \ref{ass:Lip_noise} we obtain  
\begin{align}\label{eq:secondtermlipschn}
    \frac{d}{2\tau}  \E_{\be} \left[ \la (\delta(z+\tau \be) - \delta(z-\tau \be)) \be, r\ra\right] \geq - \frac{d}{2\tau} M_{2,\delta} 2\tau \E_{\be} \left[ \|\be\|_2 \left|\la\be, r\ra \right|\right] = -d M_{2,\delta}  \E_{\be} \left[ \left|\la\be, r\ra\right|\right].
\end{align}
\end{enumerate}


Using Eq. \eqref{eq:nablaeqfunc} and \eqref{eq:secondtermlipschnass2} (or Eq. \eqref{eq:secondtermlipschn}) for Eq. \eqref{eq:sqprod} we get the statement of the lemma.
% \begin{align}
%   \E\left[ g(z,\be,\xi)\right]  \geq  \nabla f^\tau (z)  - d M_{2,\delta} \E_{\be} \left[ \be\right]
% \end{align}

\end{proof}








\begin{lemma}\citet[Lemma 9]{shamir2017optimal}\label{lm:shamirLm9}
For any function $f(\be)$ which is $M$-Lipschitz w.r.t. the $\ell_2$-norm, it holds that if $\be$ is uniformly distributed on the Euclidean unit sphere, then
\[
\sqrt{\E\left[(f(\be) - \E f(\be))^4 \right]} \leq cM_2^2/d
\]
for some numerical constant $c$.
\end{lemma}






\begin{lemma}\label{lm:shamirEnabla}
 For $g(z,\xi,\be)$ from \eqref{eq:grad_approx}, the following holds
%  and $f^\tau(z)$ from \eqref{eq:smoothedfunc}, it holds that   $\E\left[g(z,\xi,\be)\right] = \nabla f^\tau(z)$. Moreover,  
 under Assumption \ref{ass:Lip_obj} 
 \begin{enumerate}
     \item  and Assumption  \ref{ass:err_noise}
     \[\E_{\xi,\be}\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}/{\tau^2},\]
     \item  and Assumption \ref{ass:Lip_noise} 
\[\E_{\xi,\be}\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q d (M_2^2+M_{2,\delta}^2),\] 
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E \left[ \|\be\|_q^4\right]} \leq a_q^2$.
\end{lemma}


% \begin{align}
%   \E\left[g(z,\xi,\be)\right] &= \E\left[ \frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be \right] \notag \\
%       &= \frac{d}{2\tau}\E \left[  \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right) \be \right] \notag\\
%         &= \frac{d}{2\tau}\E \left[ f(z+\tau \be,\xi)\be \right] + \frac{d}{2\tau}\E \left[\delta(z+\tau\be)\be \right]\notag \\
%         &+\frac{d}{2\tau}\E \left[  f(z-\tau \be,\xi)(-\be) \right]  +\frac{d}{2\tau}\E \left[\delta(z-\tau\be) (-\be) \right] \notag\\
%          &= \frac{d}{\tau}\E \left[ f(z+\tau \be,\xi)\be\right] + \frac{d}{\tau}\E \left[\delta(z+\tau\be)\be \right], \qquad /*\mbox{ the  distribution of $\be$ is symmetric } */  \notag\\
%          &=\nabla f^\tau (z)  + \frac{d}{\tau}\E \left[\delta(z+\tau\be)\be \right]. \qquad /* ~ \mbox{ Lemma \ref{lm:flax} } ~ */ 
% \end{align}

\begin{proof} Let us consider
\begin{align}\label{eq:sqnormE}
    &\E_{\xi,\be} \left[\|g(z,\xi,\be)\|^2_q \right] = \E_{\xi,\be}\left[ \left\|\frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be\right\|^2_q \right] \notag \\
    &= \frac{d^2}{4\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right)^2 \right] \notag\\
     &\leq \frac{d^2}{2\tau^2}\left(\E_{\xi,\be} \left[\|\be\|_q^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right] + \E_{\be} \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \right).
\end{align}
For the first term in the r.h.s. of Eq. \eqref{eq:sqnormE}, the following holds with an arbitrary parameter $\alpha$
\begin{align}\label{eq:fgkbbhgdddgh}
 & \frac{d^2}{2\tau^2}\E_{\xi,\be} \left[\|\be\|_q^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right]  \notag\\
  &= \frac{d^2}{2\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 \left((f(z+\tau \be,\xi) -\alpha) -(f(z-\tau \be,\xi) - \alpha)   \right)^2 \right] \notag\\
    &\leq \frac{d^2}{\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 + (f(z-\tau \be,\xi) -\alpha)^2 \right] \qquad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
     &=  \frac{d^2}{\tau^2}\left(\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] + \E_{\xi,\be} \left[\|\be\|_q^2(f(z-\tau \be,\xi) -\alpha)^2 \right] \right) \notag\\
    &= \frac{2d^2}{\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
\end{align}
Applying the Cauchy--Schwartz inequality for Eq. \eqref{eq:fgkbbhgdddgh} and using $\sqrt{\E \left[ \|\be\|_q^4\right]} \leq a_q^2$ we obtain 
\begin{align}\label{eq:funcsq}
     \frac{d^2}{\tau^2}\E_{\xi,\be} \left[ \|\be\|_q^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] 
     &\leq \frac{d^2}{\tau^2} \E_{\xi} \left[\sqrt{\E \left[ \|\be\|_q^4\right]} \sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]} \right]\notag\\
     &\leq \frac{d^2 a_q^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right] . 
\end{align}
Then we assume $\alpha = \E_{\be}\left[f(z+\tau \be,\xi)\right]$
% , $\beta = \E\left[\delta(z+\tau \be)\right]$ 
and use Lemma \ref{lm:shamirLm9} along with the fact that $f(z+\tau\be,\xi)$ is $\tau M_2(\xi)$-Lipschitz, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus for Eq. \eqref{eq:funcsq}, it holds  
\begin{align}\label{eq:finlhkjfsvn}
    \frac{d^2 a_q^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right]
    &\leq \frac{d^2 a_q^2}{\tau^2} \cdot c\frac{\tau^2 \E M_2^2(\xi)}{d} = c d a_q^2 M_2^2.  
    %\red{\text{it seems should be} \leq}
\end{align}
\begin{enumerate}[leftmargin=*]
    \item Under the Assumption \ref{ass:err_noise}
     for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE}, the following holds
    \begin{align}\label{eq:fgkssssffdgh}
        &\frac{d^2}{4\tau^2}\E_{\be} \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \leq  \frac{d^2\Delta^2}{\tau^2} \E \left[ \|\be\|_q^2  \right]\leq \frac{d^2 a_q^2\Delta^2}{\tau^2}.
    \end{align}
   % where we used $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$.
    \item Under the Assumption \ref{ass:Lip_noise}
    for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE}, the following holds with an arbitrary parameter $\beta$
    \begin{align}\label{eq:fgklljgsdgh}
        &\frac{d^2}{4\tau^2}\E_{\be} \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \notag \\
     &= \frac{d^2}{2\tau^2}\E \left[ \|\be\|_q^2 \left((\delta(z+\tau\be) -\beta) -(\delta(z-\tau\be)  -\beta) \right)^2 \right] \notag\\
    &\leq \frac{d^2}{\tau^2}\E \left[ \|\be\|_q^2 \left((\delta(z+\tau\be)-\beta)^2  +(\delta(z-\tau\be) -\beta)^2 \right) \right] \quad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
    &= \frac{d^2}{2\tau^2}\left(\E \left[ \|\be\|_q^2 (\delta(z+\tau \be)-\beta)^2 \right] + \E \left[\|\be\|_q^2(\delta(z-\tau \be) -\beta)^2 \right] \right) \notag\\
    &= \frac{d^2}{\tau^2}\E \left[ \|\be\|_q^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
    \end{align}
\end{enumerate}
and for the second term in the Eq. \eqref{eq:sqnormE}, we get
\begin{align}\label{eq:noisesq}
   \frac{d^2}{\tau^2}\E_{\be}\left[ \|\be\|_q^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]
   &\leq \frac{d^2}{\tau^2}\sqrt{\E \left[ \|\be\|_q^4\right]} \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \notag \\
   &\leq \frac{d^2 a_q^2}{\tau^2} \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] }
\end{align}
Then we assume  $\beta = \E_{\be}\left[\delta(z+\tau \be)\right]$ and use Lemma \ref{lm:shamirLm9} together with the fact that $\delta(z+\tau\be)$ is $\tau M_{2,\delta}$-Lipschitz continuous, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus, Eq. \eqref{eq:noisesq} can be rewritten as 
\begin{align}\label{eq:fkssoomnbd}
    \frac{d^2 a_q^2}{\tau^2}  \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } 
    &\leq \frac{d^2 a_q^2}{\tau^2}  \cdot c\frac{\tau^2  M_{2,\delta}^2}{d} \leq c a^2_q d M_{2,\delta}^2. 
    %\red{\text{it seems should be} \leq}
\end{align}
Using Eq. \eqref{eq:finlhkjfsvn} and \eqref{eq:fgkssssffdgh} (or Eq. \eqref{eq:fkssoomnbd}) for Eq. \eqref{eq:sqnormE}, we get the statement of the theorem.
% \begin{align*}
%     \left[\|g(z,\xi,\be)\|^2_q \right] 
%     &\leq \frac{d^2 a_q^2}{\tau^2} \cdot c\frac{\tau^2 \E M_2^2(\xi)}{d} + \frac{d^2 a_q^2}{\tau^2}  \cdot c\frac{\tau^2 \E M_{2,\delta}^2(\xi)}{d} \leq c a^2_q d (M_2^2+M_{2,\delta}^2). 
%     %\red{\text{it seems should be} \leq}
% \end{align*}
\end{proof}

==> noise.tex <==
\section{Infinite Noise Variance}
When the second moment of the  stochastic gradient  $\nabla f(z,\xi)$ is unbounded the rate of convergence may changes dramatically, see the next section. For such a case, we consider a more general inequality for  Assumptions~\ref{ass:Lip_obj}.  We suppose  that there exists a positive constant $\tilde{M_2}$ such that for   $M_2(\xi)$  Assumptions~\ref{ass:Lip_obj} the following holds 
\begin{equation*}
    \E \left[M_2(\xi)^{1+\kappa}\right]\le \tilde{M}_2^{1+\kappa},
\end{equation*}
where $\kappa \in \left(0,1\right]$. From  \citet[Lemmas 9 -- 11]{shamir2017optimal} the following can be obtained 
 \begin{enumerate}[leftmargin=*]
     \item  under Assumption  \ref{ass:err_noise}:
     \begin{equation}\label{eq:inmainsqEtwo1}
        \E\left[\|g(z,\xi,\be)\|^{1+\kappa}_q\right] \leq \tilde{c} a^2_q d^{(1+\kappa)/2}\tilde{M}_2^{1+\kappa} + 2^{1+\kappa}{d^{1+\kappa} a_q^2\Delta^2}{\tau^{-2}}=\tilde{M}_{case1}^{1+\kappa}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise}: 
\begin{align}\label{eq:inmainsqEtwo2}
    \E\left[\|g(z,\xi,\be)\|^{1+\kappa}_q\right] \leq \tilde{c} a^2_q d^{(1+\kappa)/2} (\tilde{M}_2^{1+\kappa}+M_{2,\delta}^{1+\kappa}) = \tilde{M}_{case2}^{1+\kappa},
\end{align}
 \end{enumerate}
 where    $\tilde{c}$ is some numerical constant and
 $\sqrt{\E_{\be} \left[ \|\be\|_q^{2+2\kappa}\right]} \leq \tilde{a}_q^2$. As a particular case: $\tilde{a}_{2}^2 = 1$, $\tilde{a}_{\infty}^2 = \O\left({\frac{\log^{(1+\kappa)/2} d}{d^{(1+\kappa)/2}}}\right)$. \\
Let us assume that $q \in \left[1+\kappa,\infty\right)$, $1/p + 1/q = 1$ and prox-function determined by
\[\omega(x) = K_q^{1/\kappa} \frac{\kappa}{1+\kappa}\|x\|_p^{\frac{1+\kappa}{\kappa}} \mbox{ with } K_q = 10\max\left\{1,(q-1)^{(1+\kappa)/2}\right\}.  \]
Based on \cite{vural2022mirror} one can prove the first part of Theorem~\ref{th:conv_rate_restarts} with $M_2$ replaced by $\tilde{M_2}$, stepsize is chosen as
\[\gamma_k = \frac{\left((1+\kappa)V_{z^1}(z^{\star})/\kappa\right)^{\frac{1}{1+\kappa}}}{\tilde{M}_{case}}N^{-\frac{1}{1+\kappa}}\]
and the first terms in the r.h.s. of \eqref{eq:convergrate0_restarts}, \eqref{eq:convergrate_restarts} is determined as follows 
\[\tilde{M}_{case}\left(\frac{1+\kappa}{\kappa}V_{z^1}(z^{\star})\right)^{\frac{\kappa}{1+\kappa}} N^{-\frac{\kappa}{1+\kappa}}.\]
These results can be further generalized to $r-$growth condition for duality gap ($r\ge 2$), see Assumption~\ref{ass:strongly_convex}.


==> probability_convergence.tex <==
\section{High-probability bound}
\label{H-PB}
\begin{assumption}[Uniformly Lischitz continuity of the objective]\label{ass:uni_Lip_obj}
 Function $f(z,\xi)$ is uniformly $M_2$-Lipschitz continuous in $z\in \Z$ w.r.t. the $\ell_2$-norm, i.e.,   for all  $z_1,z_2\in \Z$ and $\xi \in \Xi$, 
 \[|f(z_1, \xi)- f(z_2,\xi)| \leq M_2 \|z_1- z_2\|_2.\] 
\end{assumption}



Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
% Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$.
%, where  $N$ is the number of iterations and $M^2 \triangleq  (M_2^2+M_{2,\delta}^2)$. 
\begin{theorem}\label{th:conv_rate_prob}
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:uni_Lip_obj}. Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
=\frac{\D}{M}\sqrt{\frac{2}{N}}$, where  $N$ is the number of iterations and $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$. Then for the output $  (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, under Assumption \ref{ass:err_noise} for some constant $c$ the following holds
% \begin{align}
%       \text{Prob} & \left\{ \e_{\rm sad} (\hat z^N)  \geq \frac{4 \Omega^2 \sqrt{d} \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2 d^2}{M}   + \right. \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 d^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
%       & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} 
% \end{align}

\begin{align}
       &\text{Prob}  \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{ \sqrt{V_{z^1}(u)} M  }{\sqrt{N}}  +  \Omega \frac{2 \sqrt{2} M \sqrt{V_{z^1}(u)}}{c N} +\right. \nonumber\\
      & \left.  + 2 \tau M_2 + \frac{ \Omega \D \sqrt{d} \Delta }{\tau }    \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} \label{eq:convergrate_prob}.
\end{align}

where 
$ \e_{\rm sad}  \triangleq \max\limits_{y\in \Y}  f(\hat x^N, y) - \min\limits_{x\in \X}   f(x, \hat y^N)$.
%is the `saddle point residual'.
\end{theorem}


















\begin{proof}[Proof of the  Theorem \ref{th:conv_rate_prob}]
By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) + \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_2^2/2   \notag
\end{align}
Summing for $k=1,\dots,N$ we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE_prob}
   \sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra 
   &\leq V_{z^1}(u)  + \sum_{k=1}^N\gamma_k^2\|g(z^k,\be^k,\xi^k)\|_2^2/2  \notag\\
   &\leq  V_{z^1}(u) + \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_2^2, 
\end{align}
For the next steps we provide the new definition of gradient approximation of $\nabla f(z, \xi)$ following the Eq. $\eqref{eq:grad_approx}$:
\begin{equation}\label{eq:grad_approx_f}
    g_f(z,\xi, \be) = \frac{d}{2\tau}\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix},
\end{equation}
{\bf Step 1.}\\
In this step we will estimate the second term in the r.h.s of inequality \eqref{eq:inmainsqE_prob}. We can rewrite this term in the form :
\begin{align}\label{eq:prob_var}
    & \|g(z^k,\be^k,\xi^k)\|_2^2  = \frac{d^2}{4\tau^2}  \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right)^2 \leq \notag\\
     &\hspace{4cm}\leq 2 \|g_f(z^k,\be^k,\xi^k)\|_2^2 + \frac{d^2}{2\tau^2} \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2  
\end{align}
\begin{enumerate}
\item To estimate the first term in the r.h.s of Eq. \eqref{eq:prob_var} we invoke the Assumtion \ref{ass:uni_Lip_obj} and the Eq.\eqref{eq:grad_approx_f}. We observe that the function $g_f(z^k,\be^k,\xi^k)$ is uniformly $M_2 d$-Lipschitz continious and $\E_{\be^k} g_f(z^k,\be^k,\xi^k) = 0$. Thus we can use Lemma 9 from  \cite{shamir2017optimal} and obtain for some constant $c$: 
\begin{align}\label{eq:estim_of_g_f}
    \text{Prob} \left\{ \| g_f(z^k,\be^k,\xi^k) \|_2 > t  \right\} \leq \exp \left\{ - \frac{c t^2}{M_2^2 d} \right\} 
\end{align}
Invoking the last inequality and  Assumtion \ref{ass:uni_Lip_obj}, the random variables \\
$\phi_k = \gamma_k^2 \|g_f(z^k,\be^k,\xi^k)\|_2^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$ satisfy the premise of case B of Lemma 2 from \cite{lan2012validation} with $\sigma_k = \frac{2 d M_2^2}{c} \gamma_k^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$:
\begin{align*}
     \E_{|t-1} \left[ \exp \{|\phi_k|/\sigma_k\} \right] & = \E_{|t-1} \left[ \exp \{ \|g_f(z^k,\be^k,\xi^k)\|_2^2/4  M_2^2 d\} \right] = \\
     &= \int_0^{\infty} \text{Prob} \left\{ \exp \{ \|g_f(z^k,\be^k,\xi^k)\|_2^2/4  M_2^2 d\} \geq \tilde{t}  \right\} d \tilde{t} \leq \int_0^{1} 1 d \tilde{t} +\\
     & + \int_1^{\infty} \underbrace{\text{Prob} \left\{ \exp \{ \|g_f(z^k,\be^k,\xi^k)\|_2^2/4  M_2^2 d\} \geq \tilde{t}  \right\}}_{\text{by } \eqref{eq:estim_of_g_f} : \text{ }\leq \exp \left\{ - \frac{c \sigma_k^2  \ln \tilde{t}}{M_2^2 d} \right\} \leq \left(\frac{1}{\tilde{t}} \right)^{\frac{c \sigma_k^2}{d M_2^2}} = \left(\frac{1}{\tilde{t}} \right)^{2}} d \tilde{t} \leq 1 + 1 \leq  \exp \{1\}
\end{align*}

Invoking case B of Lemma 2 from \cite{lan2012validation}, we get
\small{
\begin{align}
    &\text{Prob} \left\{ \left| \sum_{k=1}^N \gamma_k^2 \|g_f(z^k,\be^k,\xi^k)\|_2^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1} \right| > \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c  \sum_{k=1}^N \gamma_k } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c  \sum_{k=1}^N \gamma_k } \right\} \nonumber \\
    & \hspace{8 cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} \label{eq:first_step_var}
\end{align}}
\normalsize 
\item Under the Assumption \ref{ass:err_noise}
     for the third term in the r.h.s. of Eq. \eqref{eq:prob_var}, the following holds
    \begin{align}\label{eq:first_step_var_delta}
        &\frac{d^2}{2\tau^2}  \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2  \leq  \frac{d^2\Delta^2}{2\tau^2} .
    \end{align}
\end{enumerate}

Thus using Eq.\eqref{eq:first_step_var} and \eqref{eq:first_step_var_delta}  we can estimate the second term in the r.h.s of inequality \eqref{eq:inmainsqE_prob} as follow:
\begin{align}
    &\text{Prob} \left\{ \left| \sum_{k=1}^N \gamma_k^2/2 \|g(z^k,\be^k,\xi^k)\|_2^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1} \right| > \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c  \sum_{k=1}^N \gamma_k } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c  \sum_{k=1}^N \gamma_k }+   \right. \nonumber \\
    &\hspace{4 cm} \left. +  \frac{d^2\Delta^2 \sum_{k=1}^N \gamma_k^2}{2 \tau^2 \sum_{k=1}^N \gamma_k } \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} \label{eq:first_step_second_term}
\end{align}
{\bf Step 2.}\\
Using the notation \eqref{eq:grad_approx_f} we rewrite the l.h.s. of  Eq. \eqref{eq:inmainsqE_prob} as following:

\begin{align}
    &\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra =\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \nonumber\\
    & + \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra + \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra \label{eq:step2_rewriten}
\end{align}
\begin{enumerate}
    \item For the first term in r.h.s. of  Eq. \eqref{eq:step2_rewriten}, we provide the following notions:
% $$\sigma_k = \gamma_k M_2 2 \mathcal D,$$
$$\sigma_k = 2 \gamma_k \sqrt{d} M_2  \sqrt{V_{z^1}(u)} \Omega ,$$
$$\phi_k (\xi_k)= \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra .$$
For applying the case A of Lemma 2 from \cite{lan2012validation} we need to estimate the module of function $\gamma_k\la g_f(z^k,\be^k,\xi^k) , z^k-u\ra$. Using Assumption \ref{ass:uni_Lip_obj} we obtain:
\begin{align}
    &\left| \gamma_k\la g_f(z^k,\be^k,\xi^k) , z^k-u\ra \right| \stackrel{\eqref{eq:grad_approx_f}}{=}  \left| \gamma_k\la \frac{d}{2\tau}\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix} , z^k-u\ra \right|\nonumber\\
    & \stackrel{Ass. \ref{ass:uni_Lip_obj}}{\leq} \gamma_k d M_2 \left| \la  \be , z^k-u\ra \right| \label{eq:estim_of_scalar_product}
\end{align}
Now we need to estimate the term $\left| \la  \be , z^k-u\ra \right|$. To do this, using the Poincaré's lemma from \cite{lifshits2012lectures} paragraph 6.3 we rewrite $\be$ in different form:
\begin{align}\label{eq:poincare_def_e}
    \be \stackrel{D}{=} \frac{\eta}{\sqrt{\eta_1^2 + \dots + \eta_d^2}},
\end{align}

where $\eta = \left( \eta_1, \eta_2, \dots , \eta_d \right)^T = \mathcal{N} \left( 0 , I_d \right)$. 
Using Lemma 1 \cite{laurent2000adaptive}
% \cite{boucheron2013concentration} 
it follows:
\begin{align}
    \text{Prob} \left\{  \sum_{k=1}^d \left|\eta_k\right|^2 \le d -  2 \sqrt{\Omega d} \right\} \leq  \exp \{- \Omega \} . \label{eq:step2_sphere_rewriten}
\end{align}
Using the definition of $\eta$ we obtain:
\begin{align}
    \la \eta, z^k-u \ra \stackrel{D}{=} \mathcal{N} \left( 0 , \|z^k - u\|_2^2 \right). \label{eq:step2_poincare}
\end{align}
Using Eq. \eqref{eq:step2_sphere_rewriten}, \eqref{eq:step2_poincare} and \eqref{eq:poincare_def_e} we can estimate the r.h.s of Eq. \eqref{eq:estim_of_scalar_product}:
\begin{align}
    \text{Prob} &\left\{     \left| \la \be, z^k-u \ra \right| > \frac{ \Omega V_{z^k}(u)}{\sqrt{d}} \right\} \leq 3 \exp \{-\Omega/4 \} . \label{eq:step1_sphere_rewriten_2}
\end{align}










Moreover, using Eq. \eqref{eq:estim_of_scalar_product}, Eq. \eqref{eq:step1_sphere_rewriten_2} and the fact that $V_{z^k}(u) = \O ( V_{z^1}(u)) \text{  } \forall k \geq 1$ from \cite{gorbunov2021gradient} we have:

\begin{align*}
    \text{Prob} \left\{\exp \left\{ \left(\gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra \right)^2/ \sigma_k^2 \right\}  \geq \exp \{1\}\right\} \leq 3 \exp \{-\Omega/4 \}
\end{align*}
It follows by case A of Lemma 2 from \cite{lan2012validation} that
\begin{align}
    & \text{Prob} \left\{ \left| \frac{\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra}{\sum_{k=1}^{N}\gamma_k}  \right| > \frac{4 \sqrt{d} \Omega^2 \sqrt{V_{z^1}(u)} M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} \right\} \leq \\
    & \hspace{8cm}\leq  2 \exp \{-\Omega^2/3 \} + 3 \exp \{-\Omega/4 \}. \label{eq:step2_martingale_rewriten}
\end{align}
\item For the second term in r.h.s of Eq. \eqref{eq:step2_rewriten} under the Assumption \ref{ass:err_noise} we obtain :
\begin{align}
    & \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra \geq - \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left|\la \be, z^k-u \ra \right| \label{eq:step2_delta_rewriten}
\end{align}

Using Eq. \eqref{eq:step1_sphere_rewriten_2} we can estimate the r.h.s of Eq. \eqref{eq:step2_delta_rewriten}:
\begin{align}
    \text{Prob} &\left\{   \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left| \la \be, z^k-u \ra \right| > \frac{ \Omega \D \sqrt{d} \Delta \sum_{k=1}^N \gamma_k}{\tau} \right\} \leq 3 \exp \{-\Omega/4 \} . \label{eq:step2_sphere_rewriten_2}
\end{align}
\item We rewrite the third term in r.h.s. of  Eq. \eqref{eq:step2_rewriten} in the following form: 
\begin{align} 
    \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra & =  \sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra  \notag \\
     &=  \sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right) \notag \\
     &\geq  \sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y)) \notag \\
     &=  \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \label{eq:eqexpfxy_prob}.
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE_prob}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq  f^\tau\left(\frac{\sum_{k=1}^N \gamma_k x^k}{\sum_{k=1}^{N}\gamma_k},y\right)  - f^\tau\left(x, \frac{\sum_{k=1}^N \gamma_k y^k}{\sum_{k=1}^{N}\gamma_k}\right)\notag \\
     &=  f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE_prob}  for Eq. \eqref{eq:eqexpfxy_prob} we get 
\begin{align}\label{eq:fpslff_prob}
      \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra  
     &\geq \left( \sum_{k=1}^{N}\gamma_k \right) \left( f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right) .
\end{align}
\end{enumerate}









{\bf Step 3.} \\
Then we use this with  Eq. \eqref{eq:step2_rewriten}, \eqref{eq:step2_delta_rewriten} and \eqref{eq:fpslff_prob} for Eq. \eqref{eq:inmainsqE_prob} and obtain
\begin{align}
      &f^\tau\left( \hat x^N,y\right)   - f^\tau\left(x, \hat y^N \right)  \leq   \frac{V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k } + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_2^2  \nonumber \\
    & - \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \la \be, z^k-u \ra \label{eq:exEeqE_prob}
\end{align}


 For the l.h.s. of Eq. \eqref{eq:exEeqE_prob} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2 \label{eq:f_tau_to_f}
 \end{align}
 Using Eq. \eqref{eq:first_step_second_term}, \eqref{eq:step2_martingale_rewriten}, \eqref{eq:step2_sphere_rewriten_2}, \eqref{eq:f_tau_to_f} and taking the maximum in $(x,y) \in (\X,\Y)$, we obtain we can rewrite Eq. \eqref{eq:exEeqE_prob} as follow:
 
 \begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \sqrt{V_{z^1}(u)} M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c \sum_{k=1}^N \gamma_k }  \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c \sum_{k=1}^N \gamma_k } +  \frac{d^2\Delta^2 \sum_{k=1}^N \gamma_k^2}{2 \tau^2 \sum_{k=1}^N \gamma_k } + \frac{V_{z^1}(u)}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
      & \hspace{3cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \}\label{eq:dghjsklslsl_proba}
\end{align}
%  \begin{align}
%       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } +\frac{d \D \Delta}{\tau} \right. \nonumber\\
%       & \left.+ \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
%       & \hspace{5cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} \label{eq:dghjsklslsl_proba}
% \end{align}

 Choosing the learning rate $\gamma_k 
=\frac{\sqrt{V_{z^1}(u)}}{M}\sqrt{\frac{2}{N}}$ with $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl_proba} we obtain
\begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \sqrt{V_{z^1}(u)} M_2  }{\sqrt{N}} + \frac{2 \sqrt{2}  \sqrt{V_{z^1}(u)} M_2^2 d}{c M\sqrt{N}}   + \right. \nonumber\\
      & \hspace{2cm}\left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2 \sqrt{2} M_2^2 d \sqrt{V_{z^1}(u)}}{c M N} +  \frac{d^2\Delta^2 \sqrt{2} \sqrt{V_{z^1}(u)}}{2 \tau^2 M \sqrt{N} }+ \frac{\sqrt{V_{z^1}(u)} M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
      & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .
\end{align}

Using the notation of $M$ we obtain:
\begin{align}
       &\text{Prob}  \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{  \sqrt{V_{z^1}(u)} M  }{\sqrt{N}}   + \frac{ \Omega \D \sqrt{d} \Delta }{\tau }  + \right. \nonumber\\
      & \left.+2 \tau M_2 + \Omega \frac{2 \sqrt{2} M \sqrt{V_{z^1}(u)}}{c N}    \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .
\end{align}

% \begin{align}
%       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2}{M}  +\frac{d \D \Delta}{\tau} + \right. \nonumber\\
%       & \left. \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} 
% \end{align}
\end{proof}




==> restarts.tex <==
\section{Restarts and Linear Convergence Rate}\label{sec:rest}
In this section we apply restart-technique \cite{juditsky2014deterministic} to  Algorithm\ref{alg:zoSPA} in the case when we additionally have $\gamma-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems). 
\begin{assumption}\label{ass:strongly_convex}
There is $\gamma \geq 1$ and $\mu_{\gamma} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
$$ \frac{\mu_{\gamma}}{2} \|z-z^{\star}\|_p^{\gamma} 
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right).
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
$$
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
Then for the output $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA},  the following holds for $ \e_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \e_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \e_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $a_q^2$ is such that $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, if Assumption \ref{ass:strongly_convex} is satisfied we can apply restarts and to achieve $\E[\e_{\rm sad}] \leq \varepsilon$ one need $N$ iterations where $N$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N &= \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right),\\
     N &=  \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right),
 \end{align}
 where $B$ is an inaccuracy associated with the $\tau$-smoothing and inexactness of the oracle. 
 Constants $A, B$ depend on noise conditions and are given by the following equality
 \begin{enumerate}
    \item under Assumption \ref{ass:err_noise} 
 \begin{align}\label{eq:err_noise_AB}
      A = \sqrt{2} M_{\rm case1}, \;\;\; B = {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2,
 \end{align}
    \item under Assumption \ref{ass:Lip_noise} 
    \begin{align}\label{eq:err_noise_AB_2}
      A = \sqrt{2} M_{\rm case2}, \;\;\; B = M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.
 \end{align}
\end{enumerate}
Thus, from \eqref{eq:err_noise_AB} $\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon^2/\left(\D M_2\sqrt{d}\right)\right)$ and from \eqref{eq:err_noise_AB_2}
$\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon/\left(\D\sqrt{d}\right)\right)$.
\end{theorem}

\begin{remark}
An important particular case of Theorem~\ref{th:conv_rate_restarts} is when $\gamma = 1$. Under this assumption the estimate on the number of iteration $\eqref{eq:estim_iter_restart}$ can be rewritten in the following form:
 \begin{align}
     N = \widetilde \O\left(\frac{64 \cdot A^2}{\mu_{1}^2 } \right) = \widetilde \O\left(\frac{A^2}{\mu_{1}^{2} } \right).
 \end{align}
As a result, it leads us to the linear convergence of the algorithm for non-smooth convex-concave saddle points problems with sharp saddle-point. For convex optimization problems with sharp minimum this effect was known \cite{juditsky1993stochastic}.
\end{remark}



%  \iffalse

\begin{proof}[Proof of the  Theorem \ref{th:conv_rate_restarts}]
By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) - \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2   \notag
\end{align}
Summing for $k=1,\dots,N$  and taking the expectation, we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE_restarts}
   \E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right]
   &\leq \E [V_{z^1}(u)]  - \E\left[\sum_{k=1}^N\frac{\gamma_k^2}{2}\|g(z^k,\be^k,\xi^k)\|_q^2 \right] \notag\\
   &\leq  \E[V_{z^1}(u)] + \sum_{k=1}^N \frac{\gamma_k^2}{2} \E\left[\|g(z^k,\be^k,\xi^k)\|_q^2\right],
\end{align}
where we took into account that $z^1$ can be chosen in stochastic way.

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE_restarts} we use Lemma \ref{lm:shamirEnabla} and obtain
 \begin{enumerate}[leftmargin=*]
     \item  under Assumption  \ref{ass:err_noise}:
     \begin{equation}\label{eq:inmainsqEtwo1_restarts}
        \E\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q dM_2^2 + {d^2 a_q^2\Delta^2}{\tau^{-2}}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise}: 
\begin{align}\label{eq:inmainsqEtwo_restarts}
    \E\left[\|g(z,\xi,\be)\|^2_q\right] \leq c a^2_q d (M_2^2+M_{2,\delta}^2),
\end{align}
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$.

{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE_restarts}, we use Lemma \ref{lm:expecapproxgrad}


 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz11_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] =  \E\left[\sum_{k=1}^N \gamma_k\left\la \E_{\be^k}\left[g(z^k,\be^k,\xi^k) \right], z^k-u\right\ra \right] \notag\\
     &\hspace{2cm}\geq  \E\left[\sum_{k=1}^N \gamma_k \la \nabla f^\tau(z^k), z^k-u \ra \right] - \E\left[\sum_{k=1}^N \gamma_k\left|\la  {d\Delta}{\tau^{-1}}  \be^k, z^k-u  \ra \right|\right].
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] =  \E\left[\sum_{k=1}^N \gamma_k\left\la \E_{\be^k}\left[g(z^k,\be^k,\xi^k) \right], z^k-u\right\ra \right] \notag\\
     &\hspace{2cm}\geq  \E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right]-\E\left[\sum_{k=1}^N \gamma_k\left|\la  dM_{2,\delta} \be^k, z^k-u\ra\right| \right].
\end{align}
 \end{enumerate}
For the first term of the r.h.s. of Eq.\eqref{eq:eqrefeqffxyz11_restarts} and \eqref{eq:eqrefeqffxyz_restarts} we have 
\begin{align}\label{eq:eqexpfxy_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right]
     =  \E\left[\sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra \right] \notag \\
     &=  \E\left[\sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right)\right] \notag \\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y))\right] \notag \\
     &=  \E\left[\sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \right].
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE_restarts}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq    f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE_restarts}  for Eq. \eqref{eq:eqexpfxy_restarts} we get 
\begin{align}\label{eq:fpslff_restarts}
      \E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right] 
     &\geq \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right].
\end{align}
Next we estimate the term $\E_{\be^k} \left[    |\la \be^k, z^k-u\ra|  \right] $ in Eq. \eqref{eq:eqrefeqffxyz11_restarts} and \eqref{eq:eqrefeqffxyz_restarts},   by the Lemma~\ref{lm:dotprodvece} 
\begin{align}\label{eq:sectermErhs_restarts}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\D}/{\sqrt{d}}. 
\end{align}
Now  we substitute  Eq. \eqref{eq:fpslff_restarts} and  \eqref{eq:sectermErhs_restarts} to Eq. \eqref{eq:eqrefeqffxyz11_restarts} and \eqref{eq:eqrefeqffxyz_restarts}, and get
 \begin{enumerate}[leftmargin=*]
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz1122_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right]
    \geq 
     \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)- f^\tau\left(x, \hat y^N \right) \right] -  \sum_{k=1}^N \gamma_k \frac{\sqrt{d}\Delta\D}{\tau}.  
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz22_restarts}
     &\E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] \geq  \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right) - f^\tau\left(x, \hat y^N \right) \right] - \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta}\D. 
\end{align}
 \end{enumerate}
 
{\bf Step 3.} (under Assumption \ref{ass:err_noise}) \\
Now we combine Eq. \eqref{eq:eqrefeqffxyz1122_restarts}   with  Eq. \eqref{eq:inmainsqEtwo1_restarts} for Eq. \eqref{eq:inmainsqE_restarts} and obtain under Assumption \ref{ass:err_noise} the following
     \begin{align}\label{eq:inmainsqEtwo133_restarts}
    & \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
     -  \sum_{k=1}^N \gamma_k \frac{\Delta\D\sqrt{d}}{\tau} \notag\\
     &\leq \E [V_{z^1}(u)] +  \sum_{k=1}^N \frac{\gamma_k^2}{2} \left(c a^2_q dM_2^2 + \frac{d^2 a_q^2\Delta^2}{\tau^2}\right).
     \end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE1_restarts}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      &\leq 
     \frac{ \E [V_{z^1}(u)]}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q dM_2^2+ d^2 a_q^2\Delta^2\tau^{-2}}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  +\frac{\Delta\D\sqrt{d}}{\tau}.
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE1_restarts} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE1_restarts} and  choosing $(x,y) = (x^{\star}, y^{\star})$, we obtain
 \begin{align}\label{eq:dghjsklslsl1_restarts}
     \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq \frac{ \E [V_{z^1}(z^{\star})]+ (c a^2_q d M_2^2 +
     d^2 a_q^2\Delta^2\tau^{-2})
    \sum_{k=1}^{N} {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
       \notag \\
    &+ {\Delta\D\sqrt{d}}{\tau^{-1}}
     +  2\tau M_2.
 \end{align}
%  where $D^2(z^1, z^{\star}) = V_{z^1}(z^{\star})$.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Choosing  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl1_restarts} we get
 \begin{align*}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  
     %\frac{V_{z^1}(u)(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E [V_{z^1}(z^{\star})]}
     + \frac{\Delta\D\sqrt{d}}{\tau} 
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 4.} (under Assumption \ref{ass:Lip_noise})\\
Now we combine Eq.  \eqref{eq:eqrefeqffxyz22_restarts}  with  Eq.  \eqref{eq:inmainsqEtwo_restarts} for Eq. \eqref{eq:inmainsqE_restarts} and obtain under Assumption~\ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo334_restarts}
    &\sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
    - \sum_{k=1}^N \gamma_k \sqrt{d}M_{2,\delta} \D \leq \E [V_{z^1}(u)] +  \sum_{k=1}^N \frac{\gamma_k^2}{2} c a^2_q d (M_2^2+M_{2,\delta}^2).
\end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE_restarts}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      &\leq 
     \frac{ \E [V_{z^1}(u)]}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c a^2_q d (M_2^2+M_{2,\delta}^2)}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  + M_{2,\delta} \D \sqrt{d}. 
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE_restarts} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE_restarts} and   chooosing $(x,y) = (x^{\star}, y^{\star})$, we obtain
 \begin{align}\label{eq:dghjsklslsl_restarts}
     \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq \frac{ \E [V_{z^1}(z^{\star})] + c a^2_q d (M_2^2+M_{2,\delta}^2)\sum_{k=1}^N {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
    \notag \\
    &+ M_{2,\delta}  \sqrt{d}\D
     +  2\tau M_2.
 \end{align}
 Choosing the learning rate 
%   $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$  in Eq. \eqref{eq:dghjsklslsl} we obtain
%  \begin{align*}
%       \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
%      &\leq  \frac{\D(1+c a^2_q d M_2^2 + c a^2_q dM_{2,\delta}^2)}{\sqrt{2N}M}  + M_{2,\delta} \D \sqrt{d} 
%      +  2\tau M_2.  
%  \end{align*}
 $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl_restarts} we obtain
 \begin{align*}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E [V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 5.} (Restart)
 At the previous step, we obtained the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq  \frac{A\sqrt{\E [V_{z^1}(z^{\star})]}}{\sqrt{N_1}}  + B,  
 \end{align}
 with an appropriate choice of constants $A, B$. Here $B$ is an inaccuracy associated with the stochastic setting of the problem and inexactness of the oracle. In this step we will employ the restart technique that is generalization of technique proposed in \cite{juditsky2014deterministic}.
 
 For the r.h.s. of Eq. \eqref{restart:rate} we use Assumption \ref{ass:strongly_convex} and the fact of remark 3 from \cite{gasnikov2018universal} that $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$ for the l.h.s 
 \begin{align}\label{restart:norms}
 \underbrace{\frac{\mu_{\gamma}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{\gamma}\right]}_{\geq\frac{\mu_{\gamma}}{2} \E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}
 \leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= A\widetilde \O(\underbrace{\E[\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}  + B.
 \end{align}
 Then by choosing ${N_1} = \frac{A^2\widetilde \O(R_0^2)}{B^2}$ and applying the Jensen inequality for l.h.s of Eq. \eqref{restart:norms} we get
 \begin{align}
 \frac{\mu_{\gamma}}{2} \underbrace{\E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}_{R_1^{\gamma}} \leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= 2A\widetilde \O(\underbrace{\E [\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}.
 \end{align}
 And finally taking ${N_1}$ so as to reduce the distance to the solution by half, we obtain
 $$ {N_1} = \widetilde \O \left( \frac{64A^2}{\mu_{\gamma}^2 R_1^{2(\gamma-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ from a similar condition for reducing the distance to the solution by a factor of $2$, and so on. 
 
 Thus, after $k$ of such restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N = N_1 +\dots + N_k = \widetilde \O \left(\frac{64 \cdot 2^{2(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}}\left(1+2^{2(\gamma-1)} + \dots + 2^{2(k-1)(\gamma-1)}\right) \right).
 \end{align} 
 It remains for us to determine the number of restarts, for this we fix the desired accuracy in terms of $\E[\e_{\rm sad}] \leq \varepsilon$ and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\e_{\rm sad}] = \widetilde \O \left(\frac{\mu_{\gamma} R_k^{\gamma}}{2}\right)=   \frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{\gamma}R_0^{\gamma}}{2^{k\gamma}}\right) \leq \varepsilon.
 \end{align} 
 Then to fulfill this condition one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{\gamma}R_0^{\gamma}/\varepsilon\right)) / \gamma$ and using Eq. \eqref{restart:N} we get the total number of iterations
 $$ N = \widetilde \O\left(\frac{64 \cdot 2^{2k(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}} \right) = \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right).$$
 Moreover, using ${N_k} = \frac{A^2\widetilde \O(R_{k-1}^2)}{B^2}$ and $\frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  \leq \varepsilon$ from Eq. \eqref{restart:epsilon} we have $B = \tilde{O}(\varepsilon)$.  This condition imposes restrictions on the final accuracy $\varepsilon$ and, as a consequence, on the choice of $N$, given by Eq. \eqref{restart:N}
 \begin{align*}
     N = \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right).
 \end{align*}
\end{proof}




\begin{remark}
The estimations on the noise $B$ in Eq. \eqref{eq:err_noise_AB} and \eqref{eq:err_noise_AB_2} can be improved in the following way: it is possible to obtain the better evaluation on the r.h.s of Eq. \eqref{eq:sectermErhs_restarts} as
\begin{align}\label{eq:sectermErhs_restarts_new}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|_2  \right] \leq {\|z^k - u\|}/{\sqrt{d}}. 
\end{align}
Choosing $u = (x^*, y^*)$ we provide exponentially decreasing sequence of $\D_2^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate}. It leads us to the more precise estimation on the noise $B$. We use this estimation on $B$ when we employ the restart technique in the proof of Theorem~\ref{th:conv_rate_restarts} and, thanks to this, we obtain the better estimate on the maximal level of noise: under Assumption \ref{ass:err_noise} $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{2-1/\gamma}}{M_2\sqrt{d}}$$  and 
under Assumption \ref{ass:Lip_noise} 
$$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{1-1/\gamma}}{\sqrt{d}}.$$
\end{remark}

\begin{remark}\label{hpb}
Based on high-probability bound from Appendix~\ref{H-PB} we can obtain high-probability bound by using the same restart-technique \cite{juditsky2014deterministic}. In the case $\gamma = 2$ it is probably possible to improve this bound in $\log \varepsilon^{-1}$ factor by using alternative algorithm \cite{harvey2019tight}. Moreover, based on stochastic-gradient clipping trick \cite{gorbunov2021near} we can obtain the result in Appendix~\ref{H-PB} in the case when the second moment of stochastic gradient is bounded (subgaussian tails are not required). When the variance of noise is not bounded (the second moment of stochastic gradient is non bounded) the rate of convergence may changes drastically, see the next section.
\end{remark}
% \fi



==> restarts_MOTOR.tex <==
\section{Restarts}\label{sec:rest}
In this section, we assume that we  additionally have the $r-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems).  For such a case, we apply the restart technique \cite{juditsky2014deterministic} to  Algorithm \ref{alg:zoSPA} 
\begin{assumption}[$r-$growth condition]\label{ass:strongly_convex}
There is $r \geq 1$ and $\mu_{r} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
\[\frac{\mu_{r}}{2} \|z-z^{\star}\|_p^{r}
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right),
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
\]
where $(x^*,y^*)$ is a solution of problem \eqref{eq:min_max_problem}.
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy Assumption \ref{ass:Lip_obj}. 
Then the following holds for $ \e_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$, where   $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ is the output of   Algorithm \ref{alg:zoSPA} 
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \e_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \e_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If the Assumption \ref{ass:strongly_convex} is satisfied for $r \geq 2$  and one of the two following statement is true
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, we can apply restart technique  to achieve $\E[\e_{\rm sad}] \leq \e$ in $N_{acc}$ iterations, where $N_{acc}$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N_{acc} = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \e^{2(r-1)/r}} \right).
 \end{align}
\end{theorem}
\textit{Proof of  Theorem \ref{th:conv_rate_restarts}.}
~We repeat the proof of Theorem \ref{th:conv_rate}, except that now $z^1$ can be chosen in a stochastic way. Moreover, now we use a rougher inequality instead of \eqref{eq:sectermErhs}
\begin{align}\label{eq:sectermErhs_restarts}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\D}/{\sqrt{d}}.
\end{align}
{\bf Step 1.} (under Assumption \ref{ass:err_noise}) \\
Taking the expectation in \eqref{eq:dghjsklslsl1}, choosing $(x,y) = (x^{\star}, y^{\star})$, and
 learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$  we get
 \begin{align} \label{rate:restarts1}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  
     %\frac{V_{z^1}(u)(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E [V_{z^1}(z^{\star})]}
     + \frac{\Delta\D\sqrt{d}}{\tau} 
     +  2\tau M_2.  
 \end{align}
 {\bf Step 2.} (under Assumption \ref{ass:Lip_noise})\\
Taking the mathematical expectation in \eqref{eq:dghjsklslsl1}, choosing $(x,y) = (x^{\star}, y^{\star})$, and  learning rate 
 $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$  we obtain
 \begin{align} \label{rate:restarts2}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E [V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.  
 \end{align}
{\bf Step 3.} (Restarts)\\
Now let $\tau$ be chosen as $\tau = \O\left(\e/M_2\right)$, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement holds
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then using \eqref{rate:restarts1} we obtain the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= \widetilde \O\left(\  a_q M_2 \sqrt{2d}\sqrt{\frac{\E [V_{z^1}(z^{\star})]}{N_1}}\right).
 \end{align}
  In this step we will employ the restart technique that is a generalization of technique proposed in \cite{juditsky2014deterministic}.\\
 For the l.h.s. of Eq. \eqref{restart:rate} we use the Assumption \ref{ass:strongly_convex}. For the r.h.s. of Eq. \eqref{restart:rate} we use $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$  from  \cite[Remark 3]{gasnikov2018universal}  
 \begin{align}\label{restart:norms}
 \frac{\mu_{r}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{r}\right]
 &\leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] \notag \\
     &= \frac{a_q M_2 \sqrt{2d}}{\sqrt{{N_1}}}\widetilde \O\left(\sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
 Then the l.h.s of Eq. \eqref{restart:norms} we  use the Jensen inequality and  get the following
 \begin{align}
 \frac{\mu_{r}}{2} \underbrace{\left(\sqrt{\E\left[\|z^{N_1} - z^{\star}\|_p^2\right]}\right)^{r}}_{R_1^{r}} &\leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] \notag\\
     &= \frac{a_q M_2 \sqrt{2d}}{\sqrt{{N_1}}}\widetilde \O\left(\sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
Finally taking ${N_1}$ so as to halve the distance to the solution, we get
 $$ {N_1} = \widetilde \O \left( \frac{a_q^2 M_2^2 d}{\mu_{r}^2 R_1^{2(r-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ similarly: we halve the distance $R_1$ to the solution, and so on. \\
 Thus, after $k$  restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N_{acc} = N_1 +\dots + N_k = \widetilde \O \left(\frac{ 2^{2(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}}\left(1+2^{2(r-1)} + \dots + 2^{2(k-1)(r-1)}\right) \right).
 \end{align} 
 Now we need  to determine the number of restarts. To do  this, we fix the desired accuracy  and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\e_{\rm sad}] = \widetilde \O \left(\frac{\mu_{r} R_k^{r}}{2}\right)=   \frac{2 a_q M_2 \sqrt{d} \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{r}R_0^{r}}{2^{kr}}\right) \leq \e.
 \end{align} 
 Then to fulfill this condition, one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{r}R_0^{r}/\e\right)) / r$ and using Eq. \eqref{restart:N} we get the total number of iterations
\[ N_{acc} = \widetilde \O\left(\frac{32 \cdot 2^{2k(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}} \right) = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \e^{2(r-1)/r}} \right).\]
\qed



\begin{remark}
If in Theorem \ref{th:conv_rate_restarts} we use a tighter inequality   \eqref{eq:sectermErhs} instead of
\eqref{eq:sectermErhs_restarts} (as in Theorem \ref{th:conv_rate}), then
the estimations on the $\Delta$ and $M_{2,\delta}$   can be improved.
Choosing $u = (x^*, y^*)$ we can provide exponentially decreasing sequence of $\D^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate} and get 
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} $\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\e^{2-1/\gamma}}{M_2\sqrt{d}}$
    \item under Assumption \ref{ass:Lip_noise} 
$M_{2,\delta} \lesssim \frac{\mu_{\gamma}^{1/\gamma}\e^{1-1/\gamma}}{\sqrt{d}}$.
\end{enumerate}

\end{remark}







==> restarts_new.tex <==
\section{Restarts}\label{sec:rest}
In this section, we assume that we  additionally have the $r-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems).  For such a case, we apply the restart technique \cite{juditsky2014deterministic} to  Algorithm \ref{alg:zoSPA} 
\begin{assumption}[$r-$growth condition]\label{ass:strongly_convex}
There is $r \geq 1$ and $\mu_{r} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
\[\frac{\mu_{r}}{2} \|z-z^{\star}\|_p^{r}
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right),
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
\]
where $(x^*,y^*)$ is a solution of problem \eqref{eq:min_max_problem}.
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
Then the following holds for $ \hat{\e}_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$, where   $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ is the output of   Algorithm \ref{alg:zoSPA},  
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \hat{\e}_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \hat{\e}_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement is true
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\E\left[\hat{\e}_{\rm sad}(\hat z^N)\right]\leq\e$  after 
% \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\D^{-2}\e^2)^2 \right)\]
\[N =  \O\left( {da_q^2M_2^2\D^2}/{\e^{2}} \right)\]
iterations. If also Assumption \ref{ass:strongly_convex} is satisfied for $r \geq 2$ we can apply restarts and to achieve $\E[\hat{\e}_{\rm sad}] \leq \varepsilon$ in $N_{acc}$ iterations where $N_{acc}$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N_{acc} = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \varepsilon^{2(r-1)/r}} \right).
 \end{align}
\end{theorem}


% \begin{corollary}\label{cor:bound_noise_restarts}
% Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}, and 
% let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement is true
% \begin{enumerate}
%     \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
%     \item Assumption \ref{ass:Lip_noise} holds and 
%  $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
% \end{enumerate}
% then 
% for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\E\left[\e_{\rm sad}(\hat z^N)\right]=\e$  after 
% % \[N =  \O\left( \frac{\D^2}{M_2^2\e^2}(1 + ca_q^2dM_2^2 + d^2a_q^2\D^{-2}\e^2)^2 \right)\]
% \[N =  \O\left( {da_q^2M_2^2\D^2}/{\e^{2}} \right)\]
% iterations, where 
%  $\sqrt{\E \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
% % \begin{enumerate}
% %     \item 
%     % under Assumption \ref{ass:err_noise}
%     % \[\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O \left( \frac{\e}{M_2} \right) \] 
  
%     % \item under Assumption \ref{ass:Lip_noise}
%     %   \[\delta(z) =\O\left( \frac{\e}{\D\sqrt{ d}}\right), \quad \mbox{ and  } \quad \tau = \O\left( \frac{\e}{M_2} \right) \] 
% %\end{enumerate}
% % where $\e = \max\limits_{y\in \Y}  f(\hat x^N, y) - \min\limits_{x\in \X}   f(x, \hat y^N)$ and $(\hat x^N, \hat y^N,)$ are the outputs of the    Algorithm \ref{alg:zoSPA} after 
% % \[N = \O\left( {M^2\D^2(1+ca_q^2d)^2}{\e^{-1}} \right)\]
% % iterations.
% \end{corollary}

% \begin{remark}
% An important particular case of Theorem~\ref{th:conv_rate_restarts} is when $\gamma = 1$. Under this assumption the estimate on the number of iteration $\eqref{eq:estim_iter_restart}$ can be rewritten in the following form:
%  \begin{align}
%      N = \widetilde \O\left(\frac{64 \cdot A^2}{\mu_{1}^2 } \right) = \widetilde \O\left(\frac{A^2}{\mu_{1}^{2} } \right).
%  \end{align}
% As a result, it leads us to the linear convergence of the algorithm for non-smooth convex-concave saddle points problems with sharp saddle-point. For convex optimization problems with sharp minimum this effect was known \cite{juditsky1993stochastic}.
% \end{remark}



%  \iffalse

\textit{Proof of  Theorem \ref{th:conv_rate_restarts}}
~We repeat the proof of Theorem \ref{th:conv_rate}, except that now $z^1$ can be chosen in a stochastic way. Moreover, now we use a rougher inequality instead of \eqref{eq:sectermErhs}
\begin{align}\label{eq:sectermErhs_restarts}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq  {\D}/{\sqrt{d}}.
\end{align}
{\bf Step 1.} (under Assumption \ref{ass:err_noise}) \\
Taking the expectation in \eqref{eq:exEeqE1}, choosing $(x,y) = (x^{\star}, y^{\star})$, and
 learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq cda_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}$  we get
 \begin{align} \label{rate:restarts1}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  
     %\frac{V_{z^1}(u)(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E [V_{z^1}(z^{\star})]}
     + \frac{\sqrt{d}\Delta\D}{\tau} 
     +  2\tau M_2.  
 \end{align}
 {\bf Step 2.} (under Assumption \ref{ass:Lip_noise})\\
Taking the expectation in \eqref{eq:exEeqE}, choosing $(x,y) = (x^{\star}, y^{\star})$, and  learning rate 
 $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d a_q^2(M_2^2+M_{2,\delta}^2)$  we obtain
 \begin{align} \label{rate:restarts2}
      \E\left[ f\left( \hat x^N,y^{\star}\right) -   f\left(x^{\star}, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E [V_{z^1}(z^{\star})]}  + M_{2,\delta}\sqrt{d} \D  
     +  2\tau M_2.  
 \end{align}
{\bf Step 3.} (Restarts)\\
Now let $\tau$ be chosen as $\tau = \O\left(\e/M_2\right)$, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If one of the two following statement holds
\begin{enumerate}
    \item Assumption \ref{ass:err_noise} holds  and $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
    \item Assumption \ref{ass:Lip_noise} holds and 
 $M_{2,\delta} =\O\left( \frac{\e}{\D \sqrt{ d}}\right) $
\end{enumerate}
then using \eqref{rate:restarts1} we obtain the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &= \widetilde \O\left(\frac{a_q M_2 \sqrt{d}}{\sqrt{N_1}}\sqrt{\E [V_{z^1}(z^{\star})]}\right).
 \end{align}
  In this step we will employ the restart technique that is a generalization of the technique proposed in \cite{juditsky2014deterministic}.\\
 For the l.h.s. of Eq. \eqref{restart:rate} we use the Assumption \ref{ass:strongly_convex}. For the r.h.s. of Eq. \eqref{restart:rate} we use $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$  from  \citet[Remark 3]{gasnikov2018universal}  
 \begin{align}\label{restart:norms}
 \frac{\mu_{r}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{r}\right]
 &\leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] = \widetilde \O\left(\frac{a_q M_2 \sqrt{d}}{\sqrt{{N_1}}} \sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
 Then the l.h.s of Eq. \eqref{restart:norms} we  use the Jensen inequality and  get the following
 \begin{align}
 \frac{\mu_{r}}{2} \left({\E\left[\|z^{N_1} - z^{\star}\|_p^2\right]}\right)^{r/2} &\leq   \frac{\mu_{r}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{r}\right] \leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right] \notag\\
     &= \widetilde \O\left( \frac{a_q M_2 \sqrt{d}}{\sqrt{{N_1}}} \sqrt{\E\left[\|z^1 -z^{\star}\|_p^2\right]}\right).
 \end{align}
Finally, 
let us introduce $R_k \triangleq \sqrt{\E\left[\|z^{N_k} - z^{\star}\|_p^2\right]}$ and $R_0 \triangleq \sqrt{\E\left[\|z^{1} - z^{\star}\|_p^2\right]}$. Then we
take ${N_1}$ so as to halve the distance to the solution and get
 $$ {N_1} = \widetilde \O \left( \frac{a_q^2 M_2^2 d}{\mu_{r}^2 R_1^{2(r-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ similarly: we halve the distance $R_1$ to the solution, and so on. \\
 Thus, after $k$  restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N_{acc} = N_1 +\dots + N_k = \widetilde \O \left(\frac{ 2^{2(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}}\left(1+2^{2(r-1)} + \dots + 2^{2(k-1)(r-1)}\right) \right).
 \end{align} 
 Now we need  to determine the number of restarts. To do  this, we fix the desired accuracy  and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\hat{\e}_{\rm sad}] =  \widetilde \O \left(\frac{\mu_{r} R_k^{r}}{2}\right)=   \widetilde \O\left( \frac{ a_q M_2 \sqrt{d} }{\sqrt{N_k}}  R_{k-1}\right) = \widetilde \O \left(\frac{\mu_{r}R_0^{r}}{2^{kr}}\right)  \leq \e.
 \end{align} 
 Then to fulfill this condition, one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{r}R_0^{r}/\e\right)) / r$ and using Eq. \eqref{restart:N} we get the total number of iterations
\[ N_{acc} = \widetilde \O\left(\frac{ 2^{2k(r-1)}a_q^2 M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}} \right) = \widetilde \O\left(\frac{a_q^2 M_2^2 d}{\mu_{r}^{2/r} \e^{2(r-1)/r}} \right).\]
\qed


\begin{remark}
If in Theorem \ref{th:conv_rate_restarts}, we use a tighter inequality   \eqref{eq:sectermErhs} instead of
\eqref{eq:sectermErhs_restarts} (as in Theorem \ref{th:conv_rate}), then
the estimations on the $\Delta$ and $M_{2,\delta}$   can be improved.
Choosing $u = (x^*, y^*)$ we can provide exponentially decreasing sequence of $\D^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate} and get 
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} $\Delta \lesssim \frac{\mu_{r}^{1/r}\e^{2-1/r}}{M_2\sqrt{d}}$
    \item under Assumption \ref{ass:Lip_noise} 
$M_{2,\delta} \lesssim \frac{\mu_{r}^{1/r}\e^{1-1/r}}{\sqrt{d}}$.
\end{enumerate}

\end{remark}

% \begin{remark}
% The estimations on the noise $B$ in Eq. \eqref{eq:err_noise_AB} and \eqref{eq:err_noise_AB_2} can be improved in the following way: it is possible to obtain the better evaluation on the r.h.s of Eq. \eqref{eq:sectermErhs_restarts} as
% \begin{align}\label{eq:sectermErhs_restarts_new}
%   \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|_2  \right] \leq {\|z^k - u\|}/{\sqrt{d}}. 
% \end{align}
% Choosing $u = (x^*, y^*)$ we provide exponentially decreasing sequence of $\D_2^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate}. It leads us to the more precise estimation on the noise $B$. We use this estimation on $B$ when we employ the restart technique in the proof of Theorem~\ref{th:conv_rate_restarts} and, thanks to this, we obtain the better estimate on the maximal level of noise: under Assumption \ref{ass:err_noise} $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{2-1/\gamma}}{M_2\sqrt{d}}$$  and 
% under Assumption \ref{ass:Lip_noise} 
% $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{1-1/\gamma}}{\sqrt{d}}.$$
% \end{remark}

\begin{remark}\label{hpb}
Based on high-probability bound  we can obtain high-probability bound by using the same restart-technique \cite{juditsky2014deterministic}. In the case $r = 2$ it is probably possible to improve this bound in $\log \varepsilon^{-1}$ factor by using alternative algorithm \cite{harvey2019tight}. 
\end{remark}
% \fi

\begin{theorem}\label{th:conv_rate_restarts_prob} 
Let function $f(x,y,\xi)$  satisfy the Assumption \ref{ass:uni_Lip_obj} and Assumption \ref{ass:err_noise} for some constant $c$. Let the learning rate of Algorithm \ref{alg:zoSPA} is chosen as  $\gamma_k 
=\frac{\D}{M}\sqrt{\frac{2}{N}}$, where  $N$ is the number of iterations and $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$. Then for the output $  (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA},  the following holds
% \begin{align}
%       \Prob & \left\{ \e_{\rm sad} (\hat z^N)  \geq \frac{4 \Omega^2 \sqrt{d} \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2 d^2}{M}   + \right. \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 d^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
%       & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} 
% \end{align}
\begin{align}
       &\Prob  \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{  \mathcal D M  }{\sqrt{N}}   + \frac{ \Omega \D \sqrt{d} \Delta }{\tau } +2 \tau M_2 + \right. \nonumber\\
      & \left.  + \Omega \frac{2 \sqrt{2} M \D}{c N}   \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} \label{eq:convergrate_prob_restarts}.
\end{align}

 Let $\tau$  be chosen as $\tau = \O\left(\e/M_2\right)$ in randomized smoothing \eqref{eq:smoothedfunc}, where $\e$ is the desired accuracy to solve problem \eqref{eq:min_max_problem}. If also Assumption \ref{ass:err_noise} holds true with $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$
then 
for the output  $  \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA}, it holds   $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$ after 
\[N =  \O\left( {d M_2^2\D^2}/{\e^{2}} \right)\]
iterations. If moreover Assumption \ref{ass:strongly_convex} is satisfied we can apply restarts and to achieve $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$ in $N_{acc}$ iterations where $N_{acc}$ is given by
 \begin{align}\label{eq:estim_iter_restart_prob}
     N_{acc} = \widetilde \O\left(\frac{M_2^2 d}{\mu_{r}^{2/r} \varepsilon^{2(r-1)/r}} \right).
 \end{align}
\end{theorem}

\begin{proof}
We recall inequality \eqref{eq:dghjsklslsl_proba} from Theorem \ref{th:conv_rate_prob}:
\begin{align}
       &\Prob  \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \|z^1 -z^{\star}\|_p M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{2  M_2^2 d \sum_{k=1}^N \gamma_k^2}{c \sum_{k=1}^N \gamma_k }  \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2  M_2^2 d \sqrt{\sum_{k=1}^N \gamma_k^4}}{c \sum_{k=1}^N \gamma_k } +  \frac{d^2\Delta^2 \sum_{k=1}^N \gamma_k^2}{2 \tau^2 \sum_{k=1}^N \gamma_k } + \frac{ \|z^1 -z^{\star}\|_p^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
      & \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \}\label{eq:dghjsklslsl_proba_restarts}.
\end{align}
%  \begin{align}
%       \Prob & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } +\frac{d \D \Delta}{\tau} \right. \nonumber\\
%       & \left.+ \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
%       & \hspace{5cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} \label{eq:dghjsklslsl_proba}
% \end{align}
 Choosing  learning rate $\gamma_k 
=\frac{\|z^1 -z^{\star}\|_p}{M}\sqrt{\frac{2}{N}}$ with $M^2 \triangleq d M_2^2+d^2 \Delta^2 \tau^{-2}$ in Eq. \eqref{eq:dghjsklslsl_proba_restarts} we obtain

\begin{align}
       \Prob & \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \frac{4 \Omega^2 \sqrt{d} \|z^1 -z^{\star}\|_p M_2  }{\sqrt{N}} + \frac{2 \sqrt{2}  \|z^1 -z^{\star}\|_p M_2^2 d}{c M\sqrt{N}}   + \right. \nonumber\\
      & \hspace{3cm}\left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{2 \sqrt{2} M_2^2 d\|z^1 -z^{\star}\|_p}{c M N} +  \frac{d^2\Delta^2 \sqrt{2} \D}{2 \tau^2 M \sqrt{N} }+ \frac{\|z^1 -z^{\star}\|_p M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
      & \hspace{2cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .
\end{align}
Using the notation of $M$ we obtain:
\begin{align}
       &\Prob  \left\{ f\left( \hat x^N,y^{\star}\right) -  f\left(x^{\star}, \hat y^N \right) \geq \left(4 \Omega^2 + \frac{2 \sqrt{2}}{c} + \frac{2}{\sqrt{2}}\right) \frac{\|z^1 -z^{\star}\|_p M  }{\sqrt{N}}   + \frac{ \Omega \D \sqrt{d} \Delta }{\tau } +2 \tau M_2 + \right. \nonumber\\
      & \left. + \Omega \frac{2 \sqrt{2} M \|z^1 -z^{\star}\|_p}{c N}    \right\}  \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 6 \exp \{-\Omega/4 \} .\label{eq:conv_proba}
\end{align}
{\bf Step 3.} (Restarts)\\
In this step we will employ the restart technique that is generalization of technique proposed in \cite{juditsky2014deterministic}.
Before we need to get a more compact convergence result in the form $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$. For this we fix $\sigma > 0$ and let $\tau$ be chosen as $\tau = \O\left(\e/M_2\right)$. If moreover Assumption \ref{ass:err_noise} holds true with $\Delta =\O\left( \frac{\e^2}{\D M_2\sqrt{ d}}\right)$, then using \eqref{eq:conv_proba} we obtain 
 \begin{align}\label{restart:rate_prob}
     \Prob & \left\{ f\left( \hat x^{N_1},y^{\star}\right) -  f\left(x^{\star}, \hat y^{N_1} \right) = \widetilde \O_1\left(\ M_2 \sqrt{d}\frac{\|z^1 -z^{\star}\|_p }{\sqrt{N_1}}  \right)   \right\}  \geq 1 - \sigma_1.
 \end{align}
 We note that now the notation $\widetilde \O_1$ contains the factor $\log \sigma_1^{-1}$.
 
  For the l.h.s. of Eq. \eqref{restart:rate_prob} we use Assumption \ref{ass:strongly_convex} then with probability at least $1 - \sigma_1$ 
 \begin{align}\label{restart:norms_prob}
 \frac{\mu_{r}}{2} \underbrace{\|z^{N_1} - z^{\star}\|_p^{r}}_{R_1^r}
 &\leq
     f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right) = \widetilde \O\left(\ M_2 \sqrt{d}\frac{\|z^1 -z^{\star}\|_p }{\sqrt{N_1}} \right).
 \end{align}
 Then taking ${N_1}$ so as to reduce the distance to the solution by half, we obtain
 $$ {N_1} = \widetilde \O_1 \left( \frac{M_2^2 d}{\mu_{r}^2 R_1^{2(r-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ from a similar condition for reducing the distance $R_1$ to the solution by a factor of $2$, and so on.  We remind that at each restart step $i \in \{1,k\}$, the resulting formula \eqref{restart:norms_prob} is valid only with probability $1 - \sigma_i$. Thus, we choose $\sigma_i = \sigma/k$ and then by the union bound inequality all inequalities are satisfied simultaneously with probability at least $1 - \sigma$. We will determine the number of restarts further, but at this stage we use the fact that $k$ depends on the accuracy only logarithmically, which entails that $\forall i\in \{1,k\} \;\;  \widetilde \O_i = \widetilde \O$.
 
 Thus, after $k$ of such restarts, the total number of iterations will be
 \begin{align} \label{restart:N_prob}
     N_{acc} = N_1 +\dots + N_k = \widetilde \O \left(\frac{ 2^{2(r-1)}M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}}\left(1+2^{2(r-1)} + \dots + 2^{2(k-1)(r-1)}\right) \right).
 \end{align} 
 It remains for us to determine the number of restarts, for this we fix the desired accuracy in terms of $\Prob\left\{\hat{\e}_{\rm sad}(\hat z^N) \leq \e \right\} \geq 1 - \sigma$ and using the inequality \eqref{restart:norms_prob} we obtain 
 \begin{align}\label{restart:epsilon_prob}
     \hat{\e}_{\rm sad} = \widetilde \O \left(\frac{\mu_{r} R_k^{r}}{2}\right)=   \frac{ M_2 \sqrt{d} \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{r}R_0^{r}}{2^{kr}}\right) \leq \varepsilon.
 \end{align} 
 Then to fulfill this condition one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{r}R_0^{r}/\varepsilon\right)) / r$ and using Eq. \eqref{restart:N} we get the total number of iterations
\[ N_{acc} = \widetilde \O\left(\frac{2^{2k(r-1)}M_2^2 d}{\mu_{r}^2 R_0^{2(r-1)}} \right) = \widetilde \O\left(\frac{M_2^2 d}{\mu_{r}^{2/r} \varepsilon^{2(r-1)/r}} \right).\]
  


\end{proof}




==> restarts_prob.tex <==
\section{Restarts and Linear Convergence Rate}\label{sec:rest}
In this section we apply restart-technique \cite{juditsky2014deterministic} to  Algorithm\ref{alg:zoSPA} in the case when we additionally have $r-$growth condition for duality gap (see, \cite{shapiro2021lectures} for convex optimization problems). 
\begin{assumption}\label{ass:strongly_convex}
There is $r \geq 1$ and $\mu_{r} > 0$ such that for all $z = (x,y) \in \Z \triangleq \X \times \Y$
$$ \frac{\mu_{r}}{2} \|z-z^{\star}\|_p^{r} 
\leq f\left(  x,y^{\star}\right) -  f\left(x^{\star},  y \right).
% \leq f^\tau\left(  x,y^{\star}\right) -  f^\tau\left(x^{\star},  y \right).
$$
\end{assumption}

\begin{theorem}\label{th:conv_rate_restarts} 
Let  $f(x,y,\xi)$  satisfy the Assumption \ref{ass:Lip_obj}. 
Then for the output $ \hat z^N \triangleq (\hat x^N, \hat y^N)$ of   Algorithm \ref{alg:zoSPA},  the following holds for $ \e_{\rm sad}  \triangleq   f(\hat x^N, y^{\star}) -    f(x^{\star}, \hat y^N)$
\begin{enumerate}
    \item under Assumption \ref{ass:err_noise} and learning rate $\gamma_k 
=\frac{\sqrt {\E [V_{z^1}(z^{\star})]}}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case1}^2\triangleq \O\left(da_q^2M_2^2 + d^2a_q^2\Delta^2\tau^{-2}\right)$ 
 \begin{align}\label{eq:convergrate0_restarts}
      \E\left[ \e_{\rm sad}\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case1}\sqrt{\E[V_{z^1}(z^{\star})]}
     + {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2.    
 \end{align}
    \item under Assumption \ref{ass:Lip_noise}  and  learning rate $\gamma_k 
=\frac{\sqrt{\E [V_{z^1}(z^{\star})]}}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with \\ $M_{\rm case2}^2 \triangleq \O\left( d a_q^2\left(M_2^2+M_{2,\delta}^2\right)\right)$
    \begin{equation}\label{eq:convergrate_restarts}
     \E\left[ \e_{\rm sad}\right]
     \leq  \sqrt{\frac{2}{N}}M_{\rm case2}\sqrt{\E[V_{z^1}(z^{\star})]}  + M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2,
\end{equation}
\end{enumerate}
where 
 $a_q^2$ is such that $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$. 
 
 Moreover, if Assumption \ref{ass:strongly_convex} is satisfied we can apply restarts and to achieve $\E[\e_{\rm sad}] \leq \varepsilon$ one need $N$ iterations where $N$ is given by
 \begin{align}\label{eq:estim_iter_restart}
     N &= \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right),\\
     N &\leq  \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right),
 \end{align}
 where $B$ is an inaccuracy associated with the $\tau$-smoothing and inexactness of the oracle. 
 Constants $A, B$ depend on noise conditions and are given by the following equality
 \begin{enumerate}
    \item under Assumption \ref{ass:err_noise} 
 \begin{align}\label{eq:err_noise_AB}
      A = \sqrt{2} M_{\rm case1}, \;\;\; B = {\Delta\D\sqrt{d}}{\tau^{-1}} 
     +  2\tau M_2,
 \end{align}
    \item under Assumption \ref{ass:Lip_noise} 
    \begin{align}\label{eq:err_noise_AB_2}
      A = \sqrt{2} M_{\rm case2}, \;\;\; B = M_{2,\delta} \D \sqrt{d} 
     +  2\tau M_2.
 \end{align}
\end{enumerate}
Thus, from \eqref{eq:err_noise_AB} $\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon^2/\left(\D M_2\sqrt{d}\right)\right)$ and from \eqref{eq:err_noise_AB_2}
$\tau = O\left(\varepsilon/M_2\right)$, $\Delta = O\left(\varepsilon/\left(\D\sqrt{d}\right)\right)$.
\end{theorem}

\begin{remark}
An important particular case of Theorem~\ref{th:conv_rate_restarts} is when $\gamma = 1$. Under this assumption the estimate on the number of iteration $\eqref{eq:estim_iter_restart}$ can be rewritten in the following form:
 \begin{align}
     N = \widetilde \O\left(\frac{64 \cdot A^2}{\mu_{1}^2 } \right) = \widetilde \O\left(\frac{A^2}{\mu_{1}^{2} } \right).
 \end{align}
As a result, it leads us to the linear convergence of the algorithm for non-smooth convex-concave saddle points problems with sharp saddle-point. For convex optimization problems with sharp minimum this effect was known \cite{juditsky1993stochastic}.
\end{remark}



%  \iffalse

\begin{proof}[Proof of the  Theorem \ref{th:conv_rate_restarts}]

The proof is based on the proof of Theorem~\ref{th:conv_rate_prob}. In the first $3$ steps, we obtain an estimate of type \eqref{eq:convergrate_prob} with a more detailed  dependence on the choice of the initial point $z_1$. Then we apply the restart technique to the obtained convergence rate.

By the definition $z^{k+1}= {\rm Prox}_{z^k}\left(\gamma_k g(z^k,\be^k,\xi^k) \right)$ we get  \cite{ben2001lectures}, for all $u\in \Z$
\begin{align}
   \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \leq V_{z^k}(u) - V_{z^{k+1}}(u) - \gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2   \notag
\end{align}
Summing for $k=1,\dots,N$ we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE_prob:rst}
   \sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra 
   &\leq V_{z^1}(u)  - \sum_{k=1}^N\gamma_k^2\|g(z^k,\be^k,\xi^k)\|_q^2/2  \notag\\
   &\leq  V_{z_1}(u) + \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_q^2.
\end{align}
where $z^1$ can be chosen in stochastic way.

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE_prob:rst}, invoking Assumtion \ref{ass:uni_Lip_obj}, the random variables $\phi_k = \gamma_k^2 \|g(z^k,\be^k,\xi^k)\|_q^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$ satisfy the premise of case B of Lemma 2 from \cite{lan2012validation} with $\sigma_k = 4 N^{2/q -1} M_2^2 \gamma_k^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1}$:
\begin{align*}
    & \E_{|t-1} \left[ \exp \{|\phi_k|/\sigma_k\} \right] = \E_{|t-1} \left[ \exp \{ \|g(z^k,\be^k,\xi^k)\|_q^2/4 N^{2/q -1} M_2^2\} \right] \leq  /* \mbox{ Holder's inequality} */ \\
    & \leq \E_{|t-1} \left[ \exp \{ 
    \|g(z^k,\be^k,\xi^k)\|_2^2/4M_2^2\} \right] \leq \exp \{1\}
\end{align*}

Invoking case B of Lemma 2 from \cite{lan2012validation}, we get
\small{
\begin{align}
    &\text{Prob} \left\{ \left| \sum_{k=1}^N \gamma_k^2 \|g(z^k,\be^k,\xi^k)\|_q^2 \left( \sum_{k=1}^N \gamma_k \right)^{-1} \right| > \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } + \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } \right\} \nonumber \\
    & \hspace{8 cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} \label{eq:first_step_var:rst}
\end{align}}





{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE_prob:rst}, we provide the new definition of gradient approximation of $\nabla f(z, \xi)$ following the Eq. $\eqref{eq:grad_approx}$:
\begin{equation}\label{eq:grad_approx_f:rst}
    g_f(z,\xi, \be) = \frac{d}{2\tau}\left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)   \right) \begin{pmatrix} \be_x \\ -\be_y \end{pmatrix},
\end{equation}

Using the notation \eqref{eq:grad_approx_f:rst} we rewrite the l.h.s. of  Eq. \eqref{eq:inmainsqE_prob:rst} as following:

\begin{align}
    &\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra =\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \nonumber\\
    & + \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra + \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra \label{eq:step2_rewriten:rst}
\end{align}
\begin{enumerate}
    \item For the first term in r.h.s. of  Eq. \eqref{eq:step2_rewriten:rst}, we use Assumption \ref{ass:uni_Lip_obj} and provide the following notions:
$$\sigma_k = \gamma_k M_2 2 \mathcal D,$$
$$\phi_k (\xi_k)= \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra .$$
Moreover, using the notion of $\omega$-diameter of $\Z$ we have that:
\begin{align*}
  \E_{|k-1} &\left[ \exp \left\{ \phi_k^2/ \sigma_k^2 \right\} \right] = \underbrace{\E_{|k-1} \left[ \exp \left\{ \left(\gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra \right)^2/ \left(  \gamma_k M_2 2 \mathcal D \right)^2 \right\} \right]}_{\leq \exp \{1\}}.  
\end{align*}
It follows by case A of Lemma 2 from \cite{lan2012validation} that
\begin{align}
    \text{Prob} \left\{ \left| \frac{\sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z) , z^k-u\ra}{\sum_{k=1}^{N}\gamma_k}  \right| > \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} \right\} \leq 2 \exp \left\{ -\frac{\Omega^2}{3} \right\} . \label{eq:step2_martingale_rewriten:rst}
\end{align}
\item For the second term in r.h.s of Eq. \eqref{eq:step2_rewriten:rst} under the Assumption \ref{ass:err_noise} we obtain :
\begin{align}
    & \sum_{k=1}^N \gamma_k\la \frac{d}{2\tau} (\delta(z^k+\tau \be) - \delta(z^k-\tau \be)) \be   , z^k-u\ra \geq - \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left|\la \be, z^k-u \ra \right| \label{eq:step2_delta_rewriten:rst}
\end{align}
Using the Poincaré's lemma from \cite{lifshits2012lectures} paragraph 6.3 we rewrite $\be$ in different form:
\begin{align}\label{eq:poincare_def_e:rst}
    \be \stackrel{D}{=} \frac{\eta}{\sqrt{\eta_1^2 + \dots + \eta_d^2}},
\end{align}

where $\eta = \left( \eta_1, \eta_2, \dots , \eta_d \right)^T = \mathcal{N} \left( 0 , I_d \right)$. 
Using Lemma 1 \cite{laurent2000adaptive}
% \cite{boucheron2013concentration} 
it follows:
\begin{align}
    \text{Prob} \left\{  \sum_{k=1}^d \left|\eta_k\right|^2 \le d -  2 \sqrt{\Omega d} \right\} \leq  \exp \{- \Omega \} . \label{eq:step2_sphere_rewriten:rst}
\end{align}
Using the definition of $\eta$ we obtain:
\begin{align}
    \la \eta, z^k-u \ra \stackrel{d}{=} \mathcal{N} \left( 0 , \|z^k - u\|^2 \right). \label{eq:step2_poincare:rst}
\end{align}
Using Eq. \eqref{eq:step2_sphere_rewriten:rst}, \eqref{eq:step2_poincare:rst} and \eqref{eq:poincare_def_e:rst} we can estimate the r.h.s of Eq. \eqref{eq:step2_delta_rewriten:rst}:
\begin{align}
    \text{Prob} &\left\{   \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \left| \la \be, z^k-u \ra \right| > \frac{ \Omega \D \sqrt{d} \Delta \sum_{k=1}^N \gamma_k}{\tau} \right\} \nonumber\\
    &\leq 3 \exp \{-\Omega/4 \} . \label{eq:step2_sphere_rewriten_2:rst}
\end{align}
\item We rewrite the third term in r.h.s. of  Eq. \eqref{eq:step2_rewriten:rst} in the following form: 
\begin{align} 
    \sum_{k=1}^N \gamma_k\la \nabla f^{\tau} (z^k) , z^k-u\ra & =  \sum_{k=1}^N \gamma_k \left\la \begin{pmatrix} \nabla_x f^\tau(x^k, y^k) \\ -\nabla_y  f^\tau(x^k,y^k) \end{pmatrix}, \begin{pmatrix} x^k-x \\ y^k-y \end{pmatrix} \right\ra  \notag \\
     &=  \sum_{k=1}^N \gamma_k\left( \la \nabla_x f^\tau(x^k,y^k), x^k-x \ra  -  \la \nabla_y  f^\tau(x^k,y^k), y^k-y \ra \right) \notag \\
     &\geq  \sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))  -  ( f^\tau(x^k,y^k) - f^\tau(x^k,y)) \notag \\
     &=  \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \label{eq:eqexpfxy_prob:rst}.
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE_prob:rst}
     \frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k))  &\leq  f^\tau\left(\frac{\sum_{k=1}^N \gamma_k x^k}{\sum_{k=1}^{N}\gamma_k},y\right)  - f^\tau\left(x, \frac{\sum_{k=1}^N \gamma_k y^k}{\sum_{k=1}^{N}\gamma_k}\right)\notag \\
     &=  f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) ,
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm \ref{alg:zoSPA}. 
Using Eq. \eqref{eq:fineqE_prob}  for Eq. \eqref{eq:eqexpfxy_prob:rst} we get 
\begin{align}\label{eq:fpslff_prob:rst}
      \sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra  
     &\geq  \sum_{k=1}^{N}\gamma_k \left( f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right) .
\end{align}
\end{enumerate}









{\bf Step 3.} \\
Then we use this with  Eq. \eqref{eq:step2_rewriten:rst}, \eqref{eq:step2_delta_rewriten} and \eqref{eq:fpslff_prob:rst} for Eq. \eqref{eq:inmainsqE_prob:rst} and obtain
\begin{align}
      &f^\tau\left( \hat x^N,y\right)   - f^\tau\left(x, \hat y^N \right)  \leq   \frac{\D^2}{\sum_{k=1}^{N}\gamma_k } + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \frac{\gamma_k^2}{2} \|g(z^k,\be^k,\xi^k)\|_q^2  \nonumber \\
    & - \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k\la g_f(z^k,\be^k,\xi^k) - \nabla f^{\tau} (z^k) , z^k-u\ra + \left(\sum_{k=1}^{N}\gamma_k \right)^{-1} \sum_{k=1}^N \gamma_k \frac{d \Delta}{\tau} \la \be, z^k-u \ra \label{eq:exEeqE_prob:rst}
\end{align}


 For the l.h.s. of Eq. \eqref{eq:exEeqE_prob:rst} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2 \label{eq:f_tau_to_f:rst}
 \end{align}
 Using Eq. \eqref{eq:f_tau_to_f:rst}, \eqref{eq:step2_martingale_rewriten:rst},  \eqref{eq:first_step_var:rst}, \eqref{eq:step2_sphere_rewriten_2:rst} and taking the maximum in $(x,y) \in (\X,\Y)$, we obtain we can rewrite Eq. \eqref{eq:exEeqE_prob:rst} as follow:
 
 \begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k }  \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
      & \hspace{3cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} + 3 \exp \{-\Omega/4 \}. \label{eq:dghjsklslsl_proba:rst}
\end{align}
%  \begin{align}
%       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  \sqrt{  \sum_{k=1}^N \gamma_k^2 }}{{\sum_{k=1}^{N}\gamma_k}} + \frac{4 N^{2/q -1} M_2^2 \sum_{k=1}^N \gamma_k^2}{ \sum_{k=1}^N \gamma_k } +\frac{d \D \Delta}{\tau} \right. \nonumber\\
%       & \left.+ \Omega \frac{4 N^{2/q -1} M_2^2 \sqrt{\sum_{k=1}^N \gamma_k^4}}{ \sum_{k=1}^N \gamma_k } + \frac{\D^2}{\sum_{k=1}^{N}\gamma_k }  +2 \tau M_2 \right\} \notag\\
%       & \hspace{5cm}\leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} +  2 \exp \{-\Omega^2/3 \} \label{eq:dghjsklslsl_proba}
% \end{align}

 Choosing the learning rate $\gamma_k 
=\frac{\D}{M}\sqrt{\frac{2}{N}}$ with $M^2 \triangleq (M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl_proba:rst} we obtain
\begin{align}
       \text{Prob} & \left\{ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right) \geq \frac{4 \Omega \mathcal D M_2  }{\sqrt{N}} + \frac{4 \sqrt{2} N^{2/q -3/2} \D M_2^2}{M}   + \right. \nonumber\\
      & \left. \frac{ \Omega \D \sqrt{d} \Delta }{\tau } + \Omega \frac{4 \sqrt{2} N^{2/q -2} M_2^2 \D}{ M} + \frac{\D M}{\sqrt{2N} }  +2 \tau M_2 \right\} \nonumber\\
      & \hspace{3cm} \leq \exp \{-\Omega^2/12 \} + \exp \{-3\sqrt{N} \Omega/4 \} + 2 \exp \{-\Omega^2/3 \} + 3 \exp \{-\Omega/4 \} 
\end{align}









 {\bf Step 5.} (Restart)
 At the previous step, we obtained the convergence rate of the following form
 \begin{align}\label{restart:rate}
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq  \frac{A\sqrt{\E [V_{z^1}(z^{\star})]}}{\sqrt{N_1}}  + B,  
 \end{align}
 with an appropriate choice of constants $A, B$. Here $B$ is an inaccuracy associated with the stochastic setting of the problem and inexactness of the oracle. In this step we will employ the restart technique that is generalization of technique proposed in \cite{juditsky2014deterministic}.
 
 For the r.h.s. of Eq. \eqref{restart:rate} we use Assumption \ref{ass:strongly_convex} and the fact of remark 3 from \cite{gasnikov2018universal} that $V_{z^1}(z^{\star}) = \widetilde \O (\|z^1 -z^{\star}\|^2_p)$ for the l.h.s 
 \begin{align}\label{restart:norms}
 \underbrace{\frac{\mu_{\gamma}}{2} \E\left[  \|z^{N_1} - z^{\star}\|_p^{\gamma}\right]}_{\geq\frac{\mu_{\gamma}}{2} \E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}
 \leq
     \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq A\widetilde \O(\underbrace{\E[\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}  + B.
 \end{align}
 Then by choosing ${N_1} \leq \frac{A^2\widetilde \O(R_0^2)}{B^2}$ and applying the Jensen inequality for l.h.s of Eq. \eqref{restart:norms} we get
 \begin{align}
 \frac{\mu_{\gamma}}{2} \underbrace{\E\left[\|z^{N_1} - z^{\star}\|_p\right]^{\gamma}}_{R_1^{\gamma}} \leq \E\left[ f\left( \hat x^{N_1},y^{\star}\right) -   f\left(x^{\star}, \hat y^{N_1} \right)\right]
     &\leq 2A\widetilde \O(\underbrace{\E [\|z^1 -z^{\star}\|_p]}_{R_0})/\sqrt{{N_1}}.
 \end{align}
 And finally taking ${N_1}$ so as to reduce the distance to the solution by half, we obtain
 $$ {N_1} = \widetilde \O \left( \frac{64A^2}{\mu_{\gamma}^2 R_1^{2(\gamma-1)}} \right).$$
 Next, after $N_1$ iterations, we restart the original method and set $z^1 = z^{N_1}$. We determine $N_2$ from a similar condition for reducing the distance to the solution by a factor of $2$, and so on. 
 
 Thus, after $k$ of such restarts, the total number of iterations will be
 \begin{align} \label{restart:N}
     N = N_1 +\dots + N_k = \widetilde \O \left(\frac{64 \cdot 2^{2(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}}\left(1+2^{2(\gamma-1)} + \dots + 2^{2(k-1)(\gamma-1)}\right) \right).
 \end{align} 
 It remains for us to determine the number of restarts, for this we fix the desired accuracy in terms of $\E[\e_{\rm sad}] \leq \varepsilon$ and using the inequality \eqref{restart:norms} we obtain 
 \begin{align}\label{restart:epsilon}
     \E [\e_{\rm sad}] = \widetilde \O \left(\frac{\mu_{\gamma} R_k^{\gamma}}{2}\right)=   \frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  = \widetilde \O \left(\frac{\mu_{\gamma}R_0^{\gamma}}{2^{k\gamma}}\right) \leq \varepsilon.
 \end{align} 
 Then to fulfill this condition one can choose $k =  \log_{2} (\widetilde \O\left( \mu_{\gamma}R_0^{\gamma}/\varepsilon\right)) / \gamma$ and using Eq. \eqref{restart:N} we get the total number of iterations
 $$ N = \widetilde \O\left(\frac{64 \cdot 2^{2k(\gamma-1)}A^2}{\mu_{\gamma}^2 R_0^{2(\gamma-1)}} \right) = \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} \varepsilon^{2(\gamma-1)/\gamma}} \right).$$
 Moreover, using ${N_k} \leq \frac{A^2\widetilde \O(R_{k-1}^2)}{B^2}$ and $\frac{2 A \widetilde \O\left(R_{k-1}\right)}{\sqrt{N_k}}  \leq \varepsilon$ from Eq. \eqref{restart:epsilon} we have $B = \tilde{O}(\varepsilon)$.  This condition imposes restrictions on the final accuracy $\varepsilon$ and, as a consequence, on the choice of $N$, given by Eq. \eqref{restart:N}
 \begin{align*}
     N \leq  \widetilde \O\left(\frac{A^2}{\mu_{\gamma}^{2/\gamma} B^{2(\gamma-1)/\gamma}} \right).
 \end{align*}
\end{proof}




\begin{remark}
The estimations on the noise $B$ in Eq. \eqref{eq:err_noise_AB} and \eqref{eq:err_noise_AB_2} can be improved in the following way: it is possible to obtain the better evaluation on the r.h.s of Eq. \eqref{eq:sectermErhs_restarts} as
\begin{align}\label{eq:sectermErhs_restarts_new}
  \E_{\be^k} \left[    \left|\la \be^k, z^k-u\ra\right|  \right] \leq {\|z^k - u\|_2}/{\sqrt{d}}. 
\end{align}
Choosing $u = (x^*, y^*)$ we provide exponentially decreasing sequence of $\D_2^k = \E \|z^k - u\|_2$ in Eq. \eqref{restart:rate}. It leads us to the more precise estimation on the noise $B$. We use this estimation on $B$ when we employ the restart technique in the proof of Theorem~\ref{th:conv_rate_restarts} and, thanks to this, we obtain the better estimate on the maximal level of noise: under Assumption \ref{ass:err_noise} $$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{2-1/\gamma}}{M_2\sqrt{d}}$$  and 
under Assumption \ref{ass:Lip_noise} 
$$\Delta \lesssim \frac{\mu_{\gamma}^{1/\gamma}\varepsilon^{1-1/\gamma}}{\sqrt{d}}.$$
\end{remark}

\begin{remark}\label{hpb}
Based on high-probability bound from Appendix~\ref{H-PB} we can obtain high-probability bound by using the same restart-technique \cite{juditsky2014deterministic}. In the case $\gamma = 2$ it is probably possible to improve this bound in $\log \varepsilon^{-1}$ factor by using alternative algorithm \cite{harvey2019tight}. Moreover, based on stochastic-gradient clipping trick \cite{gorbunov2021near} we can obtain the result in Appendix~\ref{H-PB} in the case when the second moment of stochastic gradient is bounded (subgaussian tails are not required). When the variance of noise is not bounded (the second moment of stochastic gradient is non bounded) the rate of convergence may changes drastically, see the next section.
\end{remark}
% \fi



==> variable_separation.tex <==
\section{Variable Separation}
In this section, 
we assume  proximal setups for spaces $\X$ and $\Y$ can be different.  Thus,  
 we replace the proximal step  $z^{k+1}  \leftarrow {\rm Prox}_{z^k}\left(\gamma_k g(z^k, \xi^k, \be^k)\right)$ on the  space $\Z\triangleq \X \times \Y$ from Algorithm \ref{alg:zoSPA} by two proximal steps on spaces $\X$ and $\Y$:
\begin{align*}
    x^{k+1}  &\leftarrow {\rm Prox}_{x^k}\left(\gamma_k g_x(z^k, \xi^k, \be^k)\right),\\
    y^{k+1}  &\leftarrow {\rm Prox}_{y^k}\left(\gamma_k g_y(z^k, \xi^k, \be^k)\right).
\end{align*}
We also note that we have different Bregman divergence for each space $\X, \Y$ and the step is taken according to the corresponding divergence.



\begin{lemma}\label{lm:shamirEnabla:separated}
 For $g(z,\xi,\be)$ from \eqref{eq:grad_approx}, the following holds
 under Assumption \ref{ass:Lip_obj} 
 \begin{enumerate}
     \item  and Assumption  \ref{ass:err_noise}
     \[\E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} dM_2^2 + {d^2 a_{q_x}^2\Delta^2}{\tau^{-2}},\]
     \item  and Assumption \ref{ass:Lip_noise} 
\[\E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} d (M_2^2+M_{2,\delta}^2),\] 
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E_{\be_x} \left[ \|\be_x\|_{q_x}^4\right]} \leq a_{q_x}^2$.
\end{lemma}

\begin{proof}
\begin{align}\label{eq:sqnormE:separated}
    &\E \left[\|g_x(z,\xi,\be)\|^2_{q_x} \right] = \E\left[ \left\|\frac{d}{2\tau}\left(\vp(z+\tau \be,\xi) - \vp(z-\tau \be,\xi)   \right) \be_x\right\|^2_{q_x} \right] \notag \\
    &= \frac{d^2}{4\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(f(z+\tau \be,\xi) +\delta(z+\tau\be) - f(z-\tau \be,\xi) -\delta(z-\tau\be)  \right)^2 \right] \notag\\
     &= \frac{d^2}{4\tau^2}\left(\E \left[\|\be_x\|_{q_x}^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right] + \E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \right) 
\end{align}
For the first term in the r.h.s. of Eq. \eqref{eq:sqnormE:separated}, the following holds with an arbitrary parameter $\alpha$
\begin{align}\label{eq:fgkbbhgdddgh:separated}
 & \frac{d^2}{4\tau^2}\E \left[\|\be_x\|_{q_x}^2 \left(f(z+\tau \be,\xi) - f(z-\tau \be,\xi)\right)^2\right]  \notag\\
  &= \frac{d^2}{2\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left((f(z+\tau \be,\xi) -\alpha) -(f(z-\tau \be,\xi) - \alpha)   \right)^2 \right] \notag\\
    &\leq \frac{d^2}{2\tau^2}\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 + (f(z-\tau \be,\xi) -\alpha)^2 \right] \quad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
     &=  \frac{d^2}{2\tau^2}\left(\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] + \E \left[\|\be_x\|_{q_x}^2(f(z-\tau \be,\xi) -\alpha)^2 \right] \right) \notag\\
    &= \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
\end{align}
Applying the Cauchy--Schwartz inequality for Eq. \eqref{eq:fgkbbhgdddgh:separated} and using $\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \leq a_{q_x}^2$ we obtain 
\begin{align}\label{eq:funcsq:separated}
     \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 (f(z+\tau \be,\xi)-\alpha)^2 \right] 
     &\leq \frac{d^2}{\tau^2}\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \sqrt{\E \left[ f(z+\tau \be,\xi)-\alpha)^4\right]} \notag\\
     &\leq \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right] . 
\end{align}
Then we assume $\alpha = \E\left[f(z+\tau \be,\xi)\right]$, $\beta = \E\left[\delta(z+\tau \be)\right]$ and use Lemma \ref{lm:shamirLm9} along with the fact that $f(z+\tau\be,\xi)$ is $\tau M_2(\xi)$-Lipschitz continuous, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus, it holds for the Eq. \eqref{eq:funcsq:separated}  
\begin{align}\label{eq:finlhkjfsvn:separated}
    \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[\sqrt{\E_{\be} \left[ f(z+\tau \be,\xi)-\alpha)^4\right]}\right]
    &\leq \frac{d^2 a_{q_x}^2}{\tau^2} \cdot c\frac{\tau^2 \E M_2^2(\xi)}{d} = c d a_{q_x}^2 M_2^2.  
    %\red{\text{it seems should be} \leq}
\end{align}
\begin{enumerate}
    \item Under the Assumption \ref{ass:err_noise}
     for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE:separated}, the following holds
    \begin{align}\label{eq:fgkssssffdgh:separated}
        &\frac{d^2}{4\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \leq  \frac{d^2\Delta^2}{\tau^2} \E \left[ \|\be_x\|_{q_x}^2  \right]\leq \frac{d^2 a_{q_x}^2\Delta^2}{\tau^2}.
    \end{align}
   % where we used $\sqrt{\E_{\be} \left[ \|\be\|_q^4\right]} \leq a_q^2$.
    \item Under the Assumption \ref{ass:Lip_noise}
    for the second term in the r.h.s. of Eq. \eqref{eq:sqnormE:separated}, the following holds with an arbitrary parameter $\beta$
    \begin{align}\label{eq:fgklljgsdgh:separated}
        &\frac{d^2}{4\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)  -\delta(z-\tau\be)  \right)^2 \right] \notag \\
     &= \frac{d^2}{2\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left((\delta(z+\tau\be) -\beta) -(\delta(z-\tau\be)  -\beta) \right)^2 \right] \notag\\
    &\leq \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left((\delta(z+\tau\be)-\beta)^2  +(\delta(z-\tau\be) -\beta)^2 \right) \right] \qquad /* \forall a,b, (a-b)^2\leq 2a^2+2b^2 */ \notag\\
    &= \frac{d^2}{2\tau^2}\left(\E \left[ \|\be_x\|_{q_x}^2 (\delta(z+\tau \be)-\beta)^2 \right] + \E \left[\|\be_x\|_{q_x}^2(\delta(z-\tau \be) -\beta)^2 \right] \right) \notag\\
    &= \frac{d^2}{\tau^2}\E \left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]. \qquad /* \mbox{ the distribution of $\be$ is  symmetric  } */
    \end{align}
\end{enumerate}





and for the second term in the Eq. \eqref{eq:sqnormE:separated}, we get
\begin{align}\label{eq:noisesq:separated}
   \frac{d^2}{\tau^2}\E\left[ \|\be_x\|_{q_x}^2 \left(\delta(z+\tau\be)-\beta  \right)^2 \right]
   &\leq \frac{d^2}{\tau^2}\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \sqrt{\E \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \notag \\
   &\leq \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[ \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \right]
\end{align}

Then we assume  $\beta = \E\left[\delta(z+\tau \be)\right]$ and use Lemma \ref{lm:shamirLm9} together with the fact that $\delta(z+\tau\be)$ is $\tau M_{2,\delta}$-Lipschitz continuous, w.r.t. $\be$ in terms of the $\ell_2$-norm. Thus, Eq. \eqref{eq:noisesq:separated} can be rewritten as 
\begin{align}\label{eq:fkssoomnbd:separated}
    \frac{d^2 a_{q_x}^2}{\tau^2} \E_{\xi}\left[ \sqrt{\E_{\be} \left[ \left(\delta(z+\tau\be)-\beta  \right)^4 \right] } \right]
    &\leq \frac{d^2 a_{q_x}^2}{\tau^2}  \cdot c\frac{\tau^2  M_{2,\delta}^2}{d} \leq c a^2_{q_x} d M_{2,\delta}^2. 
    %\red{\text{it seems should be} \leq}
\end{align}

Using Eq. \eqref{eq:finlhkjfsvn:separated} and \eqref{eq:fgkssssffdgh:separated} (or Eq. \eqref{eq:fkssoomnbd:separated}) for Eq. \eqref{eq:sqnormE:separated}, we get the statement of the lemma.
\end{proof}







\begin{proof}[Proof of the  Theorem \ref{th:conv_rate}]
By the definitions 
$$x^{k+1}= {\rm Prox}_{x^k}\left(\gamma_k g_x(z^k,\be^k,\xi^k) \right),$$ 
$$y^{k+1}= {\rm Prox}_{y^k}\left(\gamma_k g_y(z^k,\be^k,\xi^k) \right)$$
we get  \cite{ben2001lectures}, for all $u = (x, y) \in \X \times \Y$
\begin{align}
   \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \leq V_{x^k}(x) - V_{x^{k+1}}(x) - \gamma_k^2\|g_x(z^k,\be^k,\xi^k)\|_{q_x}^2/2   \notag
\end{align}
\begin{align}
   \gamma_k\la g_y(z^k,\be^k,\xi^k), y^k-y\ra \leq V_{y^k}(y) - V_{y^{k+1}}(y) - \gamma_k^2\|g_y(z^k,\be^k,\xi^k)\|_{q_y}^2/2   \notag
\end{align}
where $V_x, V_y$ are Bregman divergences in $\X$ and $\Y$ spaces respectively.
Summing for $k=1,\dots,N$  and taking the expectation, we obtain, for all $u\in \Z$
\begin{align}\label{eq:inmainsqE:separated}
   \E\left[\sum_{k=1}^N \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \right]
   &\leq V_{x^1}(x)  - \E\left[\sum_{k=1}^N\gamma_k^2\|g_x(z^k,\be^k,\xi^k)\|_{q_x}^2/2 \right] \notag\\
   &\leq  \D_x^2 + \sum_{k=1}^N \frac{\gamma_k^2}{2} \E\left[\|g_x(z^k,\be^k,\xi^k)\|_{q_x}^2\right], 
\end{align}
\begin{align}\label{eq:inmainsqE_y:separated}
   \E\left[\sum_{k=1}^N \gamma_k\la g_y(z^k,\be^k,\xi^k), y^k-y\ra \right]
   &\leq V_{y^1}(y)  - \E\left[\sum_{k=1}^N\gamma_k^2\|g_y(z^k,\be^k,\xi^k)\|_{q_y}^2/2 \right] \notag\\
   &\leq  \D_y^2 + \sum_{k=1}^N \frac{\gamma_k^2}{2} \E\left[\|g_y(z^k,\be^k,\xi^k)\|_{q_y}^2\right], 
\end{align}
where $\mathcal D_x = \max_{x, \xi\in \X}\sqrt{2V_{x}(\xi)}$, $\mathcal D_x = \max_{y , \zeta \in \Y}\sqrt{2V_{y}(\zeta)}$ are the diameters  of $\X, \Y$. In what follows, we deal only with the variable $x$, taking into account the fact that the calculations for the other variable are similar.

{\bf Step 1.}\\
For the second term in the r.h.s of inequality \eqref{eq:inmainsqE:separated} we use Lemma \ref{lm:shamirEnabla:separated} and obtain
 \begin{enumerate}
     \item  under Assumption  \ref{ass:err_noise}
     \begin{equation}\label{eq:inmainsqEtwo1:separated}
        \E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} dM_2^2 + \frac{d^2 a_{q_x}^2\Delta^2}{\tau^2}, 
     \end{equation}
     \item  under Assumption \ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo:separated}
    \E\left[\|g_x(z,\xi,\be)\|^2_{q_x}\right] \leq c a^2_{q_x} d (M_2^2+M_{2,\delta}^2),
\end{align}
 \end{enumerate}
 where    $c$ is some numerical constant and $\sqrt{\E_{\be} \left[ \|\be_x\|_{q_x}^4\right]} \leq a_{q_x}^2$.

{\bf Step 2.}\\
For the l.h.s. of  Eq. \eqref{eq:inmainsqE:separated}, we use Lemma \ref{lm:expecapproxgrad}


 \begin{enumerate}
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz11:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \right] &=  \E\left[\sum_{k=1}^N \gamma_k\la \E\left[g_x(z^k,\be^k,\xi^k)\mid z^k \right], x^k-x\ra \right] \notag\\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k\left\la \nabla_x f^\tau(z^k) - \frac{d\Delta}{\tau}  \be^k_x, x^k-x\right\ra \right].
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g_x(z^k,\be^k,\xi^k), x^k-x\ra \right] &=  \E\left[\sum_{k=1}^N \gamma_k\la \E\left[g_x(z^k,\be^k,\xi^k)\mid z^k \right], x^k-x\ra \right] \notag\\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(z^k) - dM_{2,\delta} \be^k_x, x^k-x\ra \right].
\end{align}
 \end{enumerate}



For the first term of the r.h.s. of Eq.\eqref{eq:eqrefeqffxyz11:separated} and \eqref{eq:eqrefeqffxyz:separated} we have 
\begin{align}\label{eq:eqexpfxy:separated_x}
     \E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(z^k), x^k-x\ra \right]
     &=  \E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(x^k,y^k), x^k-x \ra\right] \notag \\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k ( f^\tau(x^k,y^k) - f^\tau(x,y^k))\right].
\end{align}
By exactly the same calculations, we get the inequality for dual variable $y$
\begin{align}\label{eq:eqexpfxy:separated_y}
     \E\left[\sum_{k=1}^N \gamma_k\la \nabla_y f^\tau(z^k), y^k-y\ra \right]
     &=  \E\left[\sum_{k=1}^N \gamma_k\la -\nabla_y f^\tau(x^k,y^k), y^k-y \ra\right] \notag \\
     &\geq  \E\left[\sum_{k=1}^N \gamma_k (  - f^\tau(x^k,y^k) + f^\tau(x^k,y))\right]. 
\end{align}

Summing up the inequalities \eqref{eq:eqexpfxy:separated} and \eqref{eq:eqexpfxy:separated_y} we have
\begin{align}\label{eq:eqexpfxy:separated}
\E\left[\sum_{k=1}^N \gamma_k\la \nabla_x f^\tau(z^k), x^k-x\ra \right] \notag &+ \E\left[\sum_{k=1}^N \gamma_k\la \nabla_y f^\tau(z^k), y^k-y\ra \right] \notag \\
&\geq \E\left[\sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \right].
\end{align}
Then we use the fact function $f^\tau(x,y)$ is convex in $x$ and concave in $y$ and  obtain 
\begin{align}\label{eq:fineqE:separated}
     &\E\left[\frac{1}{\sum_{i=1}^{N}\gamma_k} \sum_{k=1}^N \gamma_k (f^\tau(x^k,y)  - f^\tau(x,y^k)) \right] \notag \\
     &\hspace{2cm}\leq \E\left[ f^\tau\left(\frac{1}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \gamma_k x^k,y\right)  - f^\tau\left(x, \frac{1}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \gamma_k y^k\right) \right]\notag \\
     &\hspace{2cm}= \E\left[ f^\tau\left(\hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right],
\end{align}
where $ (\hat x^N, \hat y^N)$ is the output of the Algorithm. 
Using Eq. \eqref{eq:fineqE:separated}  for Eq. \eqref{eq:eqexpfxy:separated} we get 
\begin{align}\label{eq:fpslff:separated}
      \E\left[\sum_{k=1}^N \gamma_k\la \nabla f^\tau(z^k), z^k-u\ra \right] 
     &\geq \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right].
\end{align}
Next we estimate the term $\E_{\be_x^k} \left[   \left| \la \be_x^k, x^k-x\ra \right| \right] $ in Eq. \eqref{eq:eqrefeqffxyz11:separated} and \eqref{eq:eqrefeqffxyz:separated}  by the Lemma  \ref{lm:dotprodvece}  
\begin{align}\label{eq:sectermErhs:separated}
  \E_{\be_x^k} \left[    \left|\la \be_x^k, x^k-x\ra \right| \right] \leq  \frac{\D_x}{\sqrt{d_x}},
\end{align}
and similarly 
\begin{align}\label{eq:sectermErhs:separated_y}
  \E_{\be_x^k} \left[   \left| \la \be_y^k, y^k-y\ra \right| \right] \leq  \frac{\D_y}{\sqrt{d_y}}.
\end{align}
Now  we substitute  Eq. \eqref{eq:fpslff:separated}, \eqref{eq:sectermErhs:separated_y} and  \eqref{eq:sectermErhs:separated} to Eq. \eqref{eq:eqrefeqffxyz11:separated} and \eqref{eq:eqrefeqffxyz:separated} summed with similar ones for the variable $y$, and get
 \begin{enumerate}
 \item under Assumption \ref{ass:err_noise}
 \begin{align}\label{eq:eqrefeqffxyz1122:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] &\geq 
     \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)- f^\tau\left(x, \hat y^N \right) \right] \notag \\ 
     &-  \sum_{k=1}^N \gamma_k \Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right).  
\end{align}
     \item  under Assumption \ref{ass:Lip_noise}      
\begin{align}\label{eq:eqrefeqffxyz22:separated}
     \E\left[\sum_{k=1}^N \gamma_k\la g(z^k,\be^k,\xi^k), z^k-u\ra \right] &\geq  \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right) - f^\tau\left(x, \hat y^N \right) \right] \notag\\
     &- \sum_{k=1}^N \gamma_k M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right). 
\end{align}
 \end{enumerate}
 
{\bf Step 3.} (under Assumption \ref{ass:err_noise}) \\
Now we combine Eq. \eqref{eq:eqrefeqffxyz1122:separated}   with  Eq. \eqref{eq:inmainsqEtwo1:separated} for sum of Eq. \eqref{eq:inmainsqE:separated}, \eqref{eq:inmainsqE_y:separated} and obtain under Assumption \ref{ass:err_noise} the following
     \begin{align}\label{eq:inmainsqEtwo133:separated}
     &\sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
     -  \sum_{k=1}^N \gamma_k \Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)  \notag \\
     &\leq \D_x^2 + \D_y^2 +  \sum_{k=1}^N \frac{\gamma_k^2}{2} \left(c a^2_{q_x} dM_2^2 + c a^2_{q_y} dM_2^2 + \frac{d^2 a_{q_x}^2\Delta^2}{\tau^2} + \frac{d^2 a_{q_y}^2\Delta^2}{\tau^2}\right).
     \end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE1:separated}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      \leq 
     \frac{ \D^2}{\sum_{k=1}^{N}\gamma_k}
      &+\frac{c (a^2_{q_x}+a^2_{q_y}) dM_2^2+ d^2 (a^2_{q_x}+a^2_{q_y})\Delta^2\tau^{-2}}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2}  \notag\\
      &+\Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right).
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE1:separated} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE1:separated} and   taking $(x,y) = (x_*,y_*)$
%  the maximum in $(x,y) \in (\X,\Y)$,
 we obtain
 \begin{align}\label{eq:dghjsklslsl1:separated}
     \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
     &\leq \frac{ \D^2+ (c d M_2^2 +
     d^2\Delta^2\tau^{-2}) (a^2_{q_x}+a^2_{q_y})
    \sum_{k=1}^{N} {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
       \notag \\
    &+ \Delta \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Choosing the learning rate $\gamma_k 
=\frac{\D}{M_{\rm case1}}\sqrt{\frac{2}{N}}$ with $M^2_{\rm case1} \triangleq (c d M_2^2 +
     d^2\Delta^2\tau^{-2}) (a^2_{q_x}+a^2_{q_y})$ in Eq. \eqref{eq:dghjsklslsl1:separated} we obtain
 \begin{align*}
      \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
     &\leq  
     %\frac{\D(1+ ca_q^2dM_2^2 + d^2a_q^2\Delta^2\tau^{-2})}{\sqrt{2N} M_2}  
     \sqrt{\frac{2}{N}}M_{\rm case1}\D
     + \Delta\left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align*}
 
 {\bf Step 4.} (under Assumption \ref{ass:Lip_noise})\\
Now we combine Eq.  \eqref{eq:eqrefeqffxyz22:separated}  with  Eq.  \eqref{eq:inmainsqEtwo:separated} for sum of Eq. \eqref{eq:inmainsqE:separated}, \eqref{eq:inmainsqE_y:separated} and obtain under Assumption \ref{ass:Lip_noise} 
\begin{align}\label{eq:inmainsqEtwo334:separated}
    \sum_{k=1}^{N}\gamma_k \E\left[ f^\tau\left( \hat x^N,y\right)  - f^\tau\left(x, \hat y^N \right) \right] 
    &- \sum_{k=1}^N \gamma_k M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)\notag \\ &\leq \D^2 
    +  \sum_{k=1}^N \frac{\gamma_k^2}{2} c (a^2_{q_x} + a^2_{q_y}) d (M_2^2+M_{2,\delta}^2).
\end{align}
 We can rewrite this as follows
 \begin{align}\label{eq:exEeqE:separated}
       \E\left[ f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) \right]  
      &\leq 
     \frac{ \D^2}{\sum_{k=1}^{N}\gamma_k}
      +\frac{c (a^2_{q_x} + a^2_{q_y}) d (M_2^2+M_{2,\delta}^2)}{\sum_{k=1}^{N}\gamma_k}\sum_{k=1}^N \frac{\gamma_k^2}{2} \notag \\ &+ M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right). 
 \end{align}
 For the l.h.s. of Eq. \eqref{eq:exEeqE:separated} we use Lemma \ref{lm:shamirSmoothFun} and obtain
 \begin{align*}
    f^\tau\left( \hat x^N,y\right) -  f^\tau\left(x, \hat y^N \right) 
    &\geq f\left( \hat x^N,y\right) -  f\left(x, \hat y^N \right)  - 2\tau M_2.
 \end{align*}
 Using this for Eq. \eqref{eq:exEeqE:separated} and   taking $(x,y) =(x_*,y_*)$
%  the maximum in $(x,y) \in (\X,\Y)$,
 we obtain
 \begin{align}\label{eq:dghjsklslsl:separated}
     \E\left[ 
    %  \max_{y \in \Y}
     f\left( \hat x^N,y_*\right) -  
    %  \min_{x\in \X}
     f\left(x_*, \hat y^N \right)\right]
     &\leq \frac{ \D^2+ c (a^2_{q_x} + a^2_{q_y}) d (M_2^2+M_{2,\delta}^2)\sum_{k=1}^N {\gamma_k^2}/{2}}{\sum_{k=1}^{N}\gamma_k}
    \notag \\&+ M_{2,\delta}  \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align}
 Choosing the learning rate 
%   $\gamma_k 
% =\frac{\D}{M_2}\sqrt{\frac{2}{N}}$  in Eq. \eqref{eq:dghjsklslsl} we obtain
%  \begin{align*}
%       \E\left[ \max_{y \in \Y} f\left( \hat x^N,y\right) -  \min_{x\in \X} f\left(x, \hat y^N \right)\right]
%      &\leq  \frac{\D(1+c a^2_q d M_2^2 + c a^2_q dM_{2,\delta}^2)}{\sqrt{2N}M}  + M_{2,\delta} \D \sqrt{d} 
%      +  2\tau M_2.  
%  \end{align*}
 $\gamma_k 
=\frac{\D}{M_{\rm case2}}\sqrt{\frac{2}{N}}$ with $M_{\rm case2}^2 \triangleq c d (a^2_{q_x} + a^2_{q_y})(M_2^2+M_{2,\delta}^2)$ in Eq. \eqref{eq:dghjsklslsl1:separated} we obtain
 \begin{align*}
      \E\left[ 
    %   \max_{y \in \Y} 
      f\left( \hat x^N,y_*\right) - 
    %   \min_{x\in \X} 
      f\left(x_*, \hat y^N \right)\right]
     &\leq  \sqrt{\frac{2}{N}}M_{\rm case2}\D  + M_{2,\delta} \left( \frac{d\D_x}{\sqrt{d_x}\tau} + \frac{d\D_y}{\sqrt{d_y}\tau}\right)
     +  2\tau M_2.  
 \end{align*}
\end{proof}

